NNLO QCD corrections to jet production in deep inelastic scattering

Hadronic jets in deeply inelastic electron-proton collisions are produced by the scattering of a parton from the proton with the virtual gauge boson mediating the interaction. The HERA experiments have performed precision measurements of inclusive single jet production and di-jet production in the Breit frame, which provide important constraints on the strong coupling constant and on parton distributions in the proton. We describe the calculation of the next-to-next-to-leading order (NNLO) QCD corrections to these processes, and assess their size and impact. A detailed comparison with data from the H1 and ZEUS experiments highlights that inclusive single jet production displays a better perturbative convergence than di-jet production. We also observe that the event selection cuts in some of the di-jet measurements of both H1 and ZEUS induce an infrared sensitivity that destabilises the perturbative stability of the predictions. Our results open up new opportunities for QCD precision studies with jet production observables in deep inelastic scattering.

==> sub/autog1Bh2g1ATgtoq.tex <==
\section*{g1Bh2g1ATgtoq(1,j,k,i,6,2)}
\begin{eqnarray}
  \ph{1}&&-2J_{2,QQ,g \to q}^{1,IF}(s_{1i})\,C_0^{\gamma,0}(1,j,k,i,6,2)\,J_2^{(3)}(\lbrace p\rbrace_{3})\nonumber\\
 \ph{2}&& +J_{2,QQ,g \to q}^{1,IF}(s_{1(\widetilde{ij})})
\,E_3^{0}(i,j,k)\,B_1^{\gamma,0}((\widetilde{ij}),(\widetilde{jk}),1,6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})  \nonumber\\
 \ph{3}&& +J_{2,QQ,g \to q}^{1,IF}(s_{\overline{1}i})
\,E_{3,q}^{0}(1,j,k)\,B_1^{\gamma,0}(i,(\widetilde{jk}),\overline{1},6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})  \nonumber\\
 \ph{4}&&+\bigg[ -2J_{2,QQ,g \to q}^{1,IF}(s_{1i})
 +2J_{2,QQ,g \to q}^{1,IF}(s_{\overline{1}i})
\bigg]  E_{3,q}^{0}(1,j,k)\,B_1^{\gamma,0}((\widetilde{jk}),\overline{1},i,6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})  \nonumber\\
\end{eqnarray}


==> sub/autog1Bth2g1ATgtoq.tex <==
\section*{g1Bth2g1ATgtoq(j,1,i,k,6,2)}
\begin{eqnarray}
  \ph{1}&&-2J_{2,QQ,g \to q}^{1,IF}(s_{1i})\,C_0^{\gamma,0}(k,1,i,j,6,2)\,J_2^{(3)}(\lbrace p\rbrace_{3})\nonumber\\
 \ph{2}&& +J_{2,QQ,g \to q}^{1,IF}(s_{1(\widetilde{ij})})
\,E_3^{0}(i,j,k)\,B_1^{\gamma,0}((\widetilde{ij}),(\widetilde{jk}),1,6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})  \nonumber\\
 \ph{3}&& +J_{2,QQ,g \to q}^{1,IF}(s_{\overline{1}i})
\,E_3^{0}(1,j,k)\,B_1^{\gamma,0}(i,(\widetilde{jk}),\overline{1},6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})  \nonumber\\
\end{eqnarray}


==> sub/autog1C1g0AS.tex <==
\section*{g1C1g0AS(k,1,i,j,l,7,2)}
\begin{eqnarray}
 \ph{1}&&+E_3^{0}(l,i,j)\,B_2^{\gamma,0}(k,(\widetilde{ji}),1,(\widetilde{li}),7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{2}&&+E_3^{0}(k,j,i)\,B_2^{\gamma,0}((\widetilde{kj}),1,(\widetilde{ji}),l,7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{3}&&-a_{3,g\to q}^{0}(k,1,l)\,C_0^{\gamma,0}(\overline{1},i,j,(\widetilde{kl}),7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{4}&&-a_{3,g\to q}^{0}(l,1,k)\,C_0^{\gamma,0}((\widetilde{kl}),i,j,\overline{1},7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{5}&&-a_{3,g\to q}^{0}(i,1,j)\,C_0^{\gamma,0}(k,\overline{1},(\widetilde{ij}),l,7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{6}&&-a_{3,g\to q}^{0}(j,1,i)\,C_0^{\gamma,0}(k,(\widetilde{ij}),\overline{1},l,7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{7}&&+\,E_3^{0}(k,j,i)\,a_{3,g\to q}^{0}((\widetilde{kj}),1,l)\,B_1^{\gamma,0}(\overline{1},(\widetilde{ij}),(\widetilde{(\widetilde{kj})l}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{8}&&+\,E_3^{0}(l,i,j)\,a_{3,g\to q}^{0}((\widetilde{li}),1,k)\,B_1^{\gamma,0}((\widetilde{(\widetilde{li})k}),(\widetilde{ij}),\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\snip \ph{9}&&+\,E_4^0(l,i,j,1)\,B_1^{\gamma,0}(k,\overline{1},(\widetilde{lij}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\snip \ph{10}&&+\,E_4^0(k,j,i,1)\,B_1^{\gamma,0}((\widetilde{kji}),\overline{1},l,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{11}&&-\,A_3^{0}(k,1,l)\,E_3^{0}(\overline{1},j,i)\,B_1^{\gamma,0}((\widetilde{kl}),\overline{\overline{1}},(\widetilde{ij}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{12}&&+\,E_3^{0}(k,j,i)\,a_{3,g\to q}^{0}((\widetilde{kj}),1,l)\,B_1^{\gamma,0}((\widetilde{(\widetilde{kj})l}),\overline{1},(\widetilde{ij}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{13}&&+\,E_3^{0}(l,i,j)\,a_{3,g\to q}^{0}((\widetilde{li}),1,k)\,B_1^{\gamma,0}((\widetilde{(\widetilde{li})k}),\overline{1},(\widetilde{ij}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{14}&&-\,a_{3,g\to q}^{0}(i,1,j)\,E_3^{0}(k,(\widetilde{ij}),\overline{1})\,B_1^{\gamma,0}((\widetilde{k\widetilde{(ij})}),\overline{\overline{1}},l,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{15}&&-\,a_{3,g\to q}^{0}(j,1,i)\,E_3^{0}(l,(\widetilde{ij}),\overline{1})\,B_1^{\gamma,0}(k,\overline{\overline{1}},(\widetilde{l\widetilde{(ij})}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{16}&&-\,E_3^{0}(k,j,i)\,d_{3,g\to q}^{0}((\widetilde{kj}),1,(\widetilde{ij}))\,B_1^{\gamma,0}([(\widetilde{kj}), (\widetilde{ij})],\overline{1},l,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{17}&&-\,E_3^{0}(l,i,j)\,d_{3,g}^{0}(k,(\widetilde{ij}),1)\,B_1^{\gamma,0}((\widetilde{k\widetilde{(ij})}),\overline{1},(\widetilde{li}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{18}&&-\,E_3^{0}(l,i,j)\,d_{3,g\to q}^{0}((\widetilde{li}),1,(\widetilde{ij}))\,B_1^{\gamma,0}(k,\overline{1},[(\widetilde{li}), (\widetilde{ij})],7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{19}&&-\,E_3^{0}(k,j,i)\,d_{3,g}^{0}(l,(\widetilde{ij}),1)\,B_1^{\gamma,0}((\widetilde{kj}),\overline{1},(\widetilde{l\widetilde{(ij})}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\end{eqnarray}


==> sub/autog1Ct1g0AS.tex <==
\section*{g1Ct1g0AS(k,1,i,j,l,7,2)}
\begin{eqnarray}
 \ph{1}&&+\frac{1}{2}\,E_3^{0}(k,i,j)\,\tilde{B}_2^{\gamma,0}((\widetilde{ki}),1,(\widetilde{ij}),l,7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{2}&&+\frac{1}{2}\,E_3^{0}(l,i,j)\,\tilde{B}_2^{\gamma,0}(k,(\widetilde{ij}),1,(\widetilde{li}),7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{3}&&-a_{3,g\to q}^{0}(i,1,j)\,C_0^{\gamma,0}(k,\overline{1},(\widetilde{ij}),l,7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{4}&&-a_{3,g\to q}^{0}(k,1,l)\,C_0^{\gamma,0}(\overline{1},i,j,(\widetilde{kl}),7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{5}&&-a_{3,g\to q}^{0}(j,1,i)\,C_0^{\gamma,0}(k,(\widetilde{ij}),\overline{1},l,7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{6}&&-a_{3,g\to q}^{0}(l,1,k)\,C_0^{\gamma,0}((\widetilde{kl}),i,j,\overline{1},7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
\snip \ph{7}&&+\,B_4^0(k,i,j,l)\,B_1^{\gamma,0}((\widetilde{kij}),1,(\widetilde{lji}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{8}&&-\frac{1}{2}\,\,E_3^{0}(k,i,j)\,A_3^{0}((\widetilde{ki}),(\widetilde{ij}),l)\,B_1^{\gamma,0}([(\widetilde{ki}), (\widetilde{ij})],1,(\widetilde{l\widetilde{(ij})}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{9}&&-\frac{1}{2}\,\,E_3^{0}(l,i,j)\,A_3^{0}((\widetilde{li}),(\widetilde{ij}),k)\,B_1^{\gamma,0}((\widetilde{k\widetilde{(ij})}),1,[(\widetilde{li}), (\widetilde{ij})],7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\snip \ph{10}&&+\frac{1}{2}\,\,\tilde{E}_4^0(k,i,1,j)\,B_1^{\gamma,0}((\widetilde{kij}),\overline{1},l,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{11}&&-\frac{1}{2}\,\,A_3^{0}(i,1,j)\,E_{3,q^\prime\to g}^{0}(k,\overline{1},(\widetilde{ij}))\,B_1^{\gamma,0}((\widetilde{k\widetilde{(ij})}),\overline{\overline{1}},l,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\snip \ph{12}&&+\frac{1}{2}\,\,\tilde{E}_4^0(l,i,1,j)\,B_1^{\gamma,0}(k,\overline{1},(\widetilde{lij}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{13}&&-\frac{1}{2}\,\,A_3^{0}(i,1,j)\,E_{3,q^\prime\to g}^{0}(l,\overline{1},(\widetilde{ij}))\,B_1^{\gamma,0}(k,\overline{\overline{1}},(\widetilde{l\widetilde{(ij})}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{14}&&+\frac{1}{2}\,\,E_3^{0}(k,i,j)\,A_3^{0}((\widetilde{ki}),1,l)\,B_1^{\gamma,0}(\overline{1},(\widetilde{ij}),(\widetilde{l\widetilde{(ki})}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{15}&&+\frac{1}{2}\,\,E_3^{0}(l,i,j)\,A_3^{0}((\widetilde{li}),1,k)\,B_1^{\gamma,0}(\overline{1},(\widetilde{ij}),(\widetilde{k\widetilde{(li})}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\end{eqnarray}


==> sub/autog2Bh2g1ATgtoq.tex <==
\section*{g2Bh2g1ATgtoq(1,j,k,i,6,2)}
\begin{eqnarray}
 \ph{1}&& -J_{2,QQ,g \to q}^{1,IF}(s_{1i})
\,E_{3,q^\prime\to g}^{0}(j,1,i)\,B_1^{\gamma,0}((\widetilde{ij}),\overline{1},k,6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})  \nonumber\\
 \ph{2}&& -J_{2,QQ,g \to q}^{1,IF}(s_{1i})
\,E_{3,q^\prime\to g}^{0}(k,1,i)\,B_1^{\gamma,0}((\widetilde{ik}),\overline{1},j,6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})  \nonumber\\
\end{eqnarray}


==> sub/autog2Bth2g1ATgtoq.tex <==
\section*{g2Bth2g1ATgtoq(j,1,i,k,6,2)}
\begin{eqnarray}
 \ph{1}&& -J_{2,QQ,g \to q}^{1,IF}(s_{1i})
\,E_{3,q^\prime\to g}^{0}(j,1,i)\,B_1^{\gamma,0}((\widetilde{ji}),\overline{1},k,6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})  \nonumber\\
 \ph{2}&& -J_{2,QQ,g \to q}^{1,IF}(s_{1i})
\,E_{3,q^\prime\to g}^{0}(k,1,i)\,B_1^{\gamma,0}((\widetilde{ki}),\overline{1},j,6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})  \nonumber\\
\end{eqnarray}


==> sub/autog2C1g0AS.tex <==
\section*{g2C1g0AS(k,1,i,j,l,7,2)}
\begin{eqnarray}
 \ph{1}&&+E_3^{0}(j,k,l)\,B_2^{\gamma,0}((\widetilde{jk}),1,(\widetilde{lk}),i,7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{2}&&+E_3^{0}(i,l,k)\,B_2^{\gamma,0}(j,(\widetilde{lk}),1,(\widetilde{il}),7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{3}&&+\,E_3^{0}(i,l,k)\,a_{3,g\to q}^{0}((\widetilde{il}),1,j)\,B_1^{\gamma,0}((\widetilde{(\widetilde{il})j}),(\widetilde{kl}),\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{4}&&+\,E_3^{0}(j,k,l)\,a_{3,g\to q}^{0}((\widetilde{jk}),1,i)\,B_1^{\gamma,0}((\widetilde{(\widetilde{jk})i}),(\widetilde{kl}),\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\snip \ph{5}&&+\,E_4^0(i,l,k,1)\,B_1^{\gamma,0}(j,\overline{1},(\widetilde{kli}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\snip \ph{6}&&+\,E_4^0(j,k,l,1)\,B_1^{\gamma,0}((\widetilde{lkj}),\overline{1},i,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{7}&&-\,A_3^{0}(i,1,j)\,E_3^{0}(\overline{1},k,l)\,B_1^{\gamma,0}((\widetilde{ij}),\overline{\overline{1}},(\widetilde{kl}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{8}&&+\,E_3^{0}(i,l,k)\,a_{3,g\to q}^{0}((\widetilde{il}),1,j)\,B_1^{\gamma,0}((\widetilde{(\widetilde{il})j}),\overline{1},(\widetilde{kl}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{9}&&+\,E_3^{0}(j,k,l)\,a_{3,g\to q}^{0}((\widetilde{jk}),1,i)\,B_1^{\gamma,0}((\widetilde{(\widetilde{jk})i}),\overline{1},(\widetilde{kl}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{10}&&-\,a_{3,g\to q}^{0}(k,1,l)\,E_3^{0}(i,(\widetilde{kl}),\overline{1})\,B_1^{\gamma,0}(j,\overline{\overline{1}},(\widetilde{i\widetilde{(kl})}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{11}&&-\,a_{3,g\to q}^{0}(l,1,k)\,E_3^{0}(j,(\widetilde{kl}),\overline{1})\,B_1^{\gamma,0}((\widetilde{j\widetilde{(kl})}),\overline{\overline{1}},i,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{12}&&-\,E_3^{0}(i,l,k)\,d_{3,g\to q}^{0}((\widetilde{il}),1,(\widetilde{kl}))\,B_1^{\gamma,0}(j,\overline{1},[(\widetilde{il}), (\widetilde{kl})],7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{13}&&-\,E_3^{0}(j,k,l)\,d_{3,g}^{0}(i,(\widetilde{kl}),1)\,B_1^{\gamma,0}((\widetilde{jk}),\overline{1},(\widetilde{i\widetilde{(kl})}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{14}&&-\,E_3^{0}(j,k,l)\,d_{3,g\to q}^{0}((\widetilde{jk}),1,(\widetilde{kl}))\,B_1^{\gamma,0}([(\widetilde{jk}), (\widetilde{kl})],\overline{1},i,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{15}&&-\,E_3^{0}(i,l,k)\,d_{3,g}^{0}(j,(\widetilde{kl}),1)\,B_1^{\gamma,0}((\widetilde{j\widetilde{(kl})}),\overline{1},(\widetilde{il}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\end{eqnarray}


==> sub/autog2Ct1g0AS.tex <==
\section*{g2Ct1g0AS(k,1,i,j,l,7,2)}
\begin{eqnarray}
 \ph{1}&&+\frac{1}{2}\,E_3^{0}(i,k,l)\,\tilde{B}_2^{\gamma,0}(j,(\widetilde{kl}),1,(\widetilde{ik}),7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{2}&&+\frac{1}{2}\,E_3^{0}(j,k,l)\,\tilde{B}_2^{\gamma,0}((\widetilde{jk}),1,(\widetilde{kl}),i,7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
\snip \ph{3}&&+\,B_4^0(i,k,l,j)\,B_1^{\gamma,0}((\widetilde{jlk}),1,(\widetilde{ikl}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{4}&&-\frac{1}{2}\,\,E_3^{0}(i,k,l)\,A_3^{0}((\widetilde{ik}),(\widetilde{kl}),j)\,B_1^{\gamma,0}((\widetilde{j\widetilde{(kl})}),1,[(\widetilde{ik}), (\widetilde{kl})],7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{5}&&-\frac{1}{2}\,\,E_3^{0}(j,k,l)\,A_3^{0}((\widetilde{jk}),(\widetilde{kl}),i)\,B_1^{\gamma,0}([(\widetilde{jk}), (\widetilde{kl})],1,(\widetilde{i\widetilde{(kl})}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\snip \ph{6}&&+\frac{1}{2}\,\,\tilde{E}_4^0(i,k,1,l)\,B_1^{\gamma,0}(j,\overline{1},(\widetilde{ikl}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{7}&&-\frac{1}{2}\,\,A_3^{0}(k,1,l)\,E_{3,q^\prime\to g}^{0}(i,\overline{1},(\widetilde{kl}))\,B_1^{\gamma,0}(j,\overline{\overline{1}},(\widetilde{i\widetilde{(kl})}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\snip \ph{8}&&+\frac{1}{2}\,\,\tilde{E}_4^0(j,k,1,l)\,B_1^{\gamma,0}((\widetilde{jkl}),\overline{1},i,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{9}&&-\frac{1}{2}\,\,A_3^{0}(k,1,l)\,E_{3,q^\prime\to g}^{0}(j,\overline{1},(\widetilde{kl}))\,B_1^{\gamma,0}((\widetilde{j\widetilde{(kl})}),\overline{\overline{1}},i,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{10}&&+\frac{1}{2}\,\,E_3^{0}(i,k,l)\,A_3^{0}((\widetilde{ik}),1,j)\,B_1^{\gamma,0}((\widetilde{j\widetilde{(ik})}),(\widetilde{kl}),\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{11}&&+\frac{1}{2}\,\,E_3^{0}(j,k,l)\,A_3^{0}((\widetilde{jk}),1,i)\,B_1^{\gamma,0}((\widetilde{i\widetilde{(jk})}),(\widetilde{kl}),\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\end{eqnarray}


==> sub/autogB1g2AU.tex <==
\section*{gB1g2AU}
\begin{eqnarray}
\lefteqn{{\tt gB1g2AU(3,1,4,5,2) =}} \\
 \ph{1}&&+\bigg[ 
 -\,{\cal D}_{3,g\to g}^{0}(s_{13}) 
 +\,\Gamma^{(1)}_{gg}(z_1) 
 -\,{\cal D}_{3,g\to g}^{0}(s_{14}) 
 \bigg] 
\left( -\frac{b_0}{\epsilon}B_1^{\gamma,0}(3,1,4,5,2) +B_1^{\gamma,1}(3,1,4,5,2)\right)
 \nonumber\\
 \ph{2}&&+\bigg[ 
 -\frac{1}{2}\,\,{\cal D}_{3,g\to g}^{0}(s_{14})\otimes{\cal D}_{3,g\to g}^{0}(s_{14}) 
 -\frac{1}{2}\,\,{\cal D}_{3,g\to g}^{0}(s_{13})\otimes{\cal D}_{3,g\to g}^{0}(s_{13}) 
 -\,{\cal D}_{3,g\to g}^{0}(s_{13})\otimes{\cal D}_{3,g\to g}^{0}(s_{14}) 
 \nonumber \\ && \phantom{+\bigg[} 
 +\,\Gamma^{(1)}_{gg}(z_1)\otimes{\cal D}_{3,g\to g}^{0}(s_{13}) 
 +\,\Gamma^{(1)}_{gg}(z_1)\otimes{\cal D}_{3,g\to g}^{0}(s_{14}) 
 -\frac{1}{2}\,\,\Gamma^{(1)}_{gg}(z_1)\otimes\Gamma^{(1)}_{gg}(z_1) 
 \bigg] 
 B_1^{\gamma,0}(3,1,4,5,2)
 \nonumber\\
 \ph{3}&&+\bigg[ 
 -\frac{b_0}{\epsilon}\,\bigg( \frac{s_{13}}{\mu_R^2}\bigg)^{-\epsilon}\,{\cal D}_{3,g}^{0}(s_{13}) 
 +\,{\cal D}_{3,g\to g}^{0}(s_{13})\otimes{\cal D}_{3,g\to g}^{0}(s_{13}) 
 +\,{\cal D}_{3,q}^{0}(s_{13})\otimes{\cal D}_{3,g\to q}^{0}(s_{13}) 
 \nonumber \\ && \phantom{+\bigg[} 
 +\,\Gamma^{(1)}_{gg}(z_1)\otimes{\cal D}_{3,g\to q}^{0}(s_{13}) 
 -2\,\Gamma^{(1)}_{qq}(z_1)\otimes{\cal D}_{3,g\to q}^{0}(s_{13}) 
 +\frac{b_0}{\epsilon}\,{\cal D}_{3,g\to q}^{0}(s_{13}) 
 \nonumber \\ && \phantom{+\bigg[} 
 -\,{\cal D}_{4,g}^{0}(s_{13}) 
 -\frac{1}{2}\,\,{\cal D}_{4,g^\prime}^{0}(s_{13}) 
 -\,{\cal{D}}_{3,g}^{1}(s_{13}) 
 \nonumber \\ && \phantom{+\bigg[} 
 +\frac{1}{2}\,\,\Gamma^{(2)}_{gg}(z_1) 
 \bigg] 
 B_1^{\gamma,0}(3,1,4,5,2)
 \nonumber\\
 \ph{4}&&+\bigg[ 
 -\frac{b_0}{\epsilon}\,\bigg( \frac{s_{14}}{\mu_R^2}\bigg)^{-\epsilon}\,{\cal D}_{3,g}^{0}(s_{14}) 
 +\,\Gamma^{(1)}_{gg}(z_1)\otimes{\cal D}_{3,g\to q}^{0}(s_{14}) 
 -2\,\Gamma^{(1)}_{qq}(z_1)\otimes{\cal D}_{3,g\to q}^{0}(s_{14}) 
 \nonumber \\ && \phantom{+\bigg[} 
 +\,{\cal D}_{3,g\to g}^{0}(s_{14})\otimes{\cal D}_{3,g\to g}^{0}(s_{14}) 
 +\,{\cal D}_{3,q}^{0}(s_{14})\otimes{\cal D}_{3,g\to q}^{0}(s_{14}) 
 +\frac{b_0}{\epsilon}\,{\cal D}_{3,g\to q}^{0}(s_{14}) 
 \nonumber \\ && \phantom{+\bigg[} 
 +\frac{1}{2}\,\,\Gamma^{(2)}_{gg}(z_1) 
 -\,{\cal D}_{4,g}^{0}(s_{14}) 
 -\frac{1}{2}\,\,{\cal D}_{4,g^\prime}^{0}(s_{14}) 
 \nonumber \\ && \phantom{+\bigg[} 
 -\,{\cal{D}}_{3,g}^{1}(s_{14}) 
 \bigg] 
 B_1^{\gamma,0}(3,1,4,5,2)
 \nonumber\\
 \ph{5}&&+\bigg[ 
 +\frac{1}{2}\,\,\tilde{\cal A}_{4}^{0}(s_{34}) 
 +\,\tilde{\cal{A}}_{3}^{1}(s_{34}) 
 -\frac{1}{2}\,\,{\cal A}_{3}^{0}(s_{34})\otimes{\cal A}_{3}^{0}(s_{34}) 
 \bigg] 
 B_1^{\gamma,0}(3,1,4,5,2)
 \nonumber\\
 \ph{6}&&+\bigg[ 
 +\frac{b_0}{2\epsilon}\,\bigg( \frac{s_{13}}{\mu_R^2}\bigg)^{-\epsilon}\,{\cal A}_{3,g\to q}^{0}(s_{13}) 
 -\frac{1}{2}\,\,{\cal A}_{3,g\to q}^{0}(s_{13})\otimes\Gamma^{(1)}_{gg}(z_1) 
 +\,{\cal A}_{3,g\to q}^{0}(s_{13})\otimes\Gamma^{(1)}_{qq}(z_1) 
 \nonumber \\ && \phantom{+\bigg[} 
 -\,{\cal A}_{3,g\to q}^{0}(s_{13})\otimes{\cal A}_{3,q}^{0}(s_{13}) 
 -\frac{b_0}{2\epsilon}\,{\cal A}_{3,g\to q}^{0}(s_{13}) 
 +\,{\cal A}_{4,g}^{0}(s_{13}) 
 \nonumber \\ && \phantom{+\bigg[} 
 +\frac{1}{2}\,\,\tilde{\cal A}_{4,g}^{0}(s_{13}) 
 +\frac{1}{2}\,\,\tilde{\cal{A}}_{3,g}^{1}(s_{13}) 
 +\frac{1}{2}\,\,{\cal{A}}_{3,g}^{1}(s_{13}) 
 \bigg] 
 B_1^{\gamma,0}(3,1,4,5,2)
 \nonumber\\
 \ph{7}&&+\bigg[ 
 +\frac{b_0}{2\epsilon}\,\bigg( \frac{s_{14}}{\mu_R^2}\bigg)^{-\epsilon}\,{\cal A}_{3,g\to q}^{0}(s_{14}) 
 -\,{\cal A}_{3,g\to q}^{0}(s_{14})\otimes{\cal A}_{3,q}^{0}(s_{14}) 
 -\frac{1}{2}\,\,{\cal A}_{3,g\to q}^{0}(s_{14})\otimes\Gamma^{(1)}_{gg}(z_1) 
 \nonumber \\ && \phantom{+\bigg[} 
 +\,{\cal A}_{3,g\to q}^{0}(s_{14})\otimes\Gamma^{(1)}_{qq}(z_1) 
 -\frac{b_0}{2\epsilon}\,{\cal A}_{3,g\to q}^{0}(s_{14}) 
 +\,{\cal A}_{4,g}^{0}(s_{14}) 
 \nonumber \\ && \phantom{+\bigg[} 
 +\frac{1}{2}\,\,\tilde{\cal A}_{4,g}^{0}(s_{14}) 
 +\frac{1}{2}\,\,\tilde{\cal{A}}_{3,g}^{1}(s_{14}) 
 +\frac{1}{2}\,\,{\cal{A}}_{3,g}^{1}(s_{14}) 
 \bigg] 
 B_1^{\gamma,0}(3,1,4,5,2)
 \nonumber\\
\end{eqnarray}


==> sub/autogBh1g2AU.tex <==
\section*{gBh1g2AU}
\begin{eqnarray}
\lefteqn{{\tt gBh1g2AU(3,1,4,5,2) =}} \\
 \ph{1}&&+\bigg[ 
 -\,{\cal D}_{3,g}^{0}(s_{13}) 
 -\,{\cal D}_{3,g}^{0}(s_{14}) 
 +\frac{1}{2}\,\,{\cal A}_{3,g\to q}^{0}(s_{13}) 
 \nonumber \\ && \phantom{+\bigg[} 
 +\frac{1}{2}\,\,{\cal A}_{3,g\to q}^{0}(s_{14}) 
 +\,\Gamma^{(1)}_{gg}(z_1) 
 \bigg] 
\left( -\frac{b_F}{\epsilon}B_1^{\gamma,0}(3,1,4,5,2) +\hat{B}_1^{\gamma,1}(3,1,4,5,2)\right)
 \nonumber\\
 \ph{2}&&+\bigg[ 
 -\,\Gamma^{(1)}_{gg,F}(z_1) 
 \bigg] 
\left( +\frac{b_0}{\epsilon}B_1^{\gamma,0}(3,1,4,5,2) -B_1^{\gamma,1}(3,1,4,5,2)\right)
 \nonumber\\
 \ph{3}&&+\bigg[ 
 -\frac{b_F}{\epsilon}\,{\cal D}_{3,g}^{0}(s_{13})\,\bigg( \frac{s_{13}}{\mu_R^2}\bigg)^{-\epsilon} 
 +\frac{b_F}{2\epsilon}\,{\cal A}_{3,g\to q}^{0}(s_{13})\,\bigg( \frac{s_{13}}{\mu_R^2}\bigg)^{-\epsilon} 
 -S_{g\to q}\,\Gamma^{(1)}_{qg}(z_1)\otimes{\cal E}_{3,q^\prime \to g}^{0}(s_{13}) 
 \nonumber \\ && \phantom{+\bigg[} 
 +\,\Gamma^{(1)}_{gg,F}(z_1)\otimes{\cal D}_{3,g}^{0}(s_{13}) 
 -\frac{1}{2}\,\,{\cal A}_{3,g\to q}^{0}(s_{13})\otimes\Gamma^{(1)}_{gg,F}(z_1) 
 +\frac{1}{2}\,\,{\cal A}_{3,g\to q}^{0}(s_{13})\otimes{\cal E}_{3,q}^{0}(s_{14}) 
 \nonumber \\ && \phantom{+\bigg[} 
 -\frac{1}{2}\,\,\Gamma^{(1)}_{gg}(z_1)\otimes\Gamma^{(1)}_{gg,F}(z_1) 
 -\frac{1}{2}\,\,\Gamma^{(1)}_{qg}(z_1)\otimes\Gamma^{(1)}_{gq}(z_1) 
 -\,{\cal E}_{4,g}^{0}(s_{13}) 
 \nonumber \\ && \phantom{+\bigg[} 
 -\,\hat{\cal{D}}_{3,g}^{1}(s_{13}) 
 +\frac{1}{2}\,\,\hat{\cal{A}}_{3,g}^{1}(s_{13}) 
 +\frac{1}{2}\,\,\Gamma^{(2)}_{gg,F}(z_1) 
 \bigg] 
 B_1^{\gamma,0}(3,1,4,5,2)
 \nonumber\\
 \ph{4}&&+\bigg[ 
 -S_{g\to q}\,\Gamma^{(1)}_{qg}(z_1)\otimes{\cal E}_{3,q^\prime \to g}^{0}(s_{14}) 
 -\frac{b_F}{\epsilon}\,\bigg( \frac{s_{14}}{\mu_R^2}\bigg)^{-\epsilon}\,{\cal D}_{3,g}^{0}(s_{14}) 
 +\frac{b_F}{2\epsilon}\,\bigg( \frac{s_{14}}{\mu_R^2}\bigg)^{-\epsilon}\,{\cal A}_{3,g\to q}^{0}(s_{14}) 
 \nonumber \\ && \phantom{+\bigg[} 
 -\frac{1}{2}\,\,\Gamma^{(1)}_{qg}(z_1)\otimes\Gamma^{(1)}_{gq}(z_1) 
 -\frac{1}{2}\,\,\Gamma^{(1)}_{gg}(z_1)\otimes\Gamma^{(1)}_{gg,F}(z_1) 
 +\,\Gamma^{(1)}_{gg,F}(z_1)\otimes{\cal D}_{3,g}^{0}(s_{14}) 
 \nonumber \\ && \phantom{+\bigg[} 
 -\frac{1}{2}\,\,{\cal A}_{3,g\to q}^{0}(s_{14})\otimes\Gamma^{(1)}_{gg,F}(z_1) 
 +\frac{1}{2}\,\,{\cal A}_{3,g\to q}^{0}(s_{13})\otimes{\cal E}_{3,q}^{0}(s_{14}) 
 +\frac{1}{2}\,\,\Gamma^{(2)}_{gg,F}(z_1) 
 \nonumber \\ && \phantom{+\bigg[} 
 -\,{\cal E}_{4,g}^{0}(s_{14}) 
 -\,\hat{\cal{D}}_{3,g}^{1}(s_{14}) 
 +\frac{1}{2}\,\,\hat{\cal{A}}_{3,g}^{1}(s_{14}) 
 \bigg] 
 B_1^{\gamma,0}(3,1,4,5,2)
 \nonumber\\
\end{eqnarray}


==> sub/autogBhh1g2AU.tex <==
\section*{gBhh1g2AU}
\begin{eqnarray}
\lefteqn{{\tt gBhh1g2AU(3,1,4,5,2) =}} \\
 \ph{1}&&+\bigg[ 
 +\,\Gamma^{(1)}_{gg,F}(z_1) 
 \bigg] 
\left( -\frac{b_F}{\epsilon}B_1^{\gamma,0}(3,1,4,5,2) +\hat{B}_1^{\gamma,1}(3,1,4,5,2)\right)
 \nonumber\\
 \ph{2}&&+\bigg[ 
 -\frac{1}{2}\,\,\Gamma^{(1)}_{gg,F}(z_1)\otimes\Gamma^{(1)}_{gg,F}(z_1) 
 +\,\Gamma^{(2)}_{gg,F^2}(z_1) 
 \bigg] 
 B_1^{\gamma,0}(3,1,4,5,2)
 \nonumber\\
\end{eqnarray}


==> sub/autogBt1g2AU.tex <==
\section*{gBt1g2AU}
\begin{eqnarray}
\lefteqn{{\tt gBt1g2AU(3,1,4,5,2) =}} \\
 \ph{1}&&+\bigg[ 
 +\,{\cal A}_{3}^{0}(s_{34}) 
 \bigg] 
\left( +\frac{b_0}{\epsilon}B_1^{\gamma,0}(3,1,4,5,2) -B_1^{\gamma,1}(3,1,4,5,2)\right)
 \nonumber\\
 \ph{2}&&+\bigg[ 
 +\,\Gamma^{(1)}_{gg}(z_1) 
 -\,{\cal D}_{3,g\to g}^{0}(s_{13}) 
 -\,{\cal D}_{3,g\to g}^{0}(s_{14}) 
 \bigg] 
 \tilde{B}_3^{\gamma,1}(3,1,4,5,2)
 \nonumber\\
 \ph{3}&&+\bigg[ 
 -\,{\cal D}_{3,g\to g}^{0}(s_{13})\otimes{\cal A}_{3}^{0}(s_{34}) 
 -\,{\cal D}_{3,g\to g}^{0}(s_{14})\otimes{\cal A}_{3}^{0}(s_{34}) 
 +\,\Gamma^{(1)}_{gg}(z_1)\otimes{\cal A}_{3}^{0}(s_{34}) 
 \bigg] 
 B_1^{\gamma,0}(3,1,4,5,2)
 \nonumber\\
 \ph{4}&&+\bigg[ 
 -\frac{b_0}{\epsilon}\,\bigg( \frac{s_{34}}{\mu_R^2}\bigg)^{-\epsilon}\,{\cal A}_{3}^{0}(s_{34}) 
 +\,{\cal A}_{3}^{0}(s_{34})\otimes{\cal A}_{3}^{0}(s_{34}) 
 -\,{\cal A}_{4}^{0}(s_{34}) 
 \nonumber \\ && \phantom{+\bigg[} 
 -\,{\cal{A}}_{3}^{1}(s_{34}) 
 \bigg] 
 B_1^{\gamma,0}(3,1,4,5,2)
 \nonumber\\
 \ph{5}&&+\bigg[ 
 -\frac{1}{2}\,\,\tilde{\cal A}_{4}^{0}(s_{34}) 
 -\,\tilde{\cal{A}}_{3}^{1}(s_{34}) 
 -2\,{\cal C}_{4}^{0}(s_{34}) 
 \bigg] 
 B_1^{\gamma,0}(3,1,4,5,2)
 \nonumber\\
\end{eqnarray}


==> sub/autogBth1g2AU.tex <==
\section*{gBth1g2AU}
\begin{eqnarray}
\lefteqn{{\tt gBth1g2AU(3,1,4,5,2) =}} \\
 \ph{1}&&+\bigg[ 
 -\,{\cal A}_{3}^{0}(s_{34}) 
 \bigg] 
\left( +\frac{b_F}{\epsilon}B_1^{\gamma,0}(3,1,4,5,2) -\hat{B}_1^{\gamma,1}(3,1,4,5,2)\right)
 \nonumber\\
 \ph{2}&&+\bigg[ 
 -\,\Gamma^{(1)}_{gg,F}(z_1) 
 \bigg] 
 \tilde{B}_3^{\gamma,1}(3,1,4,5,2)
 \nonumber\\
 \ph{3}&&+\bigg[ 
 +\frac{b_F}{\epsilon}\,\bigg( \frac{s_{34}}{\mu_R^2}\bigg)^{-\epsilon}\,{\cal A}_{3}^{0}(s_{34}) 
 -\,\Gamma^{(1)}_{gg,F}(z_1)\otimes{\cal A}_{3}^{0}(s_{34}) 
 +\,{\cal B}_{4}^{0}(s_{34}) 
 \nonumber \\ && \phantom{+\bigg[} 
 +\,\hat{\cal{A}}_{3}^{1}(s_{34}) 
 +\,\widetilde{\Gamma}^{(2)}_{gg,F}(z_1) 
 \bigg] 
 B_1^{\gamma,0}(3,1,4,5,2)
 \nonumber\\
 \ph{4}&&+\bigg[ 
 +\frac{1}{2}\,\,\tilde{\cal E}_{4,g}^{0}(s_{13}) 
 +S_{g\to q}\,\Gamma^{(1)}_{qg}(z_1)\otimes{\cal E}_{3,q^\prime \to g}^{0}(s_{13}) 
 +\frac{1}{2}\,\,\Gamma^{(1)}_{qg}(z_1)\otimes\Gamma^{(1)}_{gq}(z_1) 
 \bigg] 
 B_1^{\gamma,0}(3,1,4,5,2)
 \nonumber\\
 \ph{5}&&+\bigg[ 
 +\frac{1}{2}\,\,\tilde{\cal E}_{4,g}^{0}(s_{14}) 
 +S_{g\to q}\,\Gamma^{(1)}_{qg}(z_1)\otimes{\cal E}_{3,q^\prime \to g}^{0}(s_{14}) 
 +\frac{1}{2}\,\,\Gamma^{(1)}_{qg}(z_1)\otimes\Gamma^{(1)}_{gq}(z_1) 
 \bigg] 
 B_1^{\gamma,0}(3,1,4,5,2)
 \nonumber\\
\end{eqnarray}


==> sub/autogBtt1g2AU.tex <==
\section*{gBtt1g2AU}
\begin{eqnarray}
\lefteqn{{\tt gBtt1g2AU(3,1,4,5,2) =}} \\
 \ph{1}&&+\bigg[ 
 -\,{\cal A}_{3}^{0}(s_{34}) 
 \bigg] 
 \tilde{B}_3^{\gamma,1}(3,1,4,5,2)
 \nonumber\\
 \ph{2}&&+\bigg[ 
 -\frac{1}{2}\,\,\tilde{\cal A}_{4}^{0}(s_{34}) 
 -\,\tilde{\cal{A}}_{3}^{1}(s_{34}) 
 -2\,{\cal C}_{4}^{0}(s_{34}) 
 \bigg] 
 B_1^{\gamma,0}(3,1,4,5,2)
 \nonumber\\
\end{eqnarray}


==> sub/autogD0g1AT.tex <==
\section*{gD0g1AT(1,j,k,i,6,2)}
\begin{eqnarray}
  \ph{1}&&-2J_{2,QQ,g \to q}^{1,IF}(s_{1k})\,D_0^{\gamma,0}(1,j,k,i,6,2)\,J_2^{(3)}(\lbrace p\rbrace_{3})\nonumber\\
  \ph{2}&&-2J_{2,QQ,g \to q}^{1,IF}(s_{1k})\,D_0^{\gamma,0}(i,1,j,k,6,2)\,J_2^{(3)}(\lbrace p\rbrace_{3})\nonumber\\
\end{eqnarray}


==> sub/autogDt0g1AT.tex <==
\section*{gDt0g1AT(1,j,k,i,6,2)}
\begin{eqnarray}
  \ph{1}&&-2J_{2,QQ,g \to q}^{1,IF}(s_{1k})\,D_0^{\gamma,0}(1,j,k,i,6,2)\,J_2^{(3)}(\lbrace p\rbrace_{3})\nonumber\\
  \ph{2}&&-2J_{2,QQ,g \to q}^{1,IF}(s_{1j})\,D_0^{\gamma,0}(i,1,k,j,6,2)\,J_2^{(3)}(\lbrace p\rbrace_{3})\nonumber\\
\end{eqnarray}


==> sub/autogtoqB1g2AU.tex <==
\section*{gtoqB1g2AU}
\begin{eqnarray}
\lefteqn{{\tt gtoqB1g2AU(3,1,4,5,2) =}} \\
 \ph{1}&&+\bigg[ 
 +\,{\cal A}_{3,g\to q}^{0}(s_{14}) 
 +2S_{g\to q}\,\Gamma^{(1)}_{qg}(z_1) 
 \bigg] 
\left( -\frac{b_0}{\epsilon}{sB}_1^{\gamma,0}(1,3,4,5,2) +sB1g1A(1,3,4,5,2)\right)
 \nonumber\\
 \ph{2}&&+\bigg[ 
 +\frac{1}{2}\,\,{\cal A}_{3,g\to q}^{0}(s_{14})\otimes{\cal D}_{3}^{0}(s_{34}) 
 +\frac{1}{2}\,\,{\cal A}_{3,g\to q}^{0}(s_{14})\otimes{\cal D}_{3,q}^{0}(s_{13}) 
 +S_{g\to q}\,\Gamma^{(1)}_{qg}(z_1)\otimes{\cal D}_{3,q}^{0}(s_{13}) 
 \nonumber \\ && \phantom{+\bigg[} 
 +S_{g\to q}\,\Gamma^{(1)}_{qg}(z_1)\otimes{\cal D}_{3}^{0}(s_{34}) 
 -\,\Gamma^{(1)}_{qq}(z_1)\otimes{\cal A}_{3,g\to q}^{0}(s_{14}) 
 -2S_{g\to q}\,\Gamma^{(1)}_{qg}(z_1)\otimes\Gamma^{(1)}_{qq}(z_1) 
 \bigg] 
 {sB}_1^{\gamma,0}(1,3,4,5,2)
 \nonumber\\
 \ph{3}&&+\bigg[ 
 +\frac{b_0}{\epsilon}\,\bigg( \frac{s_{14}}{\mu_R^2}\bigg)^{-\epsilon}\,{\cal A}_{3,g\to q}^{0}(s_{14}) 
 +S_{g\to q}\,\Gamma^{(1)}_{qg}(z_1)\otimes\Gamma^{(1)}_{qq}(z_1) 
 -S_{g\to q}\,\Gamma^{(1)}_{qg}(z_1)\otimes\Gamma^{(1)}_{gg}(z_1) 
 \nonumber \\ && \phantom{+\bigg[} 
 -\,{\cal A}_{3,g\to q}^{0}(s_{14})\otimes{\cal A}_{3,q}^{0}(s_{14}) 
 +\,\Gamma^{(1)}_{qq}(z_1)\otimes{\cal A}_{3,g\to q}^{0}(s_{14}) 
 -\,\Gamma^{(1)}_{gg}(z_1)\otimes{\cal A}_{3,g\to q}^{0}(s_{14}) 
 \nonumber \\ && \phantom{+\bigg[} 
 +2S_{g\to q}\,\Gamma^{(2)}_{qg}(z_1) 
 +2\,{\cal A}_{4,g}^{0}(s_{14}) 
 +\,{\cal{A}}_{3,g}^{1}(s_{14}) 
 \bigg] 
 {sB}_1^{\gamma,0}(1,3,4,5,2)
 \nonumber\\
\end{eqnarray}


==> sub/autogtoqBh1g2AU.tex <==
\section*{gtoqBh1g2AU}
\begin{eqnarray}
\lefteqn{{\tt gtoqBh1g2AU(3,1,4,5,2) =}} \\
 \ph{1}&&+\bigg[ 
 +\,{\cal A}_{3,g\to q}^{0}(s_{14}) 
 +2S_{g\to q}\,\Gamma^{(1)}_{qg}(z_1) 
 \bigg] 
\left( -\frac{b_F}{\epsilon}{sB}_1^{\gamma,0}(1,3,4,5,2) +sBh1g1A(1,3,4,5,2)\right)
 \nonumber\\
 \ph{2}&&+\bigg[ 
 +\frac{1}{2}\,\,{\cal E}_{3}^{0}(s_{34})\otimes{\cal A}_{3,g\to q}^{0}(s_{14}) 
 +\frac{1}{2}\,\,{\cal E}_{3,q}^{0}(s_{13})\otimes{\cal A}_{3,g\to q}^{0}(s_{14}) 
 +S_{g\to q}\,{\cal E}_{3}^{0}(s_{34})\otimes\Gamma^{(1)}_{qg}(z_1) 
 \nonumber \\ && \phantom{+\bigg[} 
 +S_{g\to q}\,{\cal E}_{3,q}^{0}(s_{13})\otimes\Gamma^{(1)}_{qg}(z_1) 
 \bigg] 
 {sB}_1^{\gamma,0}(1,3,4,5,2)
 \nonumber\\
 \ph{3}&&+\bigg[ 
 +\frac{b_F}{\epsilon}\,\bigg( \frac{s_{14}}{\mu_R^2}\bigg)^{-\epsilon}\,{\cal A}_{3,g\to q}^{0}(s_{14}) 
 -S_{g\to q}\,\Gamma^{(1)}_{gg,F}(z_1)\otimes\Gamma^{(1)}_{qg}(z_1) 
 -\,{\cal A}_{3,g\to q}^{0}(s_{14})\otimes\Gamma^{(1)}_{gg,F}(z_1) 
 \nonumber \\ && \phantom{+\bigg[} 
 +2S_{g\to q}\,\Gamma^{(2)}_{qg,F}(z_1) 
 +\,\hat{\cal{A}}_{3,g}^{1}(s_{14}) 
 \bigg] 
 {sB}_1^{\gamma,0}(1,3,4,5,2)
 \nonumber\\
\end{eqnarray}


==> sub/autogtoqBt1g2AU.tex <==
\section*{gtoqBt1g2AU}
\begin{eqnarray}
\lefteqn{{\tt gtoqBt1g2AU(3,1,4,5,2) =}} \\
 \ph{1}&&+\bigg[ 
 -\,{\cal A}_{3,g\to q}^{0}(s_{14}) 
 -2S_{g\to q}\,\Gamma^{(1)}_{qg}(z_1) 
 \bigg] 
\left( +\frac{b_0}{\epsilon}{sB}_1^{\gamma,0}(1,3,4,5,2) -sB1g1A(1,3,4,5,2)\right)
 \nonumber\\
 \ph{2}&&+\bigg[ 
 +\frac{1}{2}\,\,{\cal A}_{3,g\to q}^{0}(s_{14})\otimes{\cal D}_{3}^{0}(s_{34}) 
 +\frac{1}{2}\,\,{\cal A}_{3,g\to q}^{0}(s_{14})\otimes{\cal D}_{3,q}^{0}(s_{13}) 
 +S_{g\to q}\,\Gamma^{(1)}_{qg}(z_1)\otimes{\cal D}_{3,q}^{0}(s_{13}) 
 \nonumber \\ && \phantom{+\bigg[} 
 +S_{g\to q}\,\Gamma^{(1)}_{qg}(z_1)\otimes{\cal D}_{3}^{0}(s_{34}) 
 -\,\Gamma^{(1)}_{qq}(z_1)\otimes{\cal A}_{3,g\to q}^{0}(s_{14}) 
 -2S_{g\to q}\,\Gamma^{(1)}_{qg}(z_1)\otimes\Gamma^{(1)}_{qq}(z_1) 
 \bigg] 
 {sB}_1^{\gamma,0}(1,3,4,5,2)
 \nonumber\\
 \ph{3}&&+\bigg[ 
 +\frac{b_0}{\epsilon}\,\bigg( \frac{s_{14}}{\mu_R^2}\bigg)^{-\epsilon}\,{\cal A}_{3,g\to q}^{0}(s_{14}) 
 +S_{g\to q}\,\Gamma^{(1)}_{qg}(z_1)\otimes\Gamma^{(1)}_{qq}(z_1) 
 -S_{g\to q}\,\Gamma^{(1)}_{qg}(z_1)\otimes\Gamma^{(1)}_{gg}(z_1) 
 \nonumber \\ && \phantom{+\bigg[} 
 +\,\Gamma^{(1)}_{qq}(z_1)\otimes{\cal A}_{3,g\to q}^{0}(s_{14}) 
 -\,{\cal A}_{3,g\to q}^{0}(s_{14})\otimes{\cal A}_{3,q}^{0}(s_{14}) 
 -\,\Gamma^{(1)}_{gg}(z_1)\otimes{\cal A}_{3,g\to q}^{0}(s_{14}) 
 \nonumber \\ && \phantom{+\bigg[} 
 +2S_{g\to q}\,\Gamma^{(2)}_{qg}(z_1) 
 +2\,{\cal A}_{4,g}^{0}(s_{14}) 
 +\,{\cal{A}}_{3,g}^{1}(s_{14}) 
 \bigg] 
 {sB}_1^{\gamma,0}(1,3,4,5,2)
 \nonumber\\
 \ph{4}&&+\bigg[ 
 +\,{\cal A}_{3,g\to q}^{0}(s_{14}) 
 +2S_{g\to q}\,\Gamma^{(1)}_{qg}(z_1) 
 \bigg] 
 sBt1g1A(1,3,4,5,2)
 \nonumber\\
 \ph{5}&&+\bigg[ 
 +\,{\cal A}_{3,g\to q}^{0}(s_{14})\otimes{\cal A}_{3,q}^{0}(s_{14}) 
 +2S_{g\to q}\,\Gamma^{(1)}_{qg}(z_1)\otimes{\cal A}_{3,q}^{0}(s_{14}) 
 -\,\Gamma^{(1)}_{qq}(z_1)\otimes{\cal A}_{3,g\to q}^{0}(s_{14}) 
 \nonumber \\ && \phantom{+\bigg[} 
 -2S_{g\to q}\,\Gamma^{(1)}_{qg}(z_1)\otimes\Gamma^{(1)}_{qq}(z_1) 
 \bigg] 
 {sB}_1^{\gamma,0}(1,3,4,5,2)
 \nonumber\\
 \ph{6}&&+\bigg[ 
 +\,\tilde{\cal A}_{4,g}^{0}(s_{14}) 
 +\,\tilde{\cal{A}}_{3,g}^{1}(s_{14}) 
 -\,{\cal A}_{3,g\to q}^{0}(s_{14})\otimes{\cal A}_{3,q}^{0}(s_{14}) 
 \nonumber \\ && \phantom{+\bigg[} 
 +\,\Gamma^{(1)}_{qq}(z_1)\otimes{\cal A}_{3,g\to q}^{0}(s_{14}) 
 +S_{g\to q}\,\Gamma^{(1)}_{qg}(z_1)\otimes\Gamma^{(1)}_{qq}(z_1) 
 -2S_{g\to q}\,\widetilde{\Gamma}^{(2)}_{qg}(z_1) 
 \bigg] 
 {sB}_1^{\gamma,0}(1,3,4,5,2)
 \nonumber\\
\end{eqnarray}


==> sub/autogtoqBth1g2AU.tex <==
\section*{gBth1g2AUgtoq}
\begin{eqnarray}
\lefteqn{{\tt gBth1g2AUgtoq(3,1,4,5,2) =}} \\
 \ph{1}&&+\bigg[ 
 -\,{\cal A}_{3,g\to q}^{0}(s_{14}) 
 -2S_{g\to q}\,\Gamma^{(1)}_{qg}(z_1) 
 \bigg] 
\left( -\frac{b_F}{\epsilon}{sB}_1^{\gamma,0}(1,3,4,5,2) +sBh1g1A(1,3,4,5,2)\right)
 \nonumber\\
 \ph{2}&&+\bigg[ 
 -\frac{b_F}{\epsilon}\,\bigg( \frac{s_{14}}{\mu_R^2}\bigg)^{-\epsilon}\,{\cal A}_{3,g\to q}^{0}(s_{14}) 
 +S_{g\to q}\,\Gamma^{(1)}_{gg,F}(z_1)\otimes\Gamma^{(1)}_{qg}(z_1) 
 -S_{g\to q}\,{\cal E}_{3,q}^{0}(s_{13})\otimes\Gamma^{(1)}_{qg}(z_1) 
 \nonumber \\ && \phantom{+\bigg[} 
 -S_{g\to q}\,{\cal E}_{3}^{0}(s_{34})\otimes\Gamma^{(1)}_{qg}(z_1) 
 +\,{\cal A}_{3,g\to q}^{0}(s_{14})\otimes\Gamma^{(1)}_{gg,F}(z_1) 
 -\frac{1}{2}\,\,{\cal E}_{3,q}^{0}(s_{13})\otimes{\cal A}_{3,g\to q}^{0}(s_{14}) 
 \nonumber \\ && \phantom{+\bigg[} 
 -\frac{1}{2}\,\,{\cal E}_{3}^{0}(s_{34})\otimes{\cal A}_{3,g\to q}^{0}(s_{14}) 
 -2S_{g\to q}\,\Gamma^{(2)}_{qg,F}(z_1) 
 -\,\hat{\cal{A}}_{3,g}^{1}(s_{14}) 
 \bigg] 
 {sB}_1^{\gamma,0}(1,3,4,5,2)
 \nonumber\\
\end{eqnarray}


==> sub/autogtoqBtt1g2AU.tex <==
\section*{gtoqBtt1g2AU}
\begin{eqnarray}
\lefteqn{{\tt gtoqBtt1g2AU(3,1,4,5,2) =}} \\
 \ph{1}&&+\bigg[ 
 +\,{\cal A}_{3,g\to q}^{0}(s_{14}) 
 +2S_{g\to q}\,\Gamma^{(1)}_{qg}(z_1) 
 \bigg] 
 sBt1g1A(1,3,4,5,2)
 \nonumber\\
 \ph{2}&&+\bigg[ 
 +\,{\cal A}_{3,g\to q}^{0}(s_{14})\otimes{\cal A}_{3,q}^{0}(s_{14}) 
 +2S_{g\to q}\,\Gamma^{(1)}_{qg}(z_1)\otimes{\cal A}_{3,q}^{0}(s_{14}) 
 -\,\Gamma^{(1)}_{qq}(z_1)\otimes{\cal A}_{3,g\to q}^{0}(s_{14}) 
 \nonumber \\ && \phantom{+\bigg[} 
 -2S_{g\to q}\,\Gamma^{(1)}_{qg}(z_1)\otimes\Gamma^{(1)}_{qq}(z_1) 
 \bigg] 
 {sB}_1^{\gamma,0}(1,3,4,5,2)
 \nonumber\\
 \ph{3}&&+\bigg[ 
 +\,\tilde{\cal A}_{4,g}^{0}(s_{14}) 
 +\,\tilde{\cal{A}}_{3,g}^{1}(s_{14}) 
 -\,{\cal A}_{3,g\to q}^{0}(s_{14})\otimes{\cal A}_{3,q}^{0}(s_{14}) 
 \nonumber \\ && \phantom{+\bigg[} 
 +\,\Gamma^{(1)}_{qq}(z_1)\otimes{\cal A}_{3,g\to q}^{0}(s_{14}) 
 +S_{g\to q}\,\Gamma^{(1)}_{qg}(z_1)\otimes\Gamma^{(1)}_{qq}(z_1) 
 -2S_{g\to q}\,\widetilde{\Gamma}^{(2)}_{qg}(z_1) 
 \bigg] 
 {sB}_1^{\gamma,0}(1,3,4,5,2)
 \nonumber\\
\end{eqnarray}


==> sub/autoq1Bhh2g1AT.tex <==
\section*{q1C0g1NFAT(1,j,k,i,6,2)}
\begin{eqnarray}
  \ph{1}&&+\frac{1}{2}\,\,E_3^{0}(i,j,k)\,\hat{B}_1^{\gamma,1}(1,(\widetilde{jk}),(\widetilde{ij}),6,2)\,\delta(1-x_1)\,\delta(1-x_2)\nonumber\\
  \ph{2}&&+\frac{1}{2}\,\,E_{3,q}^{0}(1,j,k)\,\hat{B}_1^{\gamma,1}(\overline{1},(\widetilde{jk}),i,6,2)\,\delta(1-x_1)\,\delta(1-x_2)\nonumber\\
  \ph{3}&&+\frac{1}{2}\,\,\hat{E}_{3}^{1}(i,j,k)\,B_1^{\gamma,0}(1,(\widetilde{jk}),(\widetilde{ij}),6,2)\,\delta(1-x_1)\,\delta(1-x_2)\nonumber\\
  \ph{4}&&+\frac{1}{2}\,\,\hat{E}_{3,q}^{1}(1,j,k)\,B_1^{\gamma,0}(\overline{1},(\widetilde{jk}),i,6,2)\,\delta(1-x_1)\,\delta(1-x_2)\nonumber\\
\end{eqnarray}


==> sub/autoq1C0g0AS.tex <==
\section*{q1C0g0AS(1,i,j,k,6,2)}
\begin{eqnarray}
 \ph{1}&&+E_3^{0}(k,i,j)\,B_1^{\gamma,0}(1,(\widetilde{ji}),(\widetilde{ki}),6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\end{eqnarray}


==> sub/autoq1C0g1AT.tex <==
\section*{q1C0g1AT(1,j,k,i,6,2)}
\begin{eqnarray}
 \ph{1}&&-\bigg[ 
 +\frac{1}{2}\,J_{2,QQ}^{1,IF}(s_{1j})
 +\frac{1}{2}\,J_{2,QQ}^{1,FF}(s_{ik})\bigg]\,C_0^{\gamma,0}(1,j,k,i,6,2)\,J_2^{(3)}(\lbrace p\rbrace_{3})\nonumber\\
 \ph{2}&&-\bigg[ 
 +\frac{1}{2}\,J_{2,QQ}^{1,IF}(s_{1k})
 +\frac{1}{2}\,J_{2,QQ}^{1,FF}(s_{ij})\bigg]\,C_0^{\gamma,0}(1,k,j,i,6,2)\,J_2^{(3)}(\lbrace p\rbrace_{3})\nonumber\\
  \ph{3}&&+\frac{1}{2}\,\,E_3^{0}(i,j,k)\,\bigg[\,B_1^{\gamma,1}((\widetilde{ij}),(\widetilde{jk}),1,6,2)\,\delta(1-x_1)\,\delta(1-x_2)\nonumber\\
  &&+\,\bigg( 
 +J_{2,QG}^{1,FF}(s_{(\widetilde{ij})(\widetilde{jk})})
 +J_{2,QG}^{1,IF}(s_{1(\widetilde{jk})})\bigg)\,B_1^{\gamma,0}(1,(\widetilde{jk}),(\widetilde{ij}),6,2) \bigg]\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
  \ph{4}&&+\frac{1}{2}\,\,E_{3,q}^{0}(1,j,k)\,\bigg[\,B_1^{\gamma,1}(\overline{1},(\widetilde{jk}),i,6,2)\,\delta(1-x_1)\,\delta(1-x_2)\nonumber\\
  &&+\,\bigg( 
 +J_{2,QG}^{1,FF}(s_{i(\widetilde{jk})})
 +J_{2,QG}^{1,IF}(s_{\overline{1}(\widetilde{jk})})\bigg)\,B_1^{\gamma,0}(\overline{1},(\widetilde{jk}),i,6,2) \bigg]\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
  \ph{5}&&+\frac{1}{2}\,\bigg[\,E_{3}^{1}(i,j,k)\,\delta(1-x_1)\,\delta(1-x_2)
  \nonumber\\&&\,  
   +\bigg( 
 +J_{2,QQ}^{1,FF}(s_{ij})
 +J_{2,QQ}^{1,FF}(s_{ik})
 -2J_{2,QG}^{1,FF}(s_{(\widetilde{ij})(\widetilde{jk})})\bigg)\,E_3^{0}(i,j,k)\bigg]\,B_1^{\gamma,0}(1,(\widetilde{jk}),(\widetilde{ij}),6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
  \ph{6}&&+\frac{1}{2}\,\bigg[\,E_{3}^{1}(1,j,k)\,\delta(1-x_1)\,\delta(1-x_2)
  \nonumber\\&&\,  
   +\bigg( 
 +J_{2,QQ}^{1,IF}(s_{1j})
 +J_{2,QQ}^{1,IF}(s_{1k})
 -2J_{2,QG}^{1,IF}(s_{\overline{1}(\widetilde{jk})})\bigg)\,E_3^{0}(1,j,k)\bigg]\,B_1^{\gamma,0}(\overline{1},(\widetilde{jk}),i,6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
\end{eqnarray}


==> sub/autoq1C1g0AS.tex <==
\section*{q1C1g0AS(1,i,j,k,l,7,2)}
\begin{eqnarray}
 \ph{1}&&+A_3^{0}(1,i,j)\,C_0^{\gamma,0}(\overline{1},(\widetilde{ji}),k,l,7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{2}&&+A_3^{0}(k,i,l)\,C_0^{\gamma,0}(1,j,(\widetilde{ki}),(\widetilde{li}),7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{3}&&+E_3^{0}(l,j,k)\,f1B2g0A(1,(\widetilde{jk}),i,(\widetilde{lj}),7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{4}&&+E_3^{0}(l,j,k)\,f1B2g0A(1,i,(\widetilde{jk}),(\widetilde{lj}),7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
\snip \ph{5}&&+\,E_4^{0,a}(l,j,k,i)\,f1B1g0A(1,(\widetilde{ikj}),(\widetilde{ljk}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\snip \ph{6}&&+\,E_4^{0,b}(l,i,k,j)\,f1B1g0A(1,(\widetilde{jki}),(\widetilde{lik}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{7}&&-\,E_3^{0}(l,j,k)\,d_3^{0}((\widetilde{lj}),i,(\widetilde{jk}))\,f1B1g0A(1,(\widetilde{(\widetilde{jk})i}),(\widetilde{(\widetilde{lj})i}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{8}&&-\,E_3^{0}(l,j,k)\,d_3^{0}((\widetilde{lj}),(\widetilde{jk}),i)\,f1B1g0A(1,(\widetilde{i\widetilde{(kj})}),[(\widetilde{lj}), (\widetilde{jk})],7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{9}&&-\,A_3^{0}(k,i,l)\,E_3^{0}((\widetilde{li}),(\widetilde{ki}),j)\,f1B1g0A(1,(\widetilde{j\widetilde{(ki})}),[(\widetilde{ki}), (\widetilde{li})],7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\snip \ph{10}&&+\,E_4^0(1,k,j,i)\,f1B1g0A(\overline{1},(\widetilde{ijk}),l,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{11}&&-\,E_3^{0}(l,j,k)\,D_3^{0}(1,(\widetilde{kj}),i)\,f1B1g0A(\overline{1},(\widetilde{i\widetilde{(kj})}),(\widetilde{lj}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{12}&&-\,A_3^{0}(1,i,j)\,E_3^{0}(\overline{1},k,(\widetilde{ji}))\,f1B1g0A(\overline{\overline{1}},(\widetilde{k\widetilde{(ji})}),l,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\end{eqnarray}


==> sub/autoq1Ct0g1AT.tex <==
\section*{q1Ct0g1AT(1,j,k,i,6,2)}
\begin{eqnarray}
 \ph{1}&&-\bigg[ 
 +J_{2,QQ}^{1,FF}(s_{jk})
 +2J_{2,QQ}^{1,FF}(s_{ki})
 +J_{2,QQ}^{1,IF}(s_{1i})
 -2J_{2,QQ}^{1,IF}(s_{1k})
 -2J_{2,QQ}^{1,FF}(s_{ij})
 +2J_{2,QQ}^{1,IF}(s_{1j})\bigg]\,C_0^{\gamma,0}(1,j,k,i,6,2)\,J_2^{(3)}(\lbrace p\rbrace_{3})\nonumber\\
  \ph{2}&&+\frac{1}{2}\,\bigg[\,\tilde{E}_{3}^{1}(i,j,k)\,\delta(1-x_1)\,\delta(1-x_2)
 +J_{2,QQ}^{1,FF}(s_{jk})\,E_3^{0}(i,j,k)\bigg]\,B_1^{\gamma,0}(1,(\widetilde{jk}),(\widetilde{ij}),6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
  \ph{3}&&+\frac{1}{2}\,\bigg[\,\tilde{E}_{3,q}^{1}(1,j,k)\,\delta(1-x_1)\,\delta(1-x_2)
 +J_{2,QQ}^{1,FF}(s_{jk})\,E_{3,q}^{0}(1,j,k)\bigg]\,B_1^{\gamma,0}(\overline{1},(\widetilde{jk}),i,6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
  \ph{4}&&+\frac{1}{2}\,\,E_3^{0}(i,j,k)\,\bigg[\,\tilde{B}_3^{\gamma,1}(1,(\widetilde{jk}),(\widetilde{ij}),6,2)\,\delta(1-x_1)\,\delta(1-x_2)\nonumber\\
 &&\phantom{\bigg[}+J_{2,QQ}^{1,IF}(s_{1(\widetilde{ij})})\,B_1^{\gamma,0}(1,(\widetilde{jk}),(\widetilde{ij}),6,2) \bigg]\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
  \ph{5}&&+\frac{1}{2}\,\,E_{3,q}^{0}(1,j,k)\,\bigg[\,\tilde{B}_3^{\gamma,1}(\overline{1},(\widetilde{jk}),i,6,2)\,\delta(1-x_1)\,\delta(1-x_2)\nonumber\\
 &&\phantom{\bigg[}+J_{2,QQ}^{1,IF}(s_{\overline{1}i})\,B_1^{\gamma,0}(\overline{1},(\widetilde{jk}),i,6,2) \bigg]\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
 \ph{6}&&+2\bigg[ +J_{2,QQ}^{1,FF}(s_{ki})
 -J_{2,QQ}^{1,IF}(s_{1k})
 -J_{2,QQ}^{1,FF}(s_{ij})
 +J_{2,QQ}^{1,IF}(s_{1j})
 \nonumber\\ &&+\bigg(  +{\cal S}^{FF}(s_{1k},s_{kj},x_{1k,kj})
 +{\cal S}^{FF}(s_{ij},s_{kj},x_{ij,kj})
 -{\cal S}^{FF}(s_{1j},s_{kj},x_{1j,kj})
 -{\cal S}^{FF}(s_{ki},s_{kj},x_{ki,kj})
 \bigg)\bigg]\nonumber\\
 &&\times E_3^{0}(i,j,k)\,B_1^{\gamma,0}(1,(\widetilde{jk}),(\widetilde{ij}),6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\end{eqnarray}


==> sub/autoq1Ct1g0AS.tex <==
\section*{q1Ct1g0AS(1,i,j,k,l,7,2)}
\begin{eqnarray}
 \ph{1}&&+A_3^{0}(1,i,l)\,C_0^{\gamma,0}(\overline{1},j,k,(\widetilde{il}),7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{2}&&+A_3^{0}(j,i,k)\,C_0^{\gamma,0}(1,(\widetilde{ji}),(\widetilde{ki}),l,7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{3}&&-2A_3^{0}(1,i,k)\,C_0^{\gamma,0}(\overline{1},j,(\widetilde{ki}),l,7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{4}&&-2A_3^{0}(j,i,l)\,C_0^{\gamma,0}(1,(\widetilde{ji}),k,(\widetilde{li}),7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{5}&&+2A_3^{0}(1,i,j)\,C_0^{\gamma,0}(\overline{1},(\widetilde{ji}),k,l,7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{6}&&+2A_3^{0}(l,i,k)\,C_0^{\gamma,0}(1,j,(\widetilde{ki}),(\widetilde{li}),7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{7}&&+E_3^{0}(l,j,k)\,\tilde{B}_2^{\gamma,0}(1,i,(\widetilde{kj}),(\widetilde{lj}),7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
\snip \ph{8}&&+\,B_4^0(1,j,k,l)\,B_1^{\gamma,0}(\overline{1},i,(\widetilde{jkl}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{9}&&-\,E_3^{0}(l,j,k)\,A_3^{0}(1,(\widetilde{kj}),(\widetilde{lj}))\,B_1^{\gamma,0}(\overline{1},i,[(\widetilde{kj}), (\widetilde{lj})],7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\snip \ph{10}&&+\frac{1}{2}\,\,\tilde{E}_4^0(1,j,i,k)\,B_1^{\gamma,0}(\overline{1},(\widetilde{ijk}),l,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{11}&&-\frac{1}{2}\,\,A_3^{0}(j,i,k)\,E_{3,q}^{0}(1,(\widetilde{ji}),(\widetilde{ki}))\,B_1^{\gamma,0}(\overline{1},[(\widetilde{ji}), (\widetilde{ki})],l,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\snip \ph{12}&&+\frac{1}{2}\,\,\tilde{E}_4^0(l,j,i,k)\,B_1^{\gamma,0}(1,(\widetilde{kij}),(\widetilde{lji}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{13}&&-\frac{1}{2}\,\,A_3^{0}(j,i,k)\,E_3^{0}(l,(\widetilde{ji}),(\widetilde{ki}))\,B_1^{\gamma,0}(1,[(\widetilde{ji}), (\widetilde{ki})],(\widetilde{l\widetilde{(ji})}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{14}&&-\,E_3^{0}(l,j,k)\,A_3^{0}(1,i,(\widetilde{lj}))\,B_1^{\gamma,0}(\overline{1},(\widetilde{jk}),(\widetilde{i\widetilde{(lj})}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{15}&&+\,A_3^{0}(1,i,k)\,E_3^{0}(\overline{1},(\widetilde{ik}),j)\,B_1^{\gamma,0}(\overline{\overline{1}},(\widetilde{j\widetilde{(ik})}),l,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{16}&&+\,A_3^{0}(j,i,l)\,E_3^{0}(1,k,(\widetilde{ji}))\,B_1^{\gamma,0}(\overline{1},(\widetilde{k\widetilde{(ji})}),(\widetilde{li}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{17}&&-\,A_3^{0}(1,i,j)\,E_3^{0}(\overline{1},k,(\widetilde{ji}))\,B_1^{\gamma,0}(\overline{\overline{1}},(\widetilde{k\widetilde{(ji})}),l,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{18}&&-\,A_3^{0}(l,i,k)\,E_3^{0}(1,(\widetilde{ki}),j)\,B_1^{\gamma,0}(\overline{1},(\widetilde{(\widetilde{ki})j}),(\widetilde{li}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{19}&&-\bigg[      +S^{FF}_{1i(\widetilde{ki})}       +S^{FF}_{(\widetilde{ji})il}       -S^{FF}_{1i(\widetilde{ji})}       -S^{FF}_{li(\widetilde{ik})}  \bigg]\nonumber\\
 &&\times E_3^{0}(1,(\widetilde{ki}),(\widetilde{ji}))\,B_1^{\gamma,0}(\overline{1},[(\widetilde{ki}), (\widetilde{ji})],l,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{20}&&+\,A_3^{0}(1,i,k)\,E_3^{0}(l,(\widetilde{ik}),j)\,B_1^{\gamma,0}(\overline{1},(\widetilde{j\widetilde{(ik})}),(\widetilde{l\widetilde{(ik})}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{21}&&+\,A_3^{0}(j,i,l)\,E_3^{0}((\widetilde{li}),k,(\widetilde{ji}))\,B_1^{\gamma,0}(1,(\widetilde{k\widetilde{(ji})}),(\widetilde{(\widetilde{li})k}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{22}&&-\,A_3^{0}(1,i,j)\,E_3^{0}(l,k,(\widetilde{ji}))\,B_1^{\gamma,0}(\overline{1},(\widetilde{k\widetilde{(ji})}),(\widetilde{lk}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{23}&&-\,A_3^{0}(l,i,k)\,E_3^{0}((\widetilde{li}),(\widetilde{ki}),j)\,B_1^{\gamma,0}(1,(\widetilde{(\widetilde{ki})j}),[(\widetilde{li}), (\widetilde{ki})],7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{24}&&-\bigg[      +S^{FF}_{1i(\widetilde{ki})}       +S^{FF}_{(\widetilde{ji})il}       -S^{FF}_{1i(\widetilde{ji})}       -S^{FF}_{li(\widetilde{ik})}  \bigg]\nonumber\\
 &&\times E_3^{0}(l,(\widetilde{ki}),(\widetilde{ji}))\,B_1^{\gamma,0}(1,[(\widetilde{ki}), (\widetilde{ji})],(\widetilde{l\widetilde{(ki})}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\end{eqnarray}


==> sub/autoq2Bhh2g1AT.tex <==
\section*{q2C0g1NFAT(1,j,k,i,6,2)}
\begin{eqnarray}
  \ph{1}&&-\,E_{3,q^\prime\to g}^{0}(j,1,i)\,\hat{B}_1^{\gamma,1}(k,\overline{1},(\widetilde{ij}),6,2)\,\delta(1-x_1)\,\delta(1-x_2)\nonumber\\
  \ph{2}&&-\,\hat{E}_{3,q^\prime}^{1}(j,1,i)\,B_1^{\gamma,0}(k,\overline{1},(\widetilde{ij}),6,2)\,\delta(1-x_1)\,\delta(1-x_2)\nonumber\\
\end{eqnarray}


==> sub/autoq2C0g0AS.tex <==
\section*{q2C0g0AS(1,i,j,k,6,2)}
\begin{eqnarray}
 \ph{1}&&-\frac{1}{2}\,E_{3,q^\prime\to g}^{0}(i,1,k)\,B_1^{\gamma,0}(j,\overline{1},(\widetilde{ik}),6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{2}&&-\frac{1}{2}\,E_{3,q^\prime\to g}^{0}(j,1,k)\,B_1^{\gamma,0}((\widetilde{jk}),\overline{1},i,6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\end{eqnarray}


==> sub/autoq2C0g1AT.tex <==
\section*{q2C0g1AT(1,j,k,i,6,2)}
\begin{eqnarray}
  \ph{1}&&-\frac{1}{2}\,\,E_{3,q^\prime\to g}^{0}(j,1,i)\,\bigg[\,B_1^{\gamma,1}(k,\overline{1},(\widetilde{ij}),6,2)\,\delta(1-x_1)\,\delta(1-x_2)\nonumber\\
  &&+\,\bigg( 
 +J_{2,GQ}^{1,IF}(s_{\overline{1}(\widetilde{ij})})
 -J_{2,QG,g \to q}^{1,IF}(s_{\overline{1}(\widetilde{ij})})
 +J_{2,GQ}^{1,IF}(s_{\overline{1}k})
 -J_{2,QG,g \to q}^{1,IF}(s_{\overline{1}k})\bigg)\,B_1^{\gamma,0}(k,\overline{1},(\widetilde{ij}),6,2) \bigg]\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
  \ph{2}&&-\frac{1}{2}\,\,E_{3,q^\prime\to g}^{0}(k,1,i)\,\bigg[\,B_1^{\gamma,1}((\widetilde{ik}),\overline{1},j,6,2)\,\delta(1-x_1)\,\delta(1-x_2)\nonumber\\
  &&+\,\bigg( 
 +J_{2,GQ}^{1,IF}(s_{\overline{1}(\widetilde{ik})})
 -J_{2,QG,g \to q}^{1,IF}(s_{\overline{1}(\widetilde{ik})})
 +J_{2,GQ}^{1,IF}(s_{\overline{1}j})
 -J_{2,QG,g \to q}^{1,IF}(s_{\overline{1}j})\bigg)\,B_1^{\gamma,0}((\widetilde{ik}),\overline{1},j,6,2) \bigg]\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
  \ph{3}&&-\frac{1}{2}\,\bigg[\,E_{3,q^\prime}^{1}(k,1,i)\,\delta(1-x_1)\,\delta(1-x_2)
  \nonumber\\&&\,  
   +\bigg( 
 +J_{2,QQ}^{1,IF}(s_{1k})
 +J_{2,QQ}^{1,FF}(s_{ki})
 +2J_{2,QG,g \to q}^{1,IF}(s_{\overline{1}(\widetilde{ki})})
 -2J_{2,GQ}^{1,IF}(s_{\overline{1}(\widetilde{ki})})\bigg)\,E_{3,q^\prime\to g}^{0}(k,1,i)\bigg]\,B_1^{\gamma,0}((\widetilde{ki}),\overline{1},j,6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
  \ph{4}&&-\frac{1}{2}\,\bigg[\,E_{3,q^\prime}^{1}(j,1,i)\,\delta(1-x_1)\,\delta(1-x_2)
  \nonumber\\&&\,  
   +\bigg( 
 +J_{2,QQ}^{1,IF}(s_{1j})
 +J_{2,QQ}^{1,FF}(s_{ji})
 +2J_{2,QG,g \to q}^{1,IF}(s_{\overline{1}(\widetilde{ji})})
 -2J_{2,GQ}^{1,IF}(s_{\overline{1}(\widetilde{ji})})\bigg)\,E_{3,q^\prime\to g}^{0}(j,1,i)\bigg]\,B_1^{\gamma,0}(k,\overline{1},(\widetilde{ji}),6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
\end{eqnarray}


==> sub/autoq2C1g0AS.tex <==
\section*{q2C1g0AS(1,i,j,k,l,7,2)}
\begin{eqnarray}
 \ph{1}&&-E_{3,q^\prime\to g}^{0}(k,1,l)\,B_2^{\gamma,0}((\widetilde{kl}),\overline{1},i,j,7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{2}&&-E_{3,q^\prime\to g}^{0}(j,l,1)\,B_2^{\gamma,0}(k,i,\overline{1},(\widetilde{jl}),7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
\snip \ph{3}&&-\,E_4^0(j,l,1,i)\,B_1^{\gamma,0}(k,\overline{1},(\widetilde{jli}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{4}&&+\,E_{3,q^\prime\to g}^{0}(k,1,l)\,D_3^{0}(j,\overline{1},i)\,B_1^{\gamma,0}((\widetilde{kl}),\overline{\overline{1}},(\widetilde{ij}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{5}&&+\,A_3^{0}(j,i,1)\,E_{3,q^\prime\to g}^{0}((\widetilde{ji}),\overline{1},l)\,B_1^{\gamma,0}(k,\overline{\overline{1}},(\widetilde{(\widetilde{ji})l}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\snip \ph{6}&&-\,E_4^0(k,1,l,i)\,B_1^{\gamma,0}((\widetilde{kli}),\overline{1},j,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{7}&&+\,E_{3,q^\prime\to g}^{0}(j,l,1)\,D_3^{0}(k,\overline{1},i)\,B_1^{\gamma,0}((\widetilde{ik}),\overline{\overline{1}},(\widetilde{jl}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{8}&&+\,A_3^{0}(l,i,k)\,E_{3,q^\prime\to g}^{0}((\widetilde{ki}),1,(\widetilde{li}))\,B_1^{\gamma,0}([(\widetilde{ki}), (\widetilde{li})],\overline{1},j,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\snip \ph{9}&&+\,B_4^0(k,1,l,j)\,B_1^{\gamma,0}((\widetilde{jlk}),\overline{1},i,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{10}&&-\,E_{3,q^\prime\to g}^{0}(j,l,1)\,a_{3,g\to q}^{0}(k,\overline{1},(\widetilde{jl}))\,B_1^{\gamma,0}((\widetilde{k\widetilde{(jl})}),\overline{\overline{1}},i,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{11}&&-\,E_{3,q^\prime\to g}^{0}(k,1,l)\,a_{3,g\to q}^{0}(j,\overline{1},(\widetilde{kl}))\,B_1^{\gamma,0}((\widetilde{j\widetilde{(kl})}),\overline{\overline{1}},i,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\snip \ph{12}&&+\,B_4^0(k,1,l,j)\,B_1^{\gamma,0}(\overline{1},i,(\widetilde{jlk}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{13}&&-\,E_{3,q^\prime\to g}^{0}(j,l,1)\,a_{3,g\to q}^{0}((\widetilde{jl}),\overline{1},k)\,B_1^{\gamma,0}(\overline{\overline{1}},i,(\widetilde{k\widetilde{(jl})}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{14}&&-\,E_{3,q^\prime\to g}^{0}(k,1,l)\,a_{3,g\to q}^{0}((\widetilde{kl}),\overline{1},j)\,B_1^{\gamma,0}(\overline{\overline{1}},i,(\widetilde{j\widetilde{(kl})}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\end{eqnarray}


==> sub/autoq2Ct0g1AT.tex <==
\section*{q2Ct0g1AT(1,j,k,i,6,2)}
\begin{eqnarray}
  \ph{1}&&-\frac{1}{2}\,\,E_{3,q^\prime\to g}^{0}(j,1,i)\,\bigg[\,\tilde{B}_3^{\gamma,1}(k,\overline{1},(\widetilde{ij}),6,2)\,\delta(1-x_1)\,\delta(1-x_2)\nonumber\\
 &&\phantom{\bigg[}+J_{2,QQ}^{1,FF}(s_{k(\widetilde{ij})})\,B_1^{\gamma,0}(k,\overline{1},(\widetilde{ij}),6,2) \bigg]\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
  \ph{2}&&-\frac{1}{2}\,\,E_{3,q^\prime\to g}^{0}(k,1,i)\,\bigg[\,\tilde{B}_3^{\gamma,1}((\widetilde{ik}),\overline{1},j,6,2)\,\delta(1-x_1)\,\delta(1-x_2)\nonumber\\
 &&\phantom{\bigg[}+J_{2,QQ}^{1,FF}(s_{j(\widetilde{ik})})\,B_1^{\gamma,0}((\widetilde{ik}),\overline{1},j,6,2) \bigg]\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
  \ph{3}&&-\frac{1}{2}\,\bigg[\,\tilde{E}_{3,q^\prime}^{1}(j,1,i)\,\delta(1-x_1)\,\delta(1-x_2)
 +J_{2,QQ}^{1,IF}(s_{1i})\,E_{3,q^\prime\to g}^{0}(j,1,i)\bigg]\,B_1^{\gamma,0}(k,\overline{1},(\widetilde{ij}),6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
  \ph{4}&&-\frac{1}{2}\,\bigg[\,\tilde{E}_{3,q^\prime}^{1}(k,1,i)\,\delta(1-x_1)\,\delta(1-x_2)
 +J_{2,QQ}^{1,IF}(s_{1i})\,E_{3,q^\prime\to g}^{0}(k,1,i)\bigg]\,B_1^{\gamma,0}((\widetilde{ik}),\overline{1},j,6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
 \ph{5}&&-2\bigg[ +J_{2,QQ}^{1,FF}(s_{ki})
 -J_{2,QQ}^{1,IF}(s_{1k})
 -J_{2,QQ}^{1,FF}(s_{ij})
 +J_{2,QQ}^{1,IF}(s_{1j})
 \nonumber\\ &&+\bigg(  +{\cal S}^{FF}(s_{1k},s_{jk},x_{1k,jk})
 +{\cal S}^{FF}(s_{ij},s_{jk},x_{ij,jk})
 -{\cal S}^{FF}(s_{1j},s_{jk},x_{1j,jk})
 -{\cal S}^{FF}(s_{ki},s_{jk},x_{ki,jk})
 \bigg)\bigg]\nonumber\\
 &&\times E_3^{0}(j,1,i)\,B_1^{\gamma,0}(k,\overline{1},(\widetilde{ij}),6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\end{eqnarray}


==> sub/autoq2Ct1g0AS.tex <==
\section*{q2Ct1g0AS(1,i,j,k,l,7,2)}
\begin{eqnarray}
 \ph{1}&&-\frac{1}{2}\,E_{3,q^\prime\to g}^{0}(j,1,l)\,\tilde{B}_2^{\gamma,0}(k,\overline{1},i,(\widetilde{jl}),7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{2}&&-\frac{1}{2}\,E_{3,q^\prime\to g}^{0}(k,1,l)\,\tilde{B}_2^{\gamma,0}((\widetilde{kl}),i,\overline{1},j,7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
\snip \ph{3}&&+\,B_4^0(j,1,l,k)\,B_1^{\gamma,0}(\overline{1},i,(\widetilde{jlk}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{4}&&-\frac{1}{2}\,\,E_{3,q^\prime\to g}^{0}(j,1,l)\,A_3^{0}((\widetilde{jl}),\overline{1},k)\,B_1^{\gamma,0}(\overline{\overline{1}},i,(\widetilde{(\widetilde{jl})k}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{5}&&-\frac{1}{2}\,\,E_{3,q^\prime\to g}^{0}(k,1,l)\,A_3^{0}((\widetilde{kl}),\overline{1},j)\,B_1^{\gamma,0}(\overline{\overline{1}},i,(\widetilde{(\widetilde{kl})j}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\snip \ph{6}&&-\frac{1}{2}\,\,\tilde{E}_4^0(j,1,i,l)\,B_1^{\gamma,0}(k,\overline{1},(\widetilde{jil}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{7}&&+\frac{1}{2}\,\,A_3^{0}(1,i,l)\,E_{3,q^\prime\to g}^{0}(j,\overline{1},(\widetilde{il}))\,B_1^{\gamma,0}(k,\overline{\overline{1}},(\widetilde{j\widetilde{(il})}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\snip \ph{8}&&-\frac{1}{2}\,\,\tilde{E}_4^0(k,1,i,l)\,B_1^{\gamma,0}((\widetilde{kil}),\overline{1},j,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{9}&&+\frac{1}{2}\,\,A_3^{0}(1,i,l)\,E_{3,q^\prime\to g}^{0}(k,\overline{1},(\widetilde{il}))\,B_1^{\gamma,0}((\widetilde{k\widetilde{(il})}),\overline{\overline{1}},j,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{10}&&+\frac{1}{2}\,\,E_{3,q^\prime\to g}^{0}(j,1,l)\,A_3^{0}((\widetilde{jl}),i,k)\,B_1^{\gamma,0}((\widetilde{ki}),\overline{1},(\widetilde{(\widetilde{jl})i}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{11}&&+\frac{1}{2}\,\,E_{3,q^\prime\to g}^{0}(k,1,l)\,A_3^{0}((\widetilde{kl}),i,j)\,B_1^{\gamma,0}((\widetilde{(\widetilde{kl})i}),\overline{1},(\widetilde{ij}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{12}&&-\,A_3^{0}(1,i,k)\,E_3^{0}((\widetilde{ik}),\overline{1},l)\,B_1^{\gamma,0}((\widetilde{l\widetilde{(ik})}),\overline{\overline{1}},j,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{13}&&-\,A_3^{0}(j,i,l)\,E_3^{0}(k,1,(\widetilde{li}))\,B_1^{\gamma,0}((\widetilde{k\widetilde{(li})}),\overline{1},(\widetilde{ji}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{14}&&+\,A_3^{0}(1,i,j)\,E_3^{0}(k,\overline{1},l)\,B_1^{\gamma,0}((\widetilde{lk}),\overline{\overline{1}},(\widetilde{ji}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{15}&&+\,A_3^{0}(l,i,k)\,E_3^{0}((\widetilde{ki}),1,(\widetilde{li}))\,B_1^{\gamma,0}([(\widetilde{ki}), (\widetilde{li})],\overline{1},j,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{16}&&+\bigg[      +S^{FF}_{1i(\widetilde{ik})}       +S^{FF}_{ji(\widetilde{li})}       -S^{FF}_{1ij}       -S^{FF}_{(\widetilde{li})i(\widetilde{ik})}  \bigg]\nonumber\\
 &&\times E_3^{0}((\widetilde{ik}),1,(\widetilde{li}))\,B_1^{\gamma,0}([(\widetilde{ik}), (\widetilde{li})],\overline{1},j,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{17}&&-\,A_3^{0}(1,i,k)\,E_3^{0}(j,\overline{1},l)\,B_1^{\gamma,0}((\widetilde{ki}),\overline{\overline{1}},(\widetilde{lj}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{18}&&-\,A_3^{0}(j,i,l)\,E_3^{0}((\widetilde{ji}),1,(\widetilde{li}))\,B_1^{\gamma,0}(k,\overline{1},[(\widetilde{ji}), (\widetilde{li})],7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{19}&&+\,A_3^{0}(1,i,j)\,E_3^{0}((\widetilde{ji}),\overline{1},l)\,B_1^{\gamma,0}(k,\overline{\overline{1}},(\widetilde{l\widetilde{(ji})}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{20}&&+\,A_3^{0}(l,i,k)\,E_3^{0}(j,1,(\widetilde{li}))\,B_1^{\gamma,0}((\widetilde{ki}),\overline{1},(\widetilde{j\widetilde{(li})}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{21}&&-\bigg[      +S^{FF}_{1i(\widetilde{ij})}       +S^{FF}_{ki(\widetilde{li})}       -S^{FF}_{1ik}       -S^{FF}_{(\widetilde{li})i(\widetilde{ij})}  \bigg]\nonumber\\
 &&\times E_3^{0}((\widetilde{ij}),1,(\widetilde{li}))\,B_1^{\gamma,0}(k,\overline{1},[(\widetilde{ij}), (\widetilde{li})],7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\end{eqnarray}


==> sub/autoqB1g2AU.tex <==
\section*{qB1g2AU}
\begin{eqnarray}
\lefteqn{{\tt qB1g2AU(1,3,4,5,2) =}} \\
 \ph{1}&&+\bigg[ 
 -\frac{1}{2}\,\,{\cal D}_{3,q}^{0}(s_{13}) 
 +\,\Gamma^{(1)}_{qq}(z_1) 
 -\frac{1}{2}\,\,{\cal D}_{3}^{0}(s_{34}) 
 \bigg] 
\left( -\frac{b_0}{\epsilon}B_1^{\gamma,0}(1,3,4,5,2) +B_1^{\gamma,1}(1,3,4,5,2)\right)
 \nonumber\\
 \ph{2}&&+\bigg[ 
 -\frac{1}{8}\,\,{\cal D}_{3,q}^{0}(s_{13})\otimes{\cal D}_{3,q}^{0}(s_{13}) 
 +\frac{1}{2}\,\,\Gamma^{(1)}_{qq}(z_1)\otimes{\cal D}_{3,q}^{0}(s_{13}) 
 -\frac{1}{4}\,\,{\cal D}_{3,q}^{0}(s_{13})\otimes{\cal D}_{3}^{0}(s_{34}) 
 \nonumber \\ && \phantom{+\bigg[} 
 -\frac{1}{2}\,\,\Gamma^{(1)}_{qq}(z_1)\otimes\Gamma^{(1)}_{qq}(z_1) 
 +\frac{1}{2}\,\,\Gamma^{(1)}_{qq}(z_1)\otimes{\cal D}_{3}^{0}(s_{34}) 
 -\frac{1}{8}\,\,{\cal D}_{3}^{0}(s_{34})\otimes{\cal D}_{3}^{0}(s_{34}) 
 \bigg] 
 B_1^{\gamma,0}(1,3,4,5,2)
 \nonumber\\
 \ph{3}&&+\bigg[ 
 -\frac{b_0}{2\epsilon}\,\bigg( \frac{s_{34}}{\mu_R^2}\bigg)^{-\epsilon}\,{\cal D}_{3}^{0}(s_{34}) 
 +\frac{1}{4}\,\,{\cal D}_{3}^{0}(s_{34})\otimes{\cal D}_{3}^{0}(s_{34}) 
 -\frac{1}{2}\,\,{\cal D}_{4}^{0}(s_{34}) 
 \nonumber \\ && \phantom{+\bigg[} 
 -\frac{1}{2}\,\,{\cal{D}}_{3}^{1}(s_{34}) 
 \bigg] 
 B_1^{\gamma,0}(1,3,4,5,2)
 \nonumber\\
 \ph{4}&&+\bigg[ 
 -\frac{b_0}{2\epsilon}\,\bigg( \frac{s_{13}}{\mu_R^2}\bigg)^{-\epsilon}\,{\cal D}_{3,q}^{0}(s_{13}) 
 +\frac{1}{4}\,\,{\cal D}_{3,q}^{0}(s_{13})\otimes{\cal D}_{3,q}^{0}(s_{13}) 
 -\frac{1}{2}\,\,{\cal D}_{4,q}^{0}(s_{13}) 
 \nonumber \\ && \phantom{+\bigg[} 
 -\frac{1}{2}\,\,{\cal{D}}_{3,q}^{1}(s_{13}) 
 +\,\Gamma^{(2)}_{qq}(z_1) 
 \bigg] 
 B_1^{\gamma,0}(1,3,4,5,2)
 \nonumber\\
 \ph{5}&&+\bigg[ 
 +\frac{1}{2}\,\,\tilde{\cal A}_{4,q}^{0}(s_{14}) 
 +\,\tilde{\cal{A}}_{3,q}^{1}(s_{14}) 
 -\frac{1}{2}\,\,{\cal A}_{3,q}^{0}(s_{14})\otimes{\cal A}_{3,q}^{0}(s_{14}) 
 \bigg] 
 B_1^{\gamma,0}(1,3,4,5,2)
 \nonumber\\
\end{eqnarray}


==> sub/autoqBh1g2AU.tex <==
\section*{qBh1g2AU}
\begin{eqnarray}
\lefteqn{{\tt qBh1g2AU(1,3,4,5,2) =}} \\
 \ph{1}&&+\bigg[ 
 -\frac{1}{2}\,\,{\cal D}_{3}^{0}(s_{34}) 
 -\frac{1}{2}\,\,{\cal D}_{3,q}^{0}(s_{13}) 
 +\,\Gamma^{(1)}_{qq}(z_1) 
 \bigg] 
\left( -\frac{b_F}{\epsilon}B_1^{\gamma,0}(1,3,4,5,2) +\hat{B}_1^{\gamma,1}(1,3,4,5,2)\right)
 \nonumber\\
 \ph{2}&&+\bigg[ 
 +\frac{1}{2}\,\,{\cal E}_{3,q}^{0}(s_{13}) 
 +\frac{1}{2}\,\,{\cal E}_{3}^{0}(s_{34}) 
 \bigg] 
\left( +\frac{b_0}{\epsilon}B_1^{\gamma,0}(1,3,4,5,2) -B_1^{\gamma,1}(1,3,4,5,2)\right)
 \nonumber\\
 \ph{3}&&+\bigg[ 
 -\frac{1}{4}\,\,{\cal D}_{3}^{0}(s_{34})\otimes{\cal E}_{3,q}^{0}(s_{13}) 
 -\frac{1}{4}\,\,{\cal D}_{3,q}^{0}(s_{13})\otimes{\cal E}_{3,q}^{0}(s_{13}) 
 +\frac{1}{2}\,\,\Gamma^{(1)}_{qq}(z_1)\otimes{\cal E}_{3,q}^{0}(s_{13}) 
 \nonumber \\ && \phantom{+\bigg[} 
 -\frac{1}{4}\,\,{\cal D}_{3}^{0}(s_{34})\otimes{\cal E}_{3}^{0}(s_{34}) 
 -\frac{1}{4}\,\,{\cal D}_{3,q}^{0}(s_{13})\otimes{\cal E}_{3}^{0}(s_{34}) 
 +\frac{1}{2}\,\,\Gamma^{(1)}_{qq}(z_1)\otimes{\cal E}_{3}^{0}(s_{34}) 
 \bigg] 
 B_1^{\gamma,0}(1,3,4,5,2)
 \nonumber\\
 \ph{4}&&+\bigg[ 
 -\frac{b_F}{2\epsilon}\,\bigg( \frac{s_{34}}{\mu_R^2}\bigg)^{-\epsilon}\,{\cal D}_{3}^{0}(s_{34}) 
 -\frac{b_0}{2\epsilon}\,\bigg( \frac{s_{34}}{\mu_R^2}\bigg)^{-\epsilon}\,{\cal E}_{3}^{0}(s_{34}) 
 +\frac{1}{2}\,\,{\cal D}_{3}^{0}(s_{34})\otimes{\cal E}_{3}^{0}(s_{34}) 
 \nonumber \\ && \phantom{+\bigg[} 
 -\,{\cal E}_{4}^{0}(s_{34}) 
 -\frac{1}{2}\,\,{\cal{E}}_{3}^{1}(s_{34}) 
 -\frac{1}{2}\,\,\hat{\cal{D}}_{3}^{1}(s_{34}) 
 \bigg] 
 B_1^{\gamma,0}(1,3,4,5,2)
 \nonumber\\
 \ph{5}&&+\bigg[ 
 -\frac{b_0}{2\epsilon}\,\bigg( \frac{s_{13}}{\mu_R^2}\bigg)^{-\epsilon}\,{\cal E}_{3,q}^{0}(s_{13}) 
 -\frac{b_F}{2\epsilon}\,\bigg( \frac{s_{13}}{\mu_R^2}\bigg)^{-\epsilon}\,{\cal D}_{3,q}^{0}(s_{13}) 
 +\frac{1}{2}\,\,{\cal D}_{3,q}^{0}(s_{13})\otimes{\cal E}_{3,q}^{0}(s_{13}) 
 \nonumber \\ && \phantom{+\bigg[} 
 -\,{\cal E}_{4,q}^{0}(s_{13}) 
 -\frac{1}{2}\,\,{\cal{E}}_{3,q}^{1}(s_{13}) 
 -\frac{1}{2}\,\,\hat{\cal{D}}_{3,q}^{1}(s_{13}) 
 \nonumber \\ && \phantom{+\bigg[} 
 +\,\Gamma^{(2)}_{qq,F}(z_1) 
 \bigg] 
 B_1^{\gamma,0}(1,3,4,5,2)
 \nonumber\\
\end{eqnarray}


==> sub/autoqBhh1g2AU.tex <==
\section*{qBhh1g2AU}
\begin{eqnarray}
\lefteqn{{\tt qBhh1g2AU(1,3,4,5,2) =}} \\
 \ph{1}&&+\bigg[ 
 -\frac{1}{2}\,\,{\cal E}_{3}^{0}(s_{34}) 
 -\frac{1}{2}\,\,{\cal E}_{3,q}^{0}(s_{13}) 
 \bigg] 
\left( -\frac{b_F}{\epsilon}B_1^{\gamma,0}(1,3,4,5,2) +\hat{B}_1^{\gamma,1}(1,3,4,5,2)\right)
 \nonumber\\
 \ph{2}&&+\bigg[ 
 -\frac{b_F}{2\epsilon}\,{\cal E}_{3}^{0}(s_{34})\,\bigg( \frac{s_{34}}{\mu_R^2}\bigg)^{-\epsilon} 
 -\frac{b_F}{2\epsilon}\,{\cal E}_{3,q}^{0}(s_{13})\,\bigg( \frac{s_{13}}{\mu_R^2}\bigg)^{-\epsilon} 
 -\frac{1}{2}\,\,\hat{\cal{E}}_{3}^{1}(s_{34}) 
 \nonumber \\ && \phantom{+\bigg[} 
 -\frac{1}{2}\,\,\hat{\cal{E}}_{3,q}^{1}(s_{13}) 
 \bigg] 
 B_1^{\gamma,0}(1,3,4,5,2)
 \nonumber\\
\end{eqnarray}


==> sub/autoqBt1g2AU.tex <==
\section*{qBt1g2AU}
\begin{eqnarray}
\lefteqn{{\tt qBt1g2AU(1,3,4,5,2) =}} \\
 \ph{1}&&+\bigg[ 
 -\frac{1}{2}\,\,{\cal D}_{3,q}^{0}(s_{13}) 
 +\,\Gamma^{(1)}_{qq}(z_1) 
 -\frac{1}{2}\,\,{\cal D}_{3}^{0}(s_{34}) 
 \bigg] 
 \tilde{B}_3^{\gamma,1}(1,3,4,5,2)
 \nonumber\\
 \ph{2}&&+\bigg[ 
 -\,{\cal A}_{3,q}^{0}(s_{14}) 
 +\,\Gamma^{(1)}_{qq}(z_1) 
 \bigg] 
\left( -\frac{b_0}{\epsilon}B_1^{\gamma,0}(1,3,4,5,2) +B_1^{\gamma,1}(1,3,4,5,2)\right)
 \nonumber\\
 \ph{3}&&+\bigg[ 
 -\frac{1}{2}\,\,{\cal D}_{3,q}^{0}(s_{13})\otimes{\cal A}_{3,q}^{0}(s_{14}) 
 +\frac{1}{2}\,\,\Gamma^{(1)}_{qq}(z_1)\otimes{\cal D}_{3,q}^{0}(s_{13}) 
 +\,\Gamma^{(1)}_{qq}(z_1)\otimes{\cal A}_{3,q}^{0}(s_{14}) 
 \nonumber \\ && \phantom{+\bigg[} 
 -\,\Gamma^{(1)}_{qq}(z_1)\otimes\Gamma^{(1)}_{qq}(z_1) 
 \bigg] 
 B_1^{\gamma,0}(1,3,4,5,2)
 \nonumber\\
 \ph{4}&&+\bigg[ 
 -\frac{1}{2}\,\,{\cal D}_{3}^{0}(s_{34})\otimes{\cal A}_{3,q}^{0}(s_{14}) 
 +\frac{1}{2}\,\,\Gamma^{(1)}_{qq}(z_1)\otimes{\cal D}_{3}^{0}(s_{34}) 
 \bigg] 
 B_1^{\gamma,0}(1,3,4,5,2)
 \nonumber\\
 \ph{5}&&+\bigg[ 
 -\frac{b_0}{\epsilon}\,\bigg( \frac{s_{14}}{\mu_R^2}\bigg)^{-\epsilon}\,{\cal A}_{3,q}^{0}(s_{14}) 
 +\,{\cal A}_{3,q}^{0}(s_{14})\otimes{\cal A}_{3,q}^{0}(s_{14}) 
 -\,{\cal A}_{4,q}^{0}(s_{14}) 
 \nonumber \\ && \phantom{+\bigg[} 
 -\,{\cal{A}}_{3,q}^{1}(s_{14}) 
 +\,\Gamma^{(2)}_{qq}(z_1) 
 \bigg] 
 B_1^{\gamma,0}(1,3,4,5,2)
 \nonumber\\
 \ph{6}&&+\bigg[ 
 -\frac{1}{2}\,\,\tilde{\cal A}_{4,q}^{0}(s_{14}) 
 -\,\tilde{\cal{A}}_{3,q}^{1}(s_{14}) 
 -\,{\cal C}_{4,\bar{q},\bar{q}q\bar{q}}^{0}(s_{14}) 
 \nonumber \\ && \phantom{+\bigg[} 
 -2\,{\cal C}_{4,q}^{0}(s_{14}) 
 -\,\widetilde{\widetilde{\Gamma}}^{(2)}_{qq}(z_1) 
 \bigg] 
 B_1^{\gamma,0}(1,3,4,5,2)
 \nonumber\\
 \ph{7}&&+\bigg[ 
 -\,{\cal C}_{4,\bar{q},q\bar{q}\bar{q}}^{0}(s_{14}) 
 -\,\Gamma^{(2)}_{q\bar{q}}t(z_1) 
 \bigg] 
 B_1^{\gamma,0}(4,3,1,5,2)
 \nonumber\\
\end{eqnarray}


==> sub/autoqBth1g2AU.tex <==
\section*{qBth1g2AU}
\begin{eqnarray}
\lefteqn{{\tt qBth1g2AU(1,3,4,5,2) =}} \\
 \ph{1}&&+\bigg[ 
 +\,{\cal A}_{3,q}^{0}(s_{14}) 
 -\,\Gamma^{(1)}_{qq}(z_1) 
 \bigg] 
\left( -\frac{b_F}{\epsilon}B_1^{\gamma,0}(1,3,4,5,2) +\hat{B}_1^{\gamma,1}(1,3,4,5,2)\right)
 \nonumber\\
 \ph{2}&&+\bigg[ 
 +\frac{1}{2}\,\,{\cal E}_{3,q}^{0}(s_{13}) 
 +\frac{1}{2}\,\,{\cal E}_{3}^{0}(s_{34}) 
 \bigg] 
 \tilde{B}_3^{\gamma,1}(1,3,4,5,2)
 \nonumber\\
 \ph{3}&&+\bigg[ 
 +\frac{1}{2}\,\,{\cal E}_{3}^{0}(s_{34})\otimes{\cal A}_{3,q}^{0}(s_{14}) 
 +\frac{1}{2}\,\,{\cal E}_{3,q}^{0}(s_{13})\otimes{\cal A}_{3,q}^{0}(s_{14}) 
 -\frac{1}{2}\,\,\Gamma^{(1)}_{qq}(z_1)\otimes{\cal E}_{3}^{0}(s_{34}) 
 \nonumber \\ && \phantom{+\bigg[} 
 -\frac{1}{2}\,\,\Gamma^{(1)}_{qq}(z_1)\otimes{\cal E}_{3,q}^{0}(s_{13}) 
 \bigg] 
 B_1^{\gamma,0}(1,3,4,5,2)
 \nonumber\\
 \ph{4}&&+\bigg[ 
 +\frac{1}{2}\,\,\tilde{\cal E}_{4,q}^{0}(s_{13}) 
 +\frac{1}{2}\,\,\tilde{\cal{E}}_{3,q}^{1}(s_{13}) 
 -\,\Gamma^{(2)}_{qq,F}(z_1) 
 \bigg] 
 B_1^{\gamma,0}(1,3,4,5,2)
 \nonumber\\
 \ph{5}&&+\bigg[ 
 +\frac{1}{2}\,\,\tilde{\cal E}_{4}^{0}(s_{34}) 
 +\frac{1}{2}\,\,\tilde{\cal{E}}_{3}^{1}(s_{34}) 
 \bigg] 
 B_1^{\gamma,0}(1,3,4,5,2)
 \nonumber\\
 \ph{6}&&+\bigg[ 
 +\frac{b_F}{\epsilon}\,\bigg( \frac{s_{14}}{\mu_R^2}\bigg)^{-\epsilon}\,{\cal A}_{3,q}^{0}(s_{14}) 
 +\,{\cal B}_{4,q}^{0}(s_{14}) 
 +\,\hat{\cal{A}}_{3,q}^{1}(s_{14}) 
 \bigg] 
 B_1^{\gamma,0}(1,3,4,5,2)
 \nonumber\\
\end{eqnarray}


==> sub/autoqBtt1g2AU.tex <==
\section*{qBtt1g2AU}
\begin{eqnarray}
\lefteqn{{\tt qBtt1g2AU(1,3,4,5,2) =}} \\
 \ph{1}&&+\bigg[ 
 -\,{\cal A}_{3,q}^{0}(s_{14}) 
 +\,\Gamma^{(1)}_{qq}(z_1) 
 \bigg] 
 \tilde{B}_3^{\gamma,1}(1,3,4,5,2)
 \nonumber\\
 \ph{2}&&+\bigg[ 
 +\,\Gamma^{(1)}_{qq}(z_1)\otimes{\cal A}_{3,q}^{0}(s_{14}) 
 -\frac{1}{2}\,\,\Gamma^{(1)}_{qq}(z_1)\otimes\Gamma^{(1)}_{qq}(z_1) 
 -\frac{1}{2}\,\,\tilde{\cal A}_{4,q}^{0}(s_{14}) 
 \nonumber \\ && \phantom{+\bigg[} 
 -\,\tilde{\cal{A}}_{3,q}^{1}(s_{14}) 
 -\,{\cal C}_{4,\bar{q},\bar{q}q\bar{q}}^{0}(s_{14}) 
 -2\,{\cal C}_{4,q}^{0}(s_{14}) 
 \nonumber \\ && \phantom{+\bigg[} 
 -\,\widetilde{\widetilde{\Gamma}}^{(2)}_{qq}(z_1) 
 \bigg] 
 B_1^{\gamma,0}(1,3,4,5,2)
 \nonumber\\
 \ph{3}&&+\bigg[ 
 -\,{\cal C}_{4,\bar{q},q\bar{q}\bar{q}}^{0}(s_{14}) 
 -\,\Gamma^{(2)}_{q\bar{q}}t(z_1) 
 \bigg] 
 B_1^{\gamma,0}(4,3,1,5,2)
 \nonumber\\
\end{eqnarray}


==> sub/autoqbB1g1AT.tex <==
\section*{qbB1g1AT(j,i,1,5,2)}
\begin{eqnarray}
  \ph{1}&&-J_{2,QG}^{1,FF}(s_{ji})\,B_1^{\gamma,0}(j,i,1,5,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
  \ph{2}&&-J_{2,QG}^{1,IF}(s_{1i})\,B_1^{\gamma,0}(j,i,1,5,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
\end{eqnarray}


==> sub/autoqbB1g2AU.tex <==
\section*{qbB1g2AU}
\begin{eqnarray}
\lefteqn{{\tt qbB1g2AU(4,3,1,5,2) =}} \\
 \ph{1}&&+\bigg[ 
 +\,\Gamma^{(1)}_{qq}(z_1) 
 -\frac{1}{2}\,\,{\cal D}_{3,q}^{0}(s_{13}) 
 -\frac{1}{2}\,\,{\cal D}_{3}^{0}(s_{34}) 
 \bigg] 
\left( -\frac{b_0}{\epsilon}B_1^{\gamma,0}(4,3,1,5,2) +B_1^{\gamma,1}(4,3,1,5,2)\right)
 \nonumber\\
 \ph{2}&&+\bigg[ 
 -\frac{1}{8}\,\,{\cal D}_{3,q}^{0}(s_{13})\otimes{\cal D}_{3,q}^{0}(s_{13}) 
 -\frac{1}{4}\,\,{\cal D}_{3,q}^{0}(s_{13})\otimes{\cal D}_{3}^{0}(s_{34}) 
 +\frac{1}{2}\,\,\Gamma^{(1)}_{qq}(z_1)\otimes{\cal D}_{3,q}^{0}(s_{13}) 
 \nonumber \\ && \phantom{+\bigg[} 
 -\frac{1}{8}\,\,{\cal D}_{3}^{0}(s_{34})\otimes{\cal D}_{3}^{0}(s_{34}) 
 +\frac{1}{2}\,\,\Gamma^{(1)}_{qq}(z_1)\otimes{\cal D}_{3}^{0}(s_{34}) 
 -\frac{1}{2}\,\,\Gamma^{(1)}_{qq}(z_1)\otimes\Gamma^{(1)}_{qq}(z_1) 
 \bigg] 
 B_1^{\gamma,0}(4,3,1,5,2)
 \nonumber\\
 \ph{3}&&+\bigg[ 
 -\frac{b_0}{2\epsilon}\,\bigg( \frac{s_{34}}{\mu_R^2}\bigg)^{-\epsilon}\,{\cal D}_{3}^{0}(s_{34}) 
 +\frac{1}{4}\,\,{\cal D}_{3}^{0}(s_{34})\otimes{\cal D}_{3}^{0}(s_{34}) 
 -\frac{1}{2}\,\,{\cal D}_{4}^{0}(s_{34}) 
 \nonumber \\ && \phantom{+\bigg[} 
 -\frac{1}{2}\,\,{\cal{D}}_{3}^{1}(s_{34}) 
 \bigg] 
 B_1^{\gamma,0}(4,3,1,5,2)
 \nonumber\\
 \ph{4}&&+\bigg[ 
 -\frac{b_0}{2\epsilon}\,\bigg( \frac{s_{13}}{\mu_R^2}\bigg)^{-\epsilon}\,{\cal D}_{3,q}^{0}(s_{13}) 
 +\frac{1}{4}\,\,{\cal D}_{3,q}^{0}(s_{13})\otimes{\cal D}_{3,q}^{0}(s_{13}) 
 -\frac{1}{2}\,\,{\cal D}_{4,q}^{0}(s_{13}) 
 \nonumber \\ && \phantom{+\bigg[} 
 -\frac{1}{2}\,\,{\cal{D}}_{3,q}^{1}(s_{13}) 
 +\,\Gamma^{(2)}_{qq}(z_1) 
 \bigg] 
 B_1^{\gamma,0}(4,3,1,5,2)
 \nonumber\\
 \ph{5}&&+\bigg[ 
 +\frac{1}{2}\,\,\tilde{\cal A}_{4,q}^{0}(s_{14}) 
 +\,\tilde{\cal{A}}_{3,q}^{1}(s_{14}) 
 -\frac{1}{2}\,\,{\cal A}_{3,q}^{0}(s_{14})\otimes{\cal A}_{3,q}^{0}(s_{14}) 
 \bigg] 
 B_1^{\gamma,0}(4,3,1,5,2)
 \nonumber\\
\end{eqnarray}


==> sub/autoqbB2g0AS.tex <==
\section*{qbB2g0AS(k,j,i,1,6,2)}
\begin{eqnarray}
\lefteqn{{\tt qbB2g0AS(k,j,i,1,6,2) =}} \\
 \ph{1}&&+d_{3,q}^{0}(1,i,j)\,B_1^{\gamma,0}(k,(\widetilde{ij}),\overline{1},6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{2}&&+d_3^{0}(k,j,i)\,B_1^{\gamma,0}((\widetilde{kj}),(\widetilde{ij}),1,6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\end{eqnarray}


==> sub/autoqbB2g1AT.tex <==
\section*{qbB2g1AT(k,j,i,1,6,2)}
\begin{eqnarray}
 \ph{1}&&-\bigg[ 
 +J_{2,QG}^{1,IF}(s_{1i})
 +J_{2,GG}^{1,FF}(s_{ij})
 +J_{2,QG}^{1,FF}(s_{kj})\bigg]\,B_2^{\gamma,0}(k,j,i,1,6,2)\,J_2^{(3)}(\lbrace p\rbrace_{3})\nonumber\\
 \ph{2}&&-\bigg[ 
 +J_{2,QG}^{1,FF}(s_{ki})
 +J_{2,QG}^{1,IF}(s_{1j})
 +J_{2,GG}^{1,FF}(s_{ji})\bigg]\,B_2^{\gamma,0}(k,i,j,1,6,2)\,J_2^{(3)}(\lbrace p\rbrace_{3})\nonumber\\
  \ph{3}&&+\,D_{3,q}^{0}(1,i,j)\,\bigg[\,B_1^{\gamma,1}(k,(\widetilde{ij}),\overline{1},6,2)\,\delta(1-x_1)\,\delta(1-x_2)\nonumber\\
  &&+\,\bigg( 
 +J_{2,QG}^{1,IF}(s_{\overline{1}(\widetilde{ij})})
 +J_{2,QG}^{1,FF}(s_{k(\widetilde{ij})})\bigg)\,B_1^{\gamma,0}(k,(\widetilde{ij}),\overline{1},6,2) \bigg]\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
  \ph{4}&&+\,d_3^{0}(k,j,i)\,\bigg[\,B_1^{\gamma,1}((\widetilde{kj}),(\widetilde{ij}),1,6,2)\,\delta(1-x_1)\,\delta(1-x_2)\nonumber\\
  &&+\,\bigg( 
 +J_{2,QG}^{1,IF}(s_{1(\widetilde{ij})})
 +J_{2,QG}^{1,FF}(s_{(\widetilde{kj})(\widetilde{ij})})\bigg)\,B_1^{\gamma,0}((\widetilde{kj}),(\widetilde{ij}),1,6,2) \bigg]\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
  \ph{5}&&+\,d_3^{0}(k,i,j)\,\bigg[\,B_1^{\gamma,1}((\widetilde{ki}),(\widetilde{ij}),1,6,2)\,\delta(1-x_1)\,\delta(1-x_2)\nonumber\\
  &&+\,\bigg( 
 +J_{2,QG}^{1,FF}(s_{(\widetilde{ki})(\widetilde{ij})})
 +J_{2,QG}^{1,IF}(s_{1(\widetilde{ij})})\bigg)\,B_1^{\gamma,0}((\widetilde{ki}),(\widetilde{ij}),1,6,2) \bigg]\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
  \ph{6}&&+\bigg[\,d_{3}^{1}(k,i,j)\,\delta(1-x_1)\,\delta(1-x_2)
  \nonumber\\&&\,  
   +\bigg( 
 +J_{2,QG}^{1,FF}(s_{kj})
 +J_{2,QG}^{1,FF}(s_{ki})
 +J_{2,GG}^{1,FF}(s_{ij})
 -2J_{2,QG}^{1,FF}(s_{(\widetilde{ki})(\widetilde{ij})})\bigg)\,d_3^{0}(k,i,j)\bigg]\,B_1^{\gamma,0}((\widetilde{ki}),(\widetilde{ij}),1,6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
  \ph{7}&&+\bigg[\,d_{3}^{1}(k,j,i)\,\delta(1-x_1)\,\delta(1-x_2)
  \nonumber\\&&\,  
   +\bigg( 
 -2J_{2,QG}^{1,FF}(s_{(\widetilde{kj})(\widetilde{ij})})
 +J_{2,QG}^{1,FF}(s_{kj})
 +J_{2,QG}^{1,FF}(s_{ki})
 +J_{2,GG}^{1,FF}(s_{ij})\bigg)\,d_3^{0}(k,j,i)\bigg]\,B_1^{\gamma,0}((\widetilde{kj}),(\widetilde{ij}),1,6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
  \ph{8}&&+\bigg[\,D_{3,q}^{1}(1,i,j)\,\delta(1-x_1)\,\delta(1-x_2)
  \nonumber\\&&\,  
   +\bigg( 
 +J_{2,QG}^{1,IF}(s_{1i})
 +J_{2,QG}^{1,IF}(s_{1j})
 -2J_{2,QG}^{1,IF}(s_{\overline{1}(\widetilde{ij})})
 +J_{2,GG}^{1,FF}(s_{ij})\bigg)\,D_3^{0}(1,i,j)\bigg]\,B_1^{\gamma,0}(k,(\widetilde{ij}),\overline{1},6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
  \ph{9}&&-\bigg[\,\tilde{A}_{3,q}^{1}(1,i,k)\,\delta(1-x_1)\,\delta(1-x_2)
  \nonumber\\&&\,  
   +\bigg( 
 +J_{2,QQ}^{1,IF}(s_{1k})
 -J_{2,QQ}^{1,IF}(s_{\overline{1}(\widetilde{ik})})\bigg)\,A_3^{0}(1,i,k)\bigg]\,B_1^{\gamma,0}((\widetilde{ki}),j,\overline{1},6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
  \ph{10}&&-\bigg[\,\tilde{A}_{3,q}^{1}(1,j,k)\,\delta(1-x_1)\,\delta(1-x_2)
  \nonumber\\&&\,  
   +\bigg( 
 +J_{2,QQ}^{1,IF}(s_{1k})
 -J_{2,QQ}^{1,IF}(s_{\overline{1}(\widetilde{jk})})\bigg)\,A_3^{0}(1,j,k)\bigg]\,B_1^{\gamma,0}((\widetilde{kj}),i,\overline{1},6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
 \ph{11}&&-\frac{1}{2}\,\bigg[ +J_{2,QG}^{1,IF}(s_{1j})
 -J_{2,QG}^{1,IF}(s_{\overline{1}(\widetilde{ij})})
 -J_{2,QG}^{1,FF}(s_{kj})
 +J_{2,QG}^{1,FF}(s_{k(\widetilde{ij})})
 -J_{2,QQ}^{1,IF}(s_{1k})
 +J_{2,QQ}^{1,IF}(s_{\overline{1}k})
 \nonumber\\&&\phantom{-\frac{1}{2}\,} \nonumber\\ &&+\bigg(  -{\cal S}^{FF}(s_{1j},s_{kj},x_{1j,kj})
 +{\cal S}^{FF}(s_{\overline{1}(\widetilde{ij})},s_{kj},x_{\overline{1}(\widetilde{ij}),kj})
 +{\cal S}^{FF}(s_{kj},s_{kj},1)
 -{\cal S}^{FF}(s_{k(\widetilde{ij})},s_{kj},x_{k(\widetilde{ij}),kj})
 \nonumber\\&&\phantom{-\frac{1}{2}\,} +{\cal S}^{FF}(s_{1k},s_{kj},x_{1k,kj})
 -{\cal S}^{FF}(s_{\overline{1}k},s_{kj},x_{\overline{1}k,kj})
 \bigg)\bigg]\nonumber\\
 &&\times d_3^{0}(1,i,j)\,B_1^{\gamma,0}(k,(\widetilde{ij}),\overline{1},6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{12}&&+\frac{1}{2}\,\bigg[ +J_{2,QQ}^{1,IF}(s_{1k})
 -J_{2,QQ}^{1,IF}(s_{\overline{1}k})
 -J_{2,QG}^{1,IF}(s_{1i})
 +J_{2,QG}^{1,IF}(s_{\overline{1}(\widetilde{ji})})
 +J_{2,QG}^{1,FF}(s_{ki})
 -J_{2,QG}^{1,FF}(s_{k(\widetilde{ji})})
 \nonumber\\&&\phantom{+\frac{1}{2}\,} \nonumber\\ &&+\bigg(  +{\cal S}^{FF}(s_{1i},s_{ki},x_{1i,ki})
 -{\cal S}^{FF}(s_{\overline{1}(\widetilde{ji})},s_{ki},x_{\overline{1}(\widetilde{ji}),ki})
 -{\cal S}^{FF}(s_{ki},s_{ki},1)
 +{\cal S}^{FF}(s_{k(\widetilde{ji})},s_{ki},x_{k(\widetilde{ji}),ki})
 \nonumber\\&&\phantom{+\frac{1}{2}\,} -{\cal S}^{FF}(s_{1k},s_{ki},x_{1k,ki})
 +{\cal S}^{FF}(s_{\overline{1}k},s_{ki},x_{\overline{1}k,ki})
 \bigg)\bigg]\nonumber\\
 &&\times d_3^{0}(1,j,i)\,B_1^{\gamma,0}(k,(\widetilde{ij}),\overline{1},6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{13}&&+\frac{1}{2}\,\bigg[ +J_{2,QQ}^{1,IF}(s_{1k})
 -J_{2,QQ}^{1,IF}(s_{1(\widetilde{ki})})
 +J_{2,QG}^{1,FF}(s_{(\widetilde{ki})(\widetilde{ij})})
 +J_{2,QG}^{1,IF}(s_{1j})
 -J_{2,QG}^{1,IF}(s_{1(\widetilde{ij})})
 -J_{2,QG}^{1,FF}(s_{kj})
 \nonumber\\&&\phantom{+\frac{1}{2}\,} \nonumber\\ &&+\bigg(  +{\cal S}^{FF}(s_{kj},s_{kj},1)
 -{\cal S}^{FF}(s_{(\widetilde{ki})(\widetilde{ij})},s_{kj},x_{(\widetilde{ki})(\widetilde{ij}),kj})
 -{\cal S}^{FF}(s_{1j},s_{kj},x_{1j,kj})
 +{\cal S}^{FF}(s_{1(\widetilde{ij})},s_{kj},x_{1(\widetilde{ij}),kj})
 \nonumber\\&&\phantom{+\frac{1}{2}\,} -{\cal S}^{FF}(s_{1k},s_{kj},x_{1k,kj})
 +{\cal S}^{FF}(s_{1(\widetilde{ki})},s_{kj},x_{1(\widetilde{ki}),kj})
 \bigg)\bigg]\nonumber\\
 &&\times d_3^{0}(k,i,j)\,B_1^{\gamma,0}(1,(\widetilde{ij}),(\widetilde{ki}),6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{14}&&+\frac{1}{2}\,\bigg[ +J_{2,QQ}^{1,IF}(s_{1k})
 -J_{2,QQ}^{1,IF}(s_{1(\widetilde{kj})})
 -J_{2,QG}^{1,FF}(s_{ki})
 +J_{2,QG}^{1,FF}(s_{(\widetilde{kj})(\widetilde{ji})})
 +J_{2,QG}^{1,IF}(s_{1i})
 -J_{2,QG}^{1,IF}(s_{1(\widetilde{ji})})
 \nonumber\\&&\phantom{+\frac{1}{2}\,} \nonumber\\ &&+\bigg(  +{\cal S}^{FF}(s_{ki},s_{ki},1)
 -{\cal S}^{FF}(s_{(\widetilde{kj})(\widetilde{ji})},s_{ki},x_{(\widetilde{kj})(\widetilde{ji}),ki})
 -{\cal S}^{FF}(s_{1i},s_{ki},x_{1i,ki})
 +{\cal S}^{FF}(s_{1(\widetilde{ji})},s_{ki},x_{1(\widetilde{ji}),ki})
 \nonumber\\&&\phantom{+\frac{1}{2}\,} -{\cal S}^{FF}(s_{1k},s_{ki},x_{1k,ki})
 +{\cal S}^{FF}(s_{1(\widetilde{kj})},s_{ki},x_{1(\widetilde{kj}),ki})
 \bigg)\bigg]\nonumber\\
 &&\times d_3^{0}(k,j,i)\,B_1^{\gamma,0}((\widetilde{kj}),(\widetilde{ji}),1,6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{15}&&+\frac{1}{2}\,\bigg[ +J_{2,QQ}^{1,IF}(s_{1k})
 -J_{2,QQ}^{1,IF}(s_{\overline{1}(\widetilde{ki})})
 -J_{2,QG}^{1,IF}(s_{1j})
 +J_{2,QG}^{1,IF}(s_{\overline{1}j})
 -J_{2,QG}^{1,FF}(s_{kj})
 +J_{2,QG}^{1,FF}(s_{(\widetilde{ki})j})
 \nonumber\\&&\phantom{+\frac{1}{2}\,} \nonumber\\ &&+\bigg(  -{\cal S}^{FF}(s_{1k},s_{kj},x_{1k,kj})
 +{\cal S}^{FF}(s_{\overline{1}(\widetilde{ki})},s_{kj},x_{\overline{1}(\widetilde{ki}),kj})
 +{\cal S}^{FF}(s_{1j},s_{kj},x_{1j,kj})
 -{\cal S}^{FF}(s_{\overline{1}j},s_{kj},x_{\overline{1}j,kj})
 \nonumber\\&&\phantom{+\frac{1}{2}\,} +{\cal S}^{FF}(s_{kj},s_{kj},1)
 -{\cal S}^{FF}(s_{(\widetilde{ki})j},s_{kj},x_{(\widetilde{ki})j,kj})
 \bigg)\bigg]\nonumber\\
 &&\times A_3^{0}(1,i,k)\,B_1^{\gamma,0}((\widetilde{ki}),j,\overline{1},6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{16}&&-\frac{1}{2}\,\bigg[ +J_{2,QG}^{1,IF}(s_{1i})
 -J_{2,QG}^{1,IF}(s_{\overline{1}i})
 +J_{2,QG}^{1,FF}(s_{ki})
 -J_{2,QG}^{1,FF}(s_{(\widetilde{kj})i})
 -J_{2,QQ}^{1,IF}(s_{1k})
 +J_{2,QQ}^{1,IF}(s_{\overline{1}(\widetilde{kj})})
 \nonumber\\&&\phantom{-\frac{1}{2}\,} \nonumber\\ &&+\bigg(  +{\cal S}^{FF}(s_{1k},s_{ki},x_{1k,ki})
 -{\cal S}^{FF}(s_{\overline{1}(\widetilde{kj})},s_{ki},x_{\overline{1}(\widetilde{kj}),ki})
 -{\cal S}^{FF}(s_{1i},s_{ki},x_{1i,ki})
 +{\cal S}^{FF}(s_{\overline{1}i},s_{ki},x_{\overline{1}i,ki})
 \nonumber\\&&\phantom{-\frac{1}{2}\,} -{\cal S}^{FF}(s_{ki},s_{ki},1)
 +{\cal S}^{FF}(s_{(\widetilde{kj})i},s_{ki},x_{(\widetilde{kj})i,ki})
 \bigg)\bigg]\nonumber\\
 &&\times A_3^{0}(1,j,k)\,B_1^{\gamma,0}((\widetilde{kj}),i,\overline{1},6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\end{eqnarray}


==> sub/autoqbB3g0AS.tex <==
\section*{qbB3g0AS(l,k,j,i,1,7,2)}
\begin{eqnarray}
\lefteqn{{\tt qbB3g0AS(l,k,j,i,1,7,2) =}} \\
 \ph{1}&&+f_3^{0}(i,j,k)\,B_2^{\gamma,0}(l,(\widetilde{jk}),(\widetilde{ij}),1,7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{2}&&+f_3^{0}(i,j,k)\,B_2^{\gamma,0}(l,(\widetilde{ij}),(\widetilde{jk}),1,7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{3}&&+d_3^{0}(l,k,j)\,B_2^{\gamma,0}((\widetilde{lk}),(\widetilde{jk}),i,1,7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{4}&&+d_3^{0}(l,i,j)\,B_2^{\gamma,0}((\widetilde{li}),(\widetilde{ji}),k,1,7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{5}&&+d_3^{0}(1,k,j)\,B_2^{\gamma,0}(l,i,(\widetilde{kj}),\overline{1},7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{6}&&+d_3^{0}(1,i,j)\,B_2^{\gamma,0}(l,k,(\widetilde{ij}),\overline{1},7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
\snip \ph{7}&&+\,D_4^{0,a}(l,i,j,k)\,B_1^{\gamma,0}((\widetilde{lij}),(\widetilde{ijk}),1,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{8}&&-\,d_3^{0}(l,i,j)\,d_3^{0}((\widetilde{li}),(\widetilde{ij}),k)\,B_1^{\gamma,0}([(\widetilde{li}), (\widetilde{ij})],(\widetilde{k\widetilde{(ij})}),1,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{9}&&-\,f_3^{0}(k,j,i)\,d_3^{0}(l,(\widetilde{kj}),(\widetilde{ji}))\,B_1^{\gamma,0}((\widetilde{l\widetilde{(kj})}),[(\widetilde{kj}), (\widetilde{ji})],1,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\snip \ph{10}&&+\,D_4^{0,a}(l,k,j,i)\,B_1^{\gamma,0}((\widetilde{lkj}),(\widetilde{kji}),1,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{11}&&-\,d_3^{0}(l,k,j)\,d_3^{0}((\widetilde{lk}),(\widetilde{kj}),i)\,B_1^{\gamma,0}([(\widetilde{lk}), (\widetilde{kj})],(\widetilde{i\widetilde{(kj})}),1,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{12}&&-\,f_3^{0}(i,j,k)\,d_3^{0}(l,(\widetilde{ij}),(\widetilde{jk}))\,B_1^{\gamma,0}((\widetilde{l\widetilde{(ij})}),[(\widetilde{ij}), (\widetilde{jk})],1,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\snip \ph{13}&&+\,D_4^0(1,i,j,k)\,B_1^{\gamma,0}(l,(\widetilde{ijk}),\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{14}&&-\,d_3^{0}(1,i,j)\,D_3^{0}(\overline{1},k,(\widetilde{ij}))\,B_1^{\gamma,0}(l,(\widetilde{(\widetilde{ij})k}),\overline{\overline{1}},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{15}&&-\,d_3^{0}(1,k,j)\,D_3^{0}(\overline{1},i,(\widetilde{kj}))\,B_1^{\gamma,0}(l,(\widetilde{(\widetilde{kj})i}),\overline{\overline{1}},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{16}&&-\,f_3^{0}(i,j,k)\,D_3^{0}(1,(\widetilde{ij}),(\widetilde{kj}))\,B_1^{\gamma,0}(l,[(\widetilde{ij}), (\widetilde{kj})],\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\snip \ph{17}&&+\,D_4^{0,c}(l,k,i,j)\,B_1^{\gamma,0}((\widetilde{lki}),(\widetilde{jik}),1,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\snip \ph{18}&&+\,D_4^{0,c}(l,i,k,j)\,B_1^{\gamma,0}((\widetilde{lik}),(\widetilde{jki}),1,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{19}&&-\,d_3^{0}(l,k,j)\,d_3^{0}((\widetilde{lk}),i,(\widetilde{kj}))\,B_1^{\gamma,0}((\widetilde{i\widetilde{(lk})}),(\widetilde{i\widetilde{(kj})}),1,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{20}&&-\,d_3^{0}(l,i,j)\,d_3^{0}((\widetilde{li}),k,(\widetilde{ij}))\,B_1^{\gamma,0}((\widetilde{k\widetilde{(li})}),(\widetilde{k\widetilde{(ij})}),1,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\snip \ph{21}&&-\,\tilde{A}_4^0(1,i,k,l)\,B_1^{\gamma,0}((\widetilde{lki}),j,\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{22}&&+\,A_3^{0}(1,i,l)\,A_3^{0}(\overline{1},k,(\widetilde{li}))\,B_1^{\gamma,0}((\widetilde{k\widetilde{(li})}),j,\overline{\overline{1}},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{23}&&+\,A_3^{0}(1,k,l)\,A_3^{0}(\overline{1},i,(\widetilde{lk}))\,B_1^{\gamma,0}((\widetilde{i\widetilde{(lk})}),j,\overline{\overline{1}},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{24}&&+\frac{1}{2}\,\,d_3^{0}(1,i,j)\,d_3^{0}(\overline{1},k,(\widetilde{ij}))\,B_1^{\gamma,0}(l,(\widetilde{k\widetilde{(ij})}),\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{25}&&-\frac{1}{2}\,\,d_3^{0}(l,i,j)\,d_3^{0}(1,k,(\widetilde{ij}))\,B_1^{\gamma,0}((\widetilde{li}),(\widetilde{k\widetilde{(ij})}),\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{26}&&-\frac{1}{2}\,\,A_3^{0}(1,i,l)\,d_3^{0}(\overline{1},k,j)\,B_1^{\gamma,0}((\widetilde{li}),(\widetilde{kj}),\overline{\overline{1}},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{27}&&-\frac{1}{2}\,\bigg[      +S^{FF}_{1i(\widetilde{ij})}       -S^{FF}_{\overline{1}i(\widetilde{k\widetilde{(ij})})}       -S^{FF}_{(\widetilde{li})i(\widetilde{ij})}       +S^{FF}_{(\widetilde{li})i(\widetilde{k\widetilde{(ij})})}       -S^{FF}_{1i(\widetilde{li})}       +S^{FF}_{\overline{1}i(\widetilde{li})}  \bigg]\nonumber\\
 &&\times d_3^{0}(1,k,(\widetilde{ij}))\,B_1^{\gamma,0}((\widetilde{li}),(\widetilde{k\widetilde{(ij})}),\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{28}&&+\frac{1}{2}\,\,d_3^{0}(1,k,j)\,d_3^{0}(\overline{1},i,(\widetilde{kj}))\,B_1^{\gamma,0}(l,(\widetilde{i\widetilde{(kj})}),\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{29}&&-\frac{1}{2}\,\,d_3^{0}(l,k,j)\,d_3^{0}(1,i,(\widetilde{kj}))\,B_1^{\gamma,0}((\widetilde{lk}),(\widetilde{i\widetilde{(kj})}),\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{30}&&-\frac{1}{2}\,\,A_3^{0}(1,k,l)\,d_3^{0}(\overline{1},i,j)\,B_1^{\gamma,0}((\widetilde{lk}),(\widetilde{ij}),\overline{\overline{1}},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{31}&&-\frac{1}{2}\,\bigg[      +S^{FF}_{1k(\widetilde{jk})}       -S^{FF}_{\overline{1}k(\widetilde{i\widetilde{(jk})})}       -S^{FF}_{(\widetilde{lk})k(\widetilde{jk})}       +S^{FF}_{(\widetilde{lk})k(\widetilde{i\widetilde{(jk})})}       -S^{FF}_{1k(\widetilde{lk})}       +S^{FF}_{\overline{1}k(\widetilde{lk})}  \bigg]\nonumber\\
 &&\times d_3^{0}(1,i,(\widetilde{jk}))\,B_1^{\gamma,0}((\widetilde{lk}),(\widetilde{i\widetilde{(jk})}),\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{32}&&+\frac{1}{2}\,\,d_3^{0}(l,i,j)\,d_3^{0}((\widetilde{li}),k,(\widetilde{ij}))\,B_1^{\gamma,0}((\widetilde{(\widetilde{li})k}),(\widetilde{k\widetilde{(ij})}),1,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{33}&&-\frac{1}{2}\,\,d_3^{0}(1,i,j)\,d_3^{0}(l,k,(\widetilde{ij}))\,B_1^{\gamma,0}((\widetilde{lk}),(\widetilde{k\widetilde{(ij})}),\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{34}&&-\frac{1}{2}\,\,A_3^{0}(1,i,l)\,d_3^{0}((\widetilde{li}),k,j)\,B_1^{\gamma,0}((\widetilde{k\widetilde{(li})}),(\widetilde{kj}),\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{35}&&-\frac{1}{2}\,\bigg[      +S^{FF}_{(\widetilde{ij})i(\widetilde{li})}       -S^{FF}_{(\widetilde{k\widetilde{(ij})})i(\widetilde{k\widetilde{(li})})}       -S^{FF}_{1i(\widetilde{ij})}       +S^{FF}_{1i(\widetilde{k\widetilde{(ij})})}       -S^{FF}_{1i(\widetilde{li})}       +S^{FF}_{1i(\widetilde{k\widetilde{(li})})}  \bigg]\nonumber\\
 &&\times d_3^{0}((\widetilde{li}),k,(\widetilde{ij}))\,B_1^{\gamma,0}((\widetilde{k\widetilde{(li})}),(\widetilde{k\widetilde{(ij})}),1,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{36}&&+\frac{1}{2}\,\,d_3^{0}(l,k,j)\,d_3^{0}((\widetilde{lk}),i,(\widetilde{kj}))\,B_1^{\gamma,0}((\widetilde{(\widetilde{lk})i}),(\widetilde{i\widetilde{(kj})}),1,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{37}&&-\frac{1}{2}\,\,d_3^{0}(1,k,j)\,d_3^{0}(l,i,(\widetilde{kj}))\,B_1^{\gamma,0}((\widetilde{li}),(\widetilde{i\widetilde{(kj})}),\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{38}&&-\frac{1}{2}\,\,A_3^{0}(1,k,l)\,d_3^{0}((\widetilde{lk}),i,j)\,B_1^{\gamma,0}((\widetilde{i\widetilde{(lk})}),(\widetilde{ij}),\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{39}&&-\frac{1}{2}\,\bigg[      +S^{FF}_{(\widetilde{kj})k(\widetilde{lk})}       -S^{FF}_{(\widetilde{i\widetilde{(kj})})k(\widetilde{i\widetilde{(lk})})}       -S^{FF}_{1k(\widetilde{kj})}       +S^{FF}_{1k(\widetilde{i\widetilde{(kj})})}       -S^{FF}_{1k(\widetilde{lk})}       +S^{FF}_{1k(\widetilde{i\widetilde{(lk})})}  \bigg]\nonumber\\
 &&\times d_3^{0}((\widetilde{lk}),i,(\widetilde{kj}))\,B_1^{\gamma,0}((\widetilde{i\widetilde{(lk})}),(\widetilde{i\widetilde{(kj})}),1,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{40}&&-\frac{1}{2}\,\,A_3^{0}(1,i,l)\,A_3^{0}(\overline{1},k,(\widetilde{li}))\,B_1^{\gamma,0}((\widetilde{k\widetilde{(li})}),j,\overline{\overline{1}},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{41}&&+\frac{1}{2}\,\,d_3^{0}(1,i,j)\,A_3^{0}(\overline{1},k,l)\,B_1^{\gamma,0}((\widetilde{lk}),(\widetilde{ij}),\overline{\overline{1}},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{42}&&+\frac{1}{2}\,\,d_3^{0}(l,i,j)\,A_3^{0}(1,k,(\widetilde{li}))\,B_1^{\gamma,0}((\widetilde{(\widetilde{li})k}),(\widetilde{ij}),\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{43}&&-\frac{1}{2}\,\bigg[      -S^{FF}_{1i(\widetilde{li})}       +S^{FF}_{\overline{1}i(\widetilde{k\widetilde{(li})})}       +S^{FF}_{(\widetilde{li})i(\widetilde{ij})}       -S^{FF}_{(\widetilde{k\widetilde{(li})})i(\widetilde{ij})}       +S^{FF}_{1i(\widetilde{ij})}       -S^{FF}_{\overline{1}i(\widetilde{ij})}  \bigg]\nonumber\\
 &&\times A_3^{0}(1,k,(\widetilde{li}))\,B_1^{\gamma,0}((\widetilde{k\widetilde{(li})}),(\widetilde{ij}),\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{44}&&-\frac{1}{2}\,\,A_3^{0}(1,k,l)\,A_3^{0}(\overline{1},i,(\widetilde{lk}))\,B_1^{\gamma,0}((\widetilde{i\widetilde{(lk})}),j,\overline{\overline{1}},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{45}&&+\frac{1}{2}\,\,d_3^{0}(1,k,j)\,A_3^{0}(\overline{1},i,l)\,B_1^{\gamma,0}((\widetilde{li}),(\widetilde{kj}),\overline{\overline{1}},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{46}&&+\frac{1}{2}\,\,d_3^{0}(l,k,j)\,A_3^{0}(1,i,(\widetilde{lk}))\,B_1^{\gamma,0}((\widetilde{(\widetilde{lk})i}),(\widetilde{kj}),\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{47}&&-\frac{1}{2}\,\bigg[      -S^{FF}_{1k(\widetilde{lk})}       +S^{FF}_{\overline{1}k(\widetilde{i\widetilde{(lk})})}       +S^{FF}_{(\widetilde{lk})k(\widetilde{kj})}       -S^{FF}_{(\widetilde{i\widetilde{(lk})})k(\widetilde{kj})}       +S^{FF}_{1k(\widetilde{kj})}       -S^{FF}_{\overline{1}k(\widetilde{kj})}  \bigg]\nonumber\\
 &&\times A_3^{0}(1,i,(\widetilde{lk}))\,B_1^{\gamma,0}((\widetilde{i\widetilde{(lk})}),(\widetilde{kj}),\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\end{eqnarray}


==> sub/autoqbBh1g1AT.tex <==
\section*{qbBh1g1AT(j,i,1,5,2)}
\begin{eqnarray}
  \ph{1}&&-2\hat{J}_{2,QG}^{1,FF}(s_{ij})\,B_1^{\gamma,0}(j,i,1,5,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
\end{eqnarray}


==> sub/autoqbBh1g1ATqtog.tex <==
\section*{qbBh1g1ATqtog(1,i,j,5,2)}
\begin{eqnarray}
  \ph{1}&&-\frac{1}{2}\,J_{2,GQ,q^\prime \to g}^{1,IF}(s_{i1})\,B_1^{\gamma,0}(j,1,i,5,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
  \ph{2}&&-\frac{1}{2}\,J_{2,GQ,q^\prime \to g}^{1,IF}(s_{j1})\,B_1^{\gamma,0}(j,1,i,5,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
\end{eqnarray}


==> sub/autoqbBh1g2AU.tex <==
\section*{qbBh1g2AU}
\begin{eqnarray}
\lefteqn{{\tt qbBh1g2AU(4,3,1,5,2) =}} \\
 \ph{1}&&+\bigg[ 
 -\frac{1}{2}\,\,{\cal D}_{3}^{0}(s_{34}) 
 -\frac{1}{2}\,\,{\cal D}_{3,q}^{0}(s_{13}) 
 +\,\Gamma^{(1)}_{qq}(z_1) 
 \bigg] 
\left( -\frac{b_F}{\epsilon}B_1^{\gamma,0}(4,3,1,5,2) +\hat{B}_1^{\gamma,1}(4,3,1,5,2)\right)
 \nonumber\\
 \ph{2}&&+\bigg[ 
 -\frac{1}{2}\,\,{\cal E}_{3}^{0}(s_{34}) 
 -\frac{1}{2}\,\,{\cal E}_{3,q}^{0}(s_{13}) 
 \bigg] 
\left( -\frac{b_0}{\epsilon}B_1^{\gamma,0}(4,3,1,5,2) +B_1^{\gamma,1}(4,3,1,5,2)\right)
 \nonumber\\
 \ph{3}&&+\bigg[ 
 -\frac{1}{4}\,\,{\cal D}_{3}^{0}(s_{34})\otimes{\cal E}_{3}^{0}(s_{34}) 
 -\frac{1}{4}\,\,{\cal D}_{3}^{0}(s_{34})\otimes{\cal E}_{3,q}^{0}(s_{13}) 
 -\frac{1}{4}\,\,{\cal D}_{3,q}^{0}(s_{13})\otimes{\cal E}_{3}^{0}(s_{34}) 
 \nonumber \\ && \phantom{+\bigg[} 
 -\frac{1}{4}\,\,{\cal D}_{3,q}^{0}(s_{13})\otimes{\cal E}_{3,q}^{0}(s_{13}) 
 +\frac{1}{2}\,\,\Gamma^{(1)}_{qq}(z_1)\otimes{\cal E}_{3}^{0}(s_{34}) 
 +\frac{1}{2}\,\,\Gamma^{(1)}_{qq}(z_1)\otimes{\cal E}_{3,q}^{0}(s_{13}) 
 \bigg] 
 B_1^{\gamma,0}(4,3,1,5,2)
 \nonumber\\
 \ph{4}&&+\bigg[ 
 -\frac{b_0}{2\epsilon}\,\bigg( \frac{s_{34}}{\mu_R^2}\bigg)^{-\epsilon}\,{\cal E}_{3}^{0}(s_{34}) 
 -\frac{b_F}{2\epsilon}\,\bigg( \frac{s_{34}}{\mu_R^2}\bigg)^{-\epsilon}\,{\cal D}_{3}^{0}(s_{34}) 
 +\frac{1}{2}\,\,{\cal D}_{3}^{0}(s_{34})\otimes{\cal E}_{3}^{0}(s_{34}) 
 \nonumber \\ && \phantom{+\bigg[} 
 -\,{\cal E}_{4}^{0}(s_{34}) 
 -\frac{1}{2}\,\,{\cal{E}}_{3}^{1}(s_{34}) 
 -\frac{1}{2}\,\,\hat{\cal{D}}_{3}^{1}(s_{34}) 
 \bigg] 
 B_1^{\gamma,0}(4,3,1,5,2)
 \nonumber\\
 \ph{5}&&+\bigg[ 
 -\frac{b_0}{2\epsilon}\,\bigg( \frac{s_{13}}{\mu_R^2}\bigg)^{-\epsilon}\,{\cal E}_{3,q}^{0}(s_{13}) 
 -\frac{b_F}{2\epsilon}\,\bigg( \frac{s_{13}}{\mu_R^2}\bigg)^{-\epsilon}\,{\cal D}_{3,q}^{0}(s_{13}) 
 +\frac{1}{2}\,\,{\cal D}_{3,q}^{0}(s_{13})\otimes{\cal E}_{3,q}^{0}(s_{13}) 
 \nonumber \\ && \phantom{+\bigg[} 
 -\,{\cal E}_{4,q}^{0}(s_{13}) 
 -\frac{1}{2}\,\,{\cal{E}}_{3,q}^{1}(s_{13}) 
 -\frac{1}{2}\,\,\hat{\cal{D}}_{3,q}^{1}(s_{13}) 
 \nonumber \\ && \phantom{+\bigg[} 
 +\,\Gamma^{(2)}_{qq,F}(z_1) 
 \bigg] 
 B_1^{\gamma,0}(4,3,1,5,2)
 \nonumber\\
\end{eqnarray}


==> sub/autoqbBh2g1AT.tex <==
\section*{qbBh2g1AT(k,j,i,1,6,2)}
\begin{eqnarray}
 \ph{1}&&-\bigg[ 
 +2\hat{J}_{2,QG}^{1,FF}(s_{ki})
 +2\hat{J}_{2,QG}^{1,FF}(s_{kj})\bigg]\,B_2^{\gamma,0}(k,j,i,1,6,2)\,J_2^{(3)}(\lbrace p\rbrace_{3})\nonumber\\
  \ph{2}&&+\,d_3^{0}(1,i,j)\,\bigg[\,\hat{B}_1^{\gamma,1}(k,(\widetilde{ij}),\overline{1},6,2)\,\delta(1-x_1)\,\delta(1-x_2)\nonumber\\
  &&+\,\bigg( 
 +\hat{J}_{2,QG}^{1,IF}(s_{\overline{1}(\widetilde{ij})})
 +\hat{J}_{2,QG}^{1,FF}(s_{k(\widetilde{ij})})\bigg)\,B_1^{\gamma,0}(k,(\widetilde{ij}),\overline{1},6,2) \bigg]\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
  \ph{3}&&+\,d_3^{0}(k,j,i)\,\bigg[\,\hat{B}_1^{\gamma,1}((\widetilde{kj}),(\widetilde{ij}),1,6,2)\,\delta(1-x_1)\,\delta(1-x_2)\nonumber\\
  &&+\,\bigg( 
 +\hat{J}_{2,QG}^{1,IF}(s_{1(\widetilde{ij})})
 +\hat{J}_{2,QG}^{1,FF}(s_{(\widetilde{kj})(\widetilde{ij})})\bigg)\,B_1^{\gamma,0}((\widetilde{kj}),(\widetilde{ij}),1,6,2) \bigg]\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
  \ph{4}&&+\bigg[\,\hat{d}_{3}^{1}(1,i,j)\,\delta(1-x_1)\,\delta(1-x_2)
  \nonumber\\&&\,  
   +\bigg( 
 +4\hat{J}_{2,QG}^{1,IF}(s_{1i})
 -\hat{J}_{2,QG}^{1,IF}(s_{\overline{1}(\widetilde{ij})})
 -\hat{J}_{2,QG}^{1,FF}(s_{k(\widetilde{ij})})\bigg)\,d_3^{0}(1,i,j)\bigg]\,B_1^{\gamma,0}(k,(\widetilde{ji}),\overline{1},6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
  \ph{5}&&+\bigg[\,\hat{d}_{3}^{1}(k,j,i)\,\delta(1-x_1)\,\delta(1-x_2)
  \nonumber\\&&\,  
   +\bigg( 
 +4\hat{J}_{2,QG}^{1,FF}(s_{kj})
 -\hat{J}_{2,QG}^{1,FF}(s_{(\widetilde{kj})(\widetilde{ji})})
 -\hat{J}_{2,QG}^{1,IF}(s_{1(\widetilde{ij})})\bigg)\,d_3^{0}(k,j,i)\bigg]\,B_1^{\gamma,0}((\widetilde{kj}),(\widetilde{ji}),1,6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
 \ph{6}&&+\bigg[ -4\hat{J}_{2,QG}^{1,IF}(s_{1i})
 +2\hat{J}_{2,QG}^{1,FF}(s_{kj})
 +2\hat{J}_{2,QG}^{1,FF}(s_{ki})
\bigg]  d_3^{0}(1,i,j)\,B_1^{\gamma,0}(k,(\widetilde{ji}),\overline{1},6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})  \nonumber\\
 \ph{7}&&+\bigg[ -2\hat{J}_{2,QG}^{1,FF}(s_{kj})
 +2\hat{J}_{2,QG}^{1,FF}(s_{ki})
\bigg]  d_3^{0}(k,j,i)\,B_1^{\gamma,0}((\widetilde{kj}),(\widetilde{ji}),1,6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})  \nonumber\\
\end{eqnarray}


==> sub/autoqbBh2g1ATqtog.tex <==
\section*{qbBh2g1ATqtog(1,i,j,k,6,2)}
\begin{eqnarray}
  \ph{1}&&-2J_{2,GQ,q^\prime \to g}^{1,IF}(s_{1k})\,B_2^{\gamma,0}(j,i,1,k,6,2)\,J_2^{(3)}(\lbrace p\rbrace_{3})\nonumber\\
  \ph{2}&&-2J_{2,GQ,q^\prime \to g}^{1,IF}(s_{1k})\,B_2^{\gamma,0}(j,1,i,k,6,2)\,J_2^{(3)}(\lbrace p\rbrace_{3})\nonumber\\
 \ph{3}&& +4J_{2,GQ,q^\prime \to g}^{1,IF}(s_{1k})
\,D_3^{0}(k,1,i)\,B_1^{\gamma,0}(j,\overline{1},(\widetilde{ki}),6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})  \nonumber\\
 \ph{4}&&+\bigg[ -2J_{2,GQ,q^\prime \to g}^{1,IF}(s_{1k})
 +2J_{2,GQ,q^\prime \to g}^{1,IF}(s_{(\widetilde{ki})1})
\bigg]  A_3^{0}(j,i,k)\,B_1^{\gamma,0}((\widetilde{ji}),1,(\widetilde{ki}),6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})  \nonumber\\
 \ph{5}&& -4J_{2,GQ,q^\prime \to g}^{1,IF}(s_{1k})
\,a_{3,g\to q}^{0}(k,1,j)\,B_1^{\gamma,0}((\widetilde{kj}),\overline{1},i,6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})  \nonumber\\
 \ph{6}&& +2J_{2,GQ,q^\prime \to g}^{1,IF}(s_{\overline{1}k})
\,d_{3,g}^{0}(j,i,1)\,B_1^{\gamma,0}((\widetilde{ji}),\overline{1},k,6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})  \nonumber\\
 \ph{7}&& -2J_{2,GQ,q^\prime \to g}^{1,IF}(s_{\overline{1}(\widetilde{ki})})
\,d_{3,g}^{0}(k,i,1)\,B_1^{\gamma,0}(j,\overline{1},(\widetilde{ki}),6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})  \nonumber\\
 \ph{8}&& -2J_{2,GQ,q^\prime \to g}^{1,IF}(s_{1k})
\,a_{3,g\to q}^{0}(k,1,j)\,B_1^{\gamma,0}((\widetilde{jk}),i,\overline{1},6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})  \nonumber\\
 \ph{9}&& -2J_{2,GQ,q^\prime \to g}^{1,IF}(s_{1k})
\,a_{3,g\to q}^{0}(j,1,k)\,B_1^{\gamma,0}(\overline{1},i,(\widetilde{jk}),6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})  \nonumber\\
\end{eqnarray}


==> sub/autoqbBhh1g2AU.tex <==
\section*{qbBhh1g2AU}
\begin{eqnarray}
\lefteqn{{\tt qbBhh1g2AU(4,3,1,5,2) =}} \\
 \ph{1}&&+\bigg[ 
 -\frac{1}{2}\,\,{\cal E}_{3}^{0}(s_{34}) 
 -\frac{1}{2}\,\,{\cal E}_{3,q}^{0}(s_{13}) 
 \bigg] 
\left( -\frac{b_F}{\epsilon}B_1^{\gamma,0}(4,3,1,5,2) +\hat{B}_1^{\gamma,1}(4,3,1,5,2)\right)
 \nonumber\\
 \ph{2}&&+\bigg[ 
 -\frac{b_F}{2\epsilon}\,{\cal E}_{3}^{0}(s_{34})\,\bigg( \frac{s_{34}}{\mu_R^2}\bigg)^{-\epsilon} 
 -\frac{b_F}{2\epsilon}\,{\cal E}_{3,q}^{0}(s_{13})\,\bigg( \frac{s_{13}}{\mu_R^2}\bigg)^{-\epsilon} 
 -\frac{1}{2}\,\,\hat{\cal{E}}_{3}^{1}(s_{34}) 
 \nonumber \\ && \phantom{+\bigg[} 
 -\frac{1}{2}\,\,\hat{\cal{E}}_{3,q}^{1}(s_{13}) 
 \bigg] 
 B_1^{\gamma,0}(4,3,1,5,2)
 \nonumber\\
\end{eqnarray}


==> sub/autoqbBt1g1AT.tex <==
\section*{qbBt1g1AT(j,i,1,5,2)}
\begin{eqnarray}
  \ph{1}&&-J_{2,QQ}^{1,IF}(s_{1j})\,B_1^{\gamma,0}(j,i,1,5,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
\end{eqnarray}


==> sub/autoqbBt1g2AU.tex <==
\section*{qbBt1g2AU}
\begin{eqnarray}
\lefteqn{{\tt qbBt1g2AU(4,3,1,5,2) =}} \\
 \ph{1}&&+\bigg[ 
 -\frac{1}{2}\,\,{\cal D}_{3,q}^{0}(s_{13}) 
 +\,\Gamma^{(1)}_{qq}(z_1) 
 -\frac{1}{2}\,\,{\cal D}_{3}^{0}(s_{34}) 
 \bigg] 
 \tilde{B}_3^{\gamma,1}(4,3,1,5,2)
 \nonumber\\
 \ph{2}&&+\bigg[ 
 +\,\Gamma^{(1)}_{qq}(z_1) 
 -\,{\cal A}_{3,q}^{0}(s_{14}) 
 \bigg] 
\left( -\frac{b_0}{\epsilon}B_1^{\gamma,0}(4,3,1,5,2) +B_1^{\gamma,1}(4,3,1,5,2)\right)
 \nonumber\\
 \ph{3}&&+\bigg[ 
 +\frac{1}{2}\,\,\Gamma^{(1)}_{qq}(z_1)\otimes{\cal D}_{3,q}^{0}(s_{13}) 
 -\,\Gamma^{(1)}_{qq}(z_1)\otimes\Gamma^{(1)}_{qq}(z_1) 
 -\frac{1}{2}\,\,{\cal D}_{3,q}^{0}(s_{13})\otimes{\cal A}_{3,q}^{0}(s_{14}) 
 \nonumber \\ && \phantom{+\bigg[} 
 +\,\Gamma^{(1)}_{qq}(z_1)\otimes{\cal A}_{3,q}^{0}(s_{14}) 
 \bigg] 
 B_1^{\gamma,0}(4,3,1,5,2)
 \nonumber\\
 \ph{4}&&+\bigg[ 
 +\frac{1}{2}\,\,\Gamma^{(1)}_{qq}(z_1)\otimes{\cal D}_{3}^{0}(s_{34}) 
 -\frac{1}{2}\,\,{\cal D}_{3}^{0}(s_{34})\otimes{\cal A}_{3,q}^{0}(s_{14}) 
 \bigg] 
 B_1^{\gamma,0}(4,3,1,5,2)
 \nonumber\\
 \ph{5}&&+\bigg[ 
 -\frac{b_0}{\epsilon}\,\bigg( \frac{s_{14}}{\mu_R^2}\bigg)^{-\epsilon}\,{\cal A}_{3,q}^{0}(s_{14}) 
 +\,{\cal A}_{3,q}^{0}(s_{14})\otimes{\cal A}_{3,q}^{0}(s_{14}) 
 -\,{\cal A}_{4,q}^{0}(s_{14}) 
 \nonumber \\ && \phantom{+\bigg[} 
 -\,{\cal{A}}_{3,q}^{1}(s_{14}) 
 +\,\Gamma^{(2)}_{qq}(z_1) 
 \bigg] 
 B_1^{\gamma,0}(4,3,1,5,2)
 \nonumber\\
 \ph{6}&&+\bigg[ 
 -\frac{1}{2}\,\,\tilde{\cal A}_{4,q}^{0}(s_{14}) 
 -\,\tilde{\cal{A}}_{3,q}^{1}(s_{14}) 
 -\,{\cal C}_{4,\bar{q},\bar{q}q\bar{q}}^{0}(s_{14}) 
 \nonumber \\ && \phantom{+\bigg[} 
 -2\,{\cal C}_{4,q}^{0}(s_{14}) 
 -\,\widetilde{\widetilde{\Gamma}}^{(2)}_{qq}(z_1) 
 \bigg] 
 B_1^{\gamma,0}(4,3,1,5,2)
 \nonumber\\
 \ph{7}&&+\bigg[ 
 -\,{\cal C}_{4,\bar{q},q\bar{q}\bar{q}}^{0}(s_{14}) 
 -\,\Gamma^{(2)}_{q\bar{q}}t(z_1) 
 \bigg] 
 B_1^{\gamma,0}(1,3,4,5,2)
 \nonumber\\
\end{eqnarray}


==> sub/autoqbBt2g0AS.tex <==
\section*{qbBt2g0AS(k,j,i,1,6,2)}
\begin{eqnarray}
\lefteqn{{\tt qbBt2g0AS(k,j,i,1,6,2) =}} \\
 \ph{1}&&+A_{3,q}^{0}(1,j,k)\,B_1^{\gamma,0}((\widetilde{jk}),i,\overline{1},6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{2}&&+A_{3,q}^{0}(1,i,k)\,B_1^{\gamma,0}((\widetilde{ik}),j,\overline{1},6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\end{eqnarray}


==> sub/autoqbBt2g1AT.tex <==
\section*{qbBt2g1AT(k,j,i,1,6,2)}
\begin{eqnarray}
  \ph{1}&&-J_{2,QQ}^{1,IF}(s_{1k})\,B_2^{\gamma,0}(k,j,i,1,6,2)\,J_2^{(3)}(\lbrace p\rbrace_{3})\nonumber\\
  \ph{2}&&-J_{2,QQ}^{1,IF}(s_{1k})\,B_2^{\gamma,0}(k,i,j,1,6,2)\,J_2^{(3)}(\lbrace p\rbrace_{3})\nonumber\\
 \ph{3}&&-\bigg[ 
 +J_{2,QG}^{1,IF}(s_{1i})
 +J_{2,QG}^{1,IF}(s_{1j})
 +J_{2,QG}^{1,FF}(s_{ki})
 +J_{2,QG}^{1,FF}(s_{kj})\bigg]\,\tilde{B}_2^{\gamma,0}(k,j,i,1,6,2)\,J_2^{(3)}(\lbrace p\rbrace_{3})\nonumber\\
  \ph{4}&&+J_{2,QQ}^{1,IF}(s_{1k})\,\tilde{B}_2^{\gamma,0}(k,i,j,1,6,2)\,J_2^{(3)}(\lbrace p\rbrace_{3})\nonumber\\
  \ph{5}&&+\,A_3^{0}(1,i,k)\,\bigg[\,B_1^{\gamma,1}((\widetilde{ki}),j,\overline{1},6,2)\,\delta(1-x_1)\,\delta(1-x_2)\nonumber\\
  &&+\,\bigg( 
 +J_{2,QG}^{1,IF}(s_{\overline{1}j})
 +J_{2,QG}^{1,FF}(s_{(\widetilde{ki})j})\bigg)\,B_1^{\gamma,0}((\widetilde{ki}),j,\overline{1},6,2) \bigg]\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
  \ph{6}&&+\,A_3^{0}(1,j,k)\,\bigg[\,B_1^{\gamma,1}((\widetilde{kj}),i,\overline{1},6,2)\,\delta(1-x_1)\,\delta(1-x_2)\nonumber\\
  &&+\,\bigg( 
 +J_{2,QG}^{1,IF}(s_{\overline{1}i})
 +J_{2,QG}^{1,FF}(s_{(\widetilde{kj})i})\bigg)\,B_1^{\gamma,0}((\widetilde{kj}),i,\overline{1},6,2) \bigg]\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
  \ph{7}&&+\,d_3^{0}(k,i,j)\,\bigg[\,\tilde{B}_3^{\gamma,1}((\widetilde{ki}),(\widetilde{ij}),1,6,2)\,\delta(1-x_1)\,\delta(1-x_2)\nonumber\\
 &&\phantom{\bigg[}+J_{2,QQ}^{1,IF}(s_{1(\widetilde{ki})})\,B_1^{\gamma,0}((\widetilde{ki}),(\widetilde{ij}),1,6,2) \bigg]\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
  \ph{8}&&+\,d_3^{0}(k,j,i)\,\bigg[\,\tilde{B}_3^{\gamma,1}((\widetilde{kj}),(\widetilde{ji}),1,6,2)\,\delta(1-x_1)\,\delta(1-x_2)\nonumber\\
 &&\phantom{\bigg[}+J_{2,QQ}^{1,IF}(s_{1(\widetilde{kj})})\,B_1^{\gamma,0}((\widetilde{kj}),(\widetilde{ji}),1,6,2) \bigg]\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
  \ph{9}&&+\,D_{3,q}^{0}(1,i,j)\,\bigg[\,\tilde{B}_3^{\gamma,1}(k,(\widetilde{ij}),\overline{1},6,2)\,\delta(1-x_1)\,\delta(1-x_2)\nonumber\\
 &&\phantom{\bigg[}+J_{2,QQ}^{1,IF}(s_{\overline{1}k})\,B_1^{\gamma,0}(k,(\widetilde{ij}),\overline{1},6,2) \bigg]\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
  \ph{10}&&+\bigg[\,A_{3,q}^{1}(1,i,k)\,\delta(1-x_1)\,\delta(1-x_2)
  \nonumber\\&&\,  
   +\bigg( 
 +J_{2,QG}^{1,IF}(s_{1i})
 +J_{2,QG}^{1,FF}(s_{ki})
 -J_{2,QQ}^{1,IF}(s_{\overline{1}(\widetilde{ki})})\bigg)\,A_3^{0}(1,i,k)\bigg]\,B_1^{\gamma,0}((\widetilde{ki}),j,\overline{1},6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
  \ph{11}&&+\bigg[\,A_{3,q}^{1}(1,j,k)\,\delta(1-x_1)\,\delta(1-x_2)
  \nonumber\\&&\,  
   +\bigg( 
 +J_{2,QG}^{1,IF}(s_{1j})
 +J_{2,QG}^{1,FF}(s_{kj})
 -J_{2,QQ}^{1,IF}(s_{\overline{1}(\widetilde{kj})})\bigg)\,A_3^{0}(1,j,k)\bigg]\,B_1^{\gamma,0}((\widetilde{kj}),i,\overline{1},6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
  \ph{12}&&+\bigg[\,\tilde{A}_{3,q}^{1}(1,i,k)\,\delta(1-x_1)\,\delta(1-x_2)
  \nonumber\\&&\,  
   +\bigg( 
 +J_{2,QQ}^{1,IF}(s_{1k})
 -J_{2,QQ}^{1,IF}(s_{\overline{1}(\widetilde{ki})})\bigg)\,A_3^{0}(1,i,k)\bigg]\,B_1^{\gamma,0}((\widetilde{ki}),j,\overline{1},6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
  \ph{13}&&+\bigg[\,\tilde{A}_{3,q}^{1}(1,j,k)\,\delta(1-x_1)\,\delta(1-x_2)
  \nonumber\\&&\,  
   +\bigg( 
 +J_{2,QQ}^{1,IF}(s_{1k})
 -J_{2,QQ}^{1,IF}(s_{\overline{1}(\widetilde{kj})})\bigg)\,A_3^{0}(1,j,k)\bigg]\,B_1^{\gamma,0}((\widetilde{kj}),i,\overline{1},6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
 \ph{14}&&-\bigg[ +J_{2,QG}^{1,FF}(s_{(\widetilde{ki})j})
 -J_{2,QQ}^{1,IF}(s_{\overline{1}(\widetilde{ki})})
 -J_{2,QG}^{1,IF}(s_{1j})
 +J_{2,QG}^{1,IF}(s_{\overline{1}j})
 -J_{2,QG}^{1,FF}(s_{kj})
 +J_{2,QQ}^{1,IF}(s_{1k})
 \nonumber\\&&\phantom{-} \nonumber\\ &&+\bigg(  -{\cal S}^{FF}(s_{1k},s_{kj},x_{1k,kj})
 +{\cal S}^{FF}(s_{\overline{1}(\widetilde{ki})},s_{kj},x_{\overline{1}(\widetilde{ki}),kj})
 +{\cal S}^{FF}(s_{1j},s_{kj},x_{1j,kj})
 -{\cal S}^{FF}(s_{\overline{1}j},s_{kj},x_{\overline{1}j,kj})
 \nonumber\\&&\phantom{-} +{\cal S}^{FF}(s_{kj},s_{kj},1)
 -{\cal S}^{FF}(s_{(\widetilde{ki})j},s_{kj},x_{(\widetilde{ki})j,kj})
 \bigg)\bigg]\nonumber\\
 &&\times A_3^{0}(1,i,k)\,B_1^{\gamma,0}((\widetilde{ki}),j,\overline{1},6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{15}&&+\bigg[ +J_{2,QG}^{1,IF}(s_{1i})
 -J_{2,QG}^{1,IF}(s_{\overline{1}i})
 +J_{2,QG}^{1,FF}(s_{ki})
 -J_{2,QG}^{1,FF}(s_{(\widetilde{kj})i})
 -J_{2,QQ}^{1,IF}(s_{1k})
 +J_{2,QQ}^{1,IF}(s_{\overline{1}(\widetilde{kj})})
 \nonumber\\&&\phantom{+} \nonumber\\ &&+\bigg(  +{\cal S}^{FF}(s_{1k},s_{ki},x_{1k,ki})
 -{\cal S}^{FF}(s_{\overline{1}(\widetilde{kj})},s_{ki},x_{\overline{1}(\widetilde{kj}),ki})
 -{\cal S}^{FF}(s_{1i},s_{ki},x_{1i,ki})
 +{\cal S}^{FF}(s_{\overline{1}i},s_{ki},x_{\overline{1}i,ki})
 \nonumber\\&&\phantom{+} -{\cal S}^{FF}(s_{ki},s_{ki},1)
 +{\cal S}^{FF}(s_{(\widetilde{kj})i},s_{ki},x_{(\widetilde{kj})i,ki})
 \bigg)\bigg]\nonumber\\
 &&\times A_3^{0}(1,j,k)\,B_1^{\gamma,0}((\widetilde{kj}),i,\overline{1},6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\end{eqnarray}


==> sub/autoqbBt3g0AS.tex <==
\section*{qbBt3g0AS(l,k,j,i,1,7,2)}
\begin{eqnarray}
\lefteqn{{\tt qbBt3g0AS(l,k,j,i,1,7,2) =}} \\
 \ph{1}&&+A_3^{0}(1,i,l)\,B_2^{\gamma,0}((\widetilde{li}),k,j,\overline{1},7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{2}&&+d_3^{0}(1,j,k)\,\tilde{B}_2^{\gamma,0}(l,(\widetilde{jk}),i,\overline{1},7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{3}&&+d_3^{0}(l,k,j)\,\tilde{B}_2^{\gamma,0}((\widetilde{lk}),(\widetilde{jk}),i,1,7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
\snip \ph{4}&&+\,A_4^0(1,j,k,l)\,B_1^{\gamma,0}((\widetilde{jkl}),i,\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{5}&&-\,d_3^{0}(1,j,k)\,A_3^{0}(\overline{1},(\widetilde{jk}),l)\,B_1^{\gamma,0}((\widetilde{l\widetilde{(jk})}),i,\overline{\overline{1}},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{6}&&-\,d_3^{0}(l,k,j)\,A_3^{0}(1,(\widetilde{jk}),(\widetilde{lk}))\,B_1^{\gamma,0}([(\widetilde{jk}), (\widetilde{lk})],i,\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\snip \ph{7}&&+\,\tilde{A}_4^0(1,i,j,l)\,B_1^{\gamma,0}((\widetilde{ijl}),k,\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{8}&&-\,A_3^{0}(1,i,l)\,A_3^{0}(\overline{1},j,(\widetilde{li}))\,B_1^{\gamma,0}((\widetilde{j\widetilde{(li})}),k,\overline{\overline{1}},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{9}&&-\,A_3^{0}(1,j,l)\,A_3^{0}(\overline{1},i,(\widetilde{lj}))\,B_1^{\gamma,0}((\widetilde{i\widetilde{(lj})}),k,\overline{\overline{1}},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{10}&&+\,A_3^{0}(1,j,l)\,A_3^{0}(\overline{1},i,(\widetilde{lj}))\,B_1^{\gamma,0}((\widetilde{i\widetilde{(lj})}),k,\overline{\overline{1}},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{11}&&-\,d_3^{0}(1,j,k)\,A_3^{0}(\overline{1},i,l)\,B_1^{\gamma,0}((\widetilde{li}),(\widetilde{jk}),\overline{\overline{1}},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{12}&&-\,d_3^{0}(l,k,j)\,A_3^{0}(1,i,(\widetilde{lk}))\,B_1^{\gamma,0}((\widetilde{i\widetilde{(lk})}),(\widetilde{kj}),\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{13}&&-\bigg[      +S^{FF}_{1j(\widetilde{lj})}       -S^{FF}_{\overline{1}j(\widetilde{i\widetilde{(lj})})}       -S^{FF}_{1j(\widetilde{kj})}       +S^{FF}_{\overline{1}j(\widetilde{kj})}       -S^{FF}_{(\widetilde{lj})j(\widetilde{kj})}       +S^{FF}_{(\widetilde{i\widetilde{(lj})})j(\widetilde{kj})}  \bigg]\nonumber\\
 &&\times A_3^{0}(1,i,(\widetilde{lj}))\,B_1^{\gamma,0}((\widetilde{i\widetilde{(lj})}),(\widetilde{kj}),\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\end{eqnarray}


==> sub/autoqbBth1g2AU.tex <==
\section*{qbBth1g2AU}
\begin{eqnarray}
\lefteqn{{\tt qbBth1g2AU(4,3,1,5,2) =}} \\
 \ph{1}&&+\bigg[ 
 +\,{\cal A}_{3,q}^{0}(s_{14}) 
 -\,\Gamma^{(1)}_{qq}(z_1) 
 \bigg] 
\left( -\frac{b_F}{\epsilon}B_1^{\gamma,0}(4,3,1,5,2) +\hat{B}_1^{\gamma,1}(4,3,1,5,2)\right)
 \nonumber\\
 \ph{2}&&+\bigg[ 
 +\frac{1}{2}\,\,{\cal E}_{3,q}^{0}(s_{13}) 
 +\frac{1}{2}\,\,{\cal E}_{3}^{0}(s_{34}) 
 \bigg] 
 \tilde{B}_3^{\gamma,1}(4,3,1,5,2)
 \nonumber\\
 \ph{3}&&+\bigg[ 
 +\frac{1}{2}\,\,{\cal E}_{3}^{0}(s_{34})\otimes{\cal A}_{3,q}^{0}(s_{14}) 
 +\frac{1}{2}\,\,{\cal E}_{3,q}^{0}(s_{13})\otimes{\cal A}_{3,q}^{0}(s_{14}) 
 -\frac{1}{2}\,\,\Gamma^{(1)}_{qq}(z_1)\otimes{\cal E}_{3}^{0}(s_{34}) 
 \nonumber \\ && \phantom{+\bigg[} 
 -\frac{1}{2}\,\,\Gamma^{(1)}_{qq}(z_1)\otimes{\cal E}_{3,q}^{0}(s_{13}) 
 \bigg] 
 B_1^{\gamma,0}(4,3,1,5,2)
 \nonumber\\
 \ph{4}&&+\bigg[ 
 +\frac{1}{2}\,\,\tilde{\cal E}_{4,q}^{0}(s_{13}) 
 +\frac{1}{2}\,\,\tilde{\cal{E}}_{3,q}^{1}(s_{13}) 
 -\,\Gamma^{(2)}_{qq,F}(z_1) 
 \bigg] 
 B_1^{\gamma,0}(4,3,1,5,2)
 \nonumber\\
 \ph{5}&&+\bigg[ 
 +\frac{1}{2}\,\,\tilde{\cal E}_{4}^{0}(s_{34}) 
 +\frac{1}{2}\,\,\tilde{\cal{E}}_{3}^{1}(s_{34}) 
 \bigg] 
 B_1^{\gamma,0}(4,3,1,5,2)
 \nonumber\\
 \ph{6}&&+\bigg[ 
 +\frac{b_F}{\epsilon}\,\bigg( \frac{s_{14}}{\mu_R^2}\bigg)^{-\epsilon}\,{\cal A}_{3,q}^{0}(s_{14}) 
 +\,{\cal B}_{4,q}^{0}(s_{14}) 
 +\,\hat{\cal{A}}_{3,q}^{1}(s_{14}) 
 \bigg] 
 B_1^{\gamma,0}(4,3,1,5,2)
 \nonumber\\
\end{eqnarray}


==> sub/autoqbBth2g1AT.tex <==
\section*{qbBth2g1AT(k,j,i,1,6,2)}
\begin{eqnarray}
  \ph{1}&&-4\hat{J}_{2,QG}^{1,FF}(s_{ki})\,\tilde{B}_2^{\gamma,0}(k,j,i,1,6,2)\,J_2^{(3)}(\lbrace p\rbrace_{3})\nonumber\\
  \ph{2}&&+2\,A_3^{0}(1,i,k)\,\bigg[\,\hat{B}_1^{\gamma,1}((\widetilde{ik}),j,\overline{1},6,2)\,\delta(1-x_1)\,\delta(1-x_2)\nonumber\\
 &&\phantom{\bigg[}+2\hat{J}_{2,QG}^{1,FF}(s_{(\widetilde{ki})j})\,B_1^{\gamma,0}((\widetilde{ik}),j,\overline{1},6,2) \bigg]\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
  \ph{3}&&+2\bigg[\,\hat{A}_{3}^{1}(1,i,k)\,\delta(1-x_1)\,\delta(1-x_2)
 +2\hat{J}_{2,QG}^{1,FF}(s_{ki})\,A_3^{0}(1,i,k)\bigg]\,B_1^{\gamma,0}((\widetilde{ik}),j,\overline{1},6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
 \ph{4}&&+\bigg[ +4\hat{J}_{2,QG}^{1,FF}(s_{kj})
 -4\hat{J}_{2,QG}^{1,FF}(s_{(\widetilde{ki})j})
\bigg]  A_3^{0}(1,i,k)\,B_1^{\gamma,0}((\widetilde{ik}),j,\overline{1},6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})  \nonumber\\
\end{eqnarray}


==> sub/autoqbBth2g1ATqtog.tex <==
\section*{qbBth2g1ATqtog(1,i,j,k,6,2)}
\begin{eqnarray}
 \ph{1}&&-\bigg[ 
 +J_{2,GQ,q^\prime \to g}^{1,IF}(s_{1k})
 +J_{2,GQ,q^\prime \to g}^{1,IF}(s_{1j})\bigg]\,\tilde{B}_2^{\gamma,0}(j,i,1,k,6,2)\,J_2^{(3)}(\lbrace p\rbrace_{3})\nonumber\\
 \ph{2}&&+\bigg[ +J_{2,GQ,q^\prime \to g}^{1,IF}(s_{1k})
 +J_{2,GQ,q^\prime \to g}^{1,IF}(s_{1j})
\bigg]  A_3^{0}(k,i,j)\,B_1^{\gamma,0}((\widetilde{ij}),1,(\widetilde{ki}),6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})  \nonumber\\
 \ph{3}&&+\bigg[ -J_{2,GQ,q^\prime \to g}^{1,IF}(s_{1k})
 -J_{2,GQ,q^\prime \to g}^{1,IF}(s_{1j})
\bigg]  a_{3,g\to q}^{0}(k,1,j)\,B_1^{\gamma,0}((\widetilde{kj}),i,\overline{1},6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})  \nonumber\\
 \ph{4}&&+\bigg[ -J_{2,GQ,q^\prime \to g}^{1,IF}(s_{1k})
 -J_{2,GQ,q^\prime \to g}^{1,IF}(s_{1j})
\bigg]  a_{3,g\to q}^{0}(j,1,k)\,B_1^{\gamma,0}(\overline{1},i,(\widetilde{kj}),6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})  \nonumber\\
\end{eqnarray}


==> sub/autoqbBtt1g2AU.tex <==
\section*{qbBtt1g2AU}
\begin{eqnarray}
\lefteqn{{\tt qbBtt1g2AU(4,3,1,5,2) =}} \\
 \ph{1}&&+\bigg[ 
 -\,{\cal A}_{3,q}^{0}(s_{14}) 
 +\,\Gamma^{(1)}_{qq}(z_1) 
 \bigg] 
 \tilde{B}_3^{\gamma,1}(4,3,1,5,2)
 \nonumber\\
 \ph{2}&&+\bigg[ 
 +\,\Gamma^{(1)}_{qq}(z_1)\otimes{\cal A}_{3,q}^{0}(s_{14}) 
 -\frac{1}{2}\,\,\Gamma^{(1)}_{qq}(z_1)\otimes\Gamma^{(1)}_{qq}(z_1) 
 -\frac{1}{2}\,\,\tilde{\cal A}_{4,q}^{0}(s_{14}) 
 \nonumber \\ && \phantom{+\bigg[} 
 -\,\tilde{\cal{A}}_{3,q}^{1}(s_{14}) 
 -2\,{\cal C}_{4,q}^{0}(s_{14}) 
 -\,{\cal C}_{4,\bar{q},\bar{q}q\bar{q}}^{0}(s_{14}) 
 \nonumber \\ && \phantom{+\bigg[} 
 -\,\widetilde{\widetilde{\Gamma}}^{(2)}_{qq}(z_1) 
 \bigg] 
 B_1^{\gamma,0}(4,3,1,5,2)
 \nonumber\\
 \ph{3}&&+\bigg[ 
 -\,{\cal C}_{4,\bar{q},q\bar{q}\bar{q}}^{0}(s_{14}) 
 -\,\Gamma^{(2)}_{q\bar{q}}t(z_1) 
 \bigg] 
 B_1^{\gamma,0}(1,3,4,5,2)
 \nonumber\\
\end{eqnarray}


==> sub/autoqbBtt2g1AT.tex <==
\section*{qbBtt2g1AT(k,j,i,1,6,2)}
\begin{eqnarray}
  \ph{1}&&-J_{2,QQ}^{1,IF}(s_{1k})\,\tilde{B}_2^{\gamma,0}(k,j,i,1,6,2)\,J_2^{(3)}(\lbrace p\rbrace_{3})\nonumber\\
  \ph{2}&&+\,A_3^{0}(1,i,k)\,\bigg[\,\tilde{B}_3^{\gamma,1}((\widetilde{ki}),j,\overline{1},6,2)\,\delta(1-x_1)\,\delta(1-x_2)\nonumber\\
 &&\phantom{\bigg[}+J_{2,QQ}^{1,IF}(s_{\overline{1}(\widetilde{ki})})\,B_1^{\gamma,0}((\widetilde{ki}),j,\overline{1},6,2) \bigg]\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
  \ph{3}&&+\,A_3^{0}(1,j,k)\,\bigg[\,\tilde{B}_3^{\gamma,1}((\widetilde{kj}),i,\overline{1},6,2)\,\delta(1-x_1)\,\delta(1-x_2)\nonumber\\
 &&\phantom{\bigg[}+J_{2,QQ}^{1,IF}(s_{\overline{1}(\widetilde{kj})})\,B_1^{\gamma,0}((\widetilde{kj}),i,\overline{1},6,2) \bigg]\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
  \ph{4}&&+\bigg[\,\tilde{A}_{3,q}^{1}(1,i,k)\,\delta(1-x_1)\,\delta(1-x_2)
  \nonumber\\&&\,  
   +\bigg( 
 +J_{2,QQ}^{1,IF}(s_{1k})
 -J_{2,QQ}^{1,IF}(s_{\overline{1}(\widetilde{ki})})\bigg)\,A_3^{0}(1,i,k)\bigg]\,B_1^{\gamma,0}((\widetilde{ki}),j,\overline{1},6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
  \ph{5}&&+\bigg[\,\tilde{A}_{3,q}^{1}(1,j,k)\,\delta(1-x_1)\,\delta(1-x_2)
  \nonumber\\&&\,  
   +\bigg( 
 +J_{2,QQ}^{1,IF}(s_{1k})
 -J_{2,QQ}^{1,IF}(s_{\overline{1}(\widetilde{kj})})\bigg)\,A_3^{0}(1,j,k)\bigg]\,B_1^{\gamma,0}((\widetilde{kj}),i,\overline{1},6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
\end{eqnarray}


==> sub/autoqbBtt3g0AS.tex <==
\section*{qbBtt3g0AS(l,k,j,i,1,7,2)}
\begin{eqnarray}
\lefteqn{{\tt qbBtt3g0AS(l,k,j,i,1,7,2) =}} \\
 \ph{1}&&+A_3^{0}(1,i,l)\,\tilde{B}_2^{\gamma,0}((\widetilde{li}),k,j,\overline{1},7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{2}&&+A_3^{0}(1,j,l)\,\tilde{B}_2^{\gamma,0}((\widetilde{lj}),k,i,\overline{1},7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{3}&&+A_3^{0}(1,k,l)\,\tilde{B}_2^{\gamma,0}((\widetilde{lk}),j,i,\overline{1},7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
\snip \ph{4}&&+\,\tilde{A}_4^0(1,i,j,l)\,B_1^{\gamma,0}((\widetilde{lij}),k,\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{5}&&-\,A_3^{0}(1,i,l)\,A_3^{0}(\overline{1},j,(\widetilde{li}))\,B_1^{\gamma,0}((\widetilde{j\widetilde{(li})}),k,\overline{\overline{1}},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{6}&&-\,A_3^{0}(1,j,l)\,A_3^{0}(\overline{1},i,(\widetilde{lj}))\,B_1^{\gamma,0}((\widetilde{i\widetilde{(lj})}),k,\overline{\overline{1}},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\snip \ph{7}&&+\,\tilde{A}_4^0(1,i,k,l)\,B_1^{\gamma,0}((\widetilde{lik}),j,\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{8}&&-\,A_3^{0}(1,i,l)\,A_3^{0}(\overline{1},k,(\widetilde{li}))\,B_1^{\gamma,0}((\widetilde{k\widetilde{(li})}),j,\overline{\overline{1}},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{9}&&-\,A_3^{0}(1,k,l)\,A_3^{0}(\overline{1},i,(\widetilde{lk}))\,B_1^{\gamma,0}((\widetilde{i\widetilde{(lk})}),j,\overline{\overline{1}},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\snip \ph{10}&&+\,\tilde{A}_4^0(1,j,k,l)\,B_1^{\gamma,0}((\widetilde{ljk}),i,\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{11}&&-\,A_3^{0}(1,j,l)\,A_3^{0}(\overline{1},k,(\widetilde{lj}))\,B_1^{\gamma,0}((\widetilde{k\widetilde{(lj})}),i,\overline{\overline{1}},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{12}&&-\,A_3^{0}(1,k,l)\,A_3^{0}(\overline{1},j,(\widetilde{lk}))\,B_1^{\gamma,0}((\widetilde{j\widetilde{(lk})}),i,\overline{\overline{1}},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\end{eqnarray}


==> sub/autoqbC0g0AS.tex <==
\section*{qbC0g0AS(k,j,i,1,6,2)}
\begin{eqnarray}
\lefteqn{{\tt qbC0g0AS(k,j,i,1,6,2) =}} \\
 \ph{1}&&+E_3^{0}(k,i,j)\,B_{1,I}^{\gamma,0}((\widetilde{ki}),(\widetilde{ji}),1,6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{2}&&-\frac{1}{2}\,E_{3,q^\prime\to g}^{0}(i,1,k)\,B_{1,,II}^{\gamma,0}((\widetilde{ik}),\overline{1},j,6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{3}&&-\frac{1}{2}\,E_{3,q^\prime\to g}^{0}(j,1,k)\,B_{1,,II}^{\gamma,0}(i,\overline{1},(\widetilde{jk}),6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\end{eqnarray}


==> sub/autoqbC0g1AT.tex <==
\section*{qbC0g1AT(i,k,j,1,6,2)}
\begin{eqnarray}
 \ph{1}&&-\bigg[ 
 +J_{2,QQ}^{1,FF}(s_{ik})
 +J_{2,QQ}^{1,IF}(s_{1j})\bigg]\,C_0^{\gamma,0}(i,k,j,1,6,2)\,J_2^{(3)}(\lbrace p\rbrace_{3})\nonumber\\
  \ph{2}&&+\frac{1}{2}\,\,E_3^{0}(i,j,k)\,\bigg[\,B_{1,I}^{\gamma,1}((\widetilde{ij}),(\widetilde{jk}),1,6,2)\,\delta(1-x_1)\,\delta(1-x_2)\nonumber\\
  &&+\,\bigg( 
 +J_{2,QG}^{1,FF}(s_{(\widetilde{ij})(\widetilde{jk})})
 +J_{2,QG}^{1,IF}(s_{1(\widetilde{jk})})\bigg)\,B_{1,I}^{\gamma,0}((\widetilde{ij}),(\widetilde{jk}),1,6,2) \bigg]\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
  \ph{3}&&+\frac{1}{2}\,\,E_{3,q}^{0}(1,j,k)\,\bigg[\,B_{1,I}^{\gamma,1}(i,(\widetilde{jk}),\overline{1},6,2)\,\delta(1-x_1)\,\delta(1-x_2)\nonumber\\
  &&+\,\bigg( 
 +J_{2,QG}^{1,IF}(s_{\overline{1}(\widetilde{jk})})
 +J_{2,QG}^{1,FF}(s_{i(\widetilde{jk})})\bigg)\,B_{1,I}^{\gamma,0}(i,(\widetilde{jk}),\overline{1},6,2) \bigg]\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
  \ph{4}&&+\frac{1}{2}\,\bigg[\,E_{3}^{1}(i,j,k)\,\delta(1-x_1)\,\delta(1-x_2)
  \nonumber\\&&\,  
   +\bigg( 
 +J_{2,QQ}^{1,FF}(s_{ij})
 +J_{2,QQ}^{1,FF}(s_{ik})
 -2J_{2,QG}^{1,FF}(s_{(\widetilde{ij})(\widetilde{jk})})\bigg)\,E_3^{0}(i,j,k)\bigg]\,B_{1,I}^{\gamma,0}((\widetilde{ij}),(\widetilde{jk}),1,6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
  \ph{5}&&+\frac{1}{2}\,\bigg[\,E_{3}^{1}(1,j,k)\,\delta(1-x_1)\,\delta(1-x_2)
  \nonumber\\&&\,  
   +\bigg( 
 +J_{2,QQ}^{1,IF}(s_{1j})
 +J_{2,QQ}^{1,IF}(s_{1k})
 -2J_{2,QG}^{1,IF}(s_{\overline{1}(\widetilde{jk})})\bigg)\,E_3^{0}(1,j,k)\bigg]\,B_{1,I}^{\gamma,0}(i,(\widetilde{jk}),\overline{1},6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
  \ph{6}&&-\,E_{3,q^\prime\to g}^{0}(k,1,i)\,\bigg[\,B_{1,II}^{\gamma,1}(j,\overline{1},(\widetilde{ik}),6,2)\,\delta(1-x_1)\,\delta(1-x_2)\nonumber\\
  &&+\,\bigg( 
 +J_{2,GQ}^{1,IF}(s_{\overline{1}(\widetilde{ik})})
 +J_{2,GQ}^{1,IF}(s_{\overline{1}j})
 -J_{2,QG,g \to q}^{1,IF}(s_{\overline{1}(\widetilde{ik})})
 -J_{2,QG,g \to q}^{1,IF}(s_{\overline{1}j})\bigg)\,B_{1,,II}^{\gamma,0}(j,\overline{1},(\widetilde{ik}),6,2) \bigg]\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
  \ph{7}&&-\bigg[\,E_{3,q^\prime}^{1}(k,1,i)\,\delta(1-x_1)\,\delta(1-x_2)
  \nonumber\\&&\,  
   +\bigg( 
 +J_{2,QQ}^{1,IF}(s_{1k})
 +J_{2,QQ}^{1,FF}(s_{ki})
 -2J_{2,GQ}^{1,IF}(s_{\overline{1}(\widetilde{ki})})
 +2J_{2,QG,g \to q}^{1,IF}(s_{\overline{1}(\widetilde{ki})})\bigg)\,E_{3,q^\prime\to g}^{0}(k,1,i)\bigg]\,B_{1,,II}^{\gamma,0}(j,\overline{1},(\widetilde{ki}),6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
 \ph{8}&&+\bigg[ +J_{2,QQ}^{1,IF}(s_{1k})
 -J_{2,GQ}^{1,IF}(s_{\overline{1}(\widetilde{ki})})
 +J_{2,QG,g \to q}^{1,IF}(s_{\overline{1}(\widetilde{ki})})
 -J_{2,QQ}^{1,IF}(s_{1j})
 -J_{2,QQ}^{1,FF}(s_{kj})
 +J_{2,QQ}^{1,FF}(s_{j(\widetilde{ki})})
 \nonumber\\&&\phantom{+} +J_{2,GQ}^{1,IF}(s_{\overline{1}j})
 -J_{2,QG,g \to q}^{1,IF}(s_{\overline{1}j})
 \nonumber\\ &&+\bigg(  -{\cal S}^{FF}(s_{1k},s_{ki},x_{1k,ki})
 +{\cal S}^{FF}(s_{kj},s_{ki},x_{kj,ki})
 -{\cal S}^{FF}(s_{j(\widetilde{ki})},s_{ki},x_{j(\widetilde{ki}),ki})
 +{\cal S}^{FF}(s_{\overline{1}(\widetilde{ki})},s_{ki},x_{\overline{1}(\widetilde{ki}),ki})
 \nonumber\\&&\phantom{+} -{\cal S}^{FF}(s_{\overline{1}j},s_{ki},x_{\overline{1}j,ki})
 +{\cal S}^{FF}(s_{1j},s_{ki},x_{1j,ki})
 \bigg)\bigg]\nonumber\\
 &&\times E_{3,q^\prime\to g}^{0}(k,1,i)\,B_{1,,II}^{\gamma,0}(j,\overline{1},(\widetilde{ki}),6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\end{eqnarray}


==> sub/autoqbC1g0AS.tex <==
\section*{qbC1g0AS(l,i,k,j,1,7,2)}
\begin{eqnarray}
\lefteqn{{\tt qbC1g0AS(l,i,k,j,1,7,2) =}} \\
 \ph{1}&&+A_3^{0}(1,i,j)\,C_0^{\gamma,0}(l,k,(\widetilde{ji}),\overline{1},7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{2}&&+A_3^{0}(k,i,l)\,C_0^{\gamma,0}((\widetilde{li}),(\widetilde{ki}),j,1,7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{3}&&+E_3^{0}(l,j,k)\,B_{2,I}^{\gamma,0}((\widetilde{lj}),i,(\widetilde{jk}),1,7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{4}&&+E_3^{0}(l,j,k)\,B_{2,I}^{\gamma,0}((\widetilde{lj}),(\widetilde{jk}),i,1,7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
\snip \ph{5}&&+\,E_4^{0,a}(l,j,k,i)\,B_{1,I}^{\gamma,0}((\widetilde{ljk}),(\widetilde{ikj}),1,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\snip \ph{6}&&+\,E_4^{0,b}(l,i,k,j)\,B_{1,I}^{\gamma,0}((\widetilde{lik}),(\widetilde{jki}),1,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{7}&&-\,E_3^{0}(l,j,k)\,d_3^{0}((\widetilde{lj}),i,(\widetilde{jk}))\,B_{1,I}^{\gamma,0}((\widetilde{(\widetilde{lj})i}),(\widetilde{(\widetilde{jk})i}),1,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{8}&&-\,E_3^{0}(l,j,k)\,d_3^{0}((\widetilde{lj}),(\widetilde{jk}),i)\,B_{1,I}^{\gamma,0}([(\widetilde{lj}), (\widetilde{jk})],(\widetilde{i\widetilde{(kj})}),1,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{9}&&-\,A_3^{0}(k,i,l)\,E_3^{0}((\widetilde{li}),(\widetilde{ki}),j)\,B_{1,I}^{\gamma,0}([(\widetilde{ki}), (\widetilde{li})],(\widetilde{j\widetilde{(ki})}),1,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\snip \ph{10}&&+\,E_4^0(1,k,j,i)\,B_{1,I}^{\gamma,0}(l,(\widetilde{ijk}),\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{11}&&-\,E_3^{0}(l,j,k)\,D_3^{0}(1,(\widetilde{kj}),i)\,B_{1,I}^{\gamma,0}((\widetilde{lj}),(\widetilde{i\widetilde{(kj})}),\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{12}&&-\,A_3^{0}(1,i,j)\,E_3^{0}(\overline{1},k,(\widetilde{ji}))\,B_{1,I}^{\gamma,0}(l,(\widetilde{k\widetilde{(ji})}),\overline{\overline{1}},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{13}&&-E_{3,q^\prime\to g}^{0}(k,1,l)\,B_{2,II}^{\gamma,0}(j,i,\overline{1},(\widetilde{kl}),7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{14}&&-E_{3,q^\prime\to g}^{0}(k,1,l)\,B_{2,II}^{\gamma,0}(j,\overline{1},i,(\widetilde{kl}),7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
\snip \ph{15}&&-\,E_4^0(k,l,1,i)\,B_{1,,II}^{\gamma,0}(j,\overline{1},(\widetilde{kli}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{16}&&+\,E_{3,q^\prime\to g}^{0}(k,1,l)\,D_3^{0}((\widetilde{kl}),\overline{1},i)\,B_{1,,II}^{\gamma,0}(j,\overline{\overline{1}},(\widetilde{(\widetilde{kl})i}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\snip \ph{17}&&-\,E_4^0(k,1,l,i)\,B_{1,,II}^{\gamma,0}(j,\overline{1},(\widetilde{kli}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{18}&&+\,E_{3,q^\prime\to g}^{0}(k,l,1)\,D_3^{0}((\widetilde{kl}),\overline{1},i)\,B_{1,,II}^{\gamma,0}(j,\overline{\overline{1}},(\widetilde{(\widetilde{lk})i}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{19}&&+\,A_3^{0}(l,i,k)\,E_{3,q^\prime\to g}^{0}((\widetilde{ki}),1,(\widetilde{li}))\,B_{1,,II}^{\gamma,0}(j,\overline{1},[(\widetilde{ki}), (\widetilde{li})],7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\snip \ph{20}&&+\,B_4^0(k,1,l,j)\,B_{1,,II}^{\gamma,0}((\widetilde{jlk}),\overline{1},i,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{21}&&-2\,E_{3,q^\prime\to g}^{0}(k,1,l)\,a_{3,g\to q}^{0}((\widetilde{kl}),\overline{1},j)\,B_{1,,II}^{\gamma,0}((\widetilde{j\widetilde{(kl})}),\overline{\overline{1}},i,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\snip \ph{22}&&+\,B_4^0(k,1,l,j)\,{sB}_{1,II}^{\gamma,0}(\overline{1},i,(\widetilde{jlk}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{23}&&-\,E_{3,q^\prime\to g}^{0}(k,l,1)\,a_{3,g\to q}^{0}(j,\overline{1},(\widetilde{kl}))\,B_{1,,II}^{\gamma,0}(\overline{\overline{1}},i,(\widetilde{j\widetilde{(kl})}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{24}&&-\,E_{3,q^\prime\to g}^{0}(k,1,l)\,a_{3,g\to q}^{0}((\widetilde{kl}),\overline{1},j)\,B_{1,,II}^{\gamma,0}((\widetilde{j\widetilde{(kl})}),i,\overline{\overline{1}},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{25}&&+\,A_{3,q}^{0}(1,i,j)\,E_{3,q^\prime\to g}^{0}(k,\overline{1},l)\,B_{1,,II}^{\gamma,0}((\widetilde{ij}),\overline{\overline{1}},(\widetilde{kl}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{26}&&+\,A_3^{0}(k,i,j)\,E_{3,q^\prime\to g}^{0}((\widetilde{ki}),1,l)\,B_{1,,II}^{\gamma,0}((\widetilde{ji}),\overline{1},(\widetilde{(\widetilde{ki})l}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{27}&&-\,E_{3,q^\prime\to g}^{0}(k,1,l)\,A_3^{0}((\widetilde{kl}),i,j)\,B_{1,,II}^{\gamma,0}((\widetilde{ij}),\overline{1},(\widetilde{(\widetilde{kl})i}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{28}&&-\bigg[      +S^{FF}_{\overline{1}i[(\widetilde{ki}), (\widetilde{li})]}       +S^{FF}_{(\widetilde{ki})ij}       -S^{FF}_{[(\widetilde{ki}), (\widetilde{li})]ij}       -S^{FF}_{1i(\widetilde{ki})}       -S^{FF}_{ji\overline{1}}       +S^{FF}_{1ij}  \bigg]\nonumber\\
 &&\times E_{3,q^\prime\to g}^{0}((\widetilde{ki}),1,(\widetilde{li}))\,B_{1,,II}^{\gamma,0}(j,\overline{1},[(\widetilde{ki}), (\widetilde{li})],7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\end{eqnarray}


==> sub/autoqbCh0g1AT.tex <==
\section*{qbCh0g1AT(i,k,j,1,6,2)}
\begin{eqnarray}
  \ph{1}&&+\frac{1}{2}\,\,E_3^{0}(i,j,k)\,\hat{B}_{1,I}^{\gamma,1}((\widetilde{ij}),(\widetilde{jk}),1,6,2)\,\delta(1-x_1)\,\delta(1-x_2)\nonumber\\
  \ph{2}&&+\frac{1}{2}\,\,E_{3,q}^{0}(1,j,k)\,\hat{B}_{1,I}^{\gamma,1}(i,(\widetilde{jk}),\overline{1},6,2)\,\delta(1-x_1)\,\delta(1-x_2)\nonumber\\
  \ph{3}&&+\frac{1}{2}\,\,\hat{E}_{3}^{1}(i,j,k)\,B_{1,I}^{\gamma,0}((\widetilde{ij}),(\widetilde{jk}),1,6,2)\,\delta(1-x_1)\,\delta(1-x_2)\nonumber\\
  \ph{4}&&+\frac{1}{2}\,\,\hat{E}_{3,q}^{1}(1,j,k)\,B_{1,I}^{\gamma,0}(i,(\widetilde{jk}),\overline{1},6,2)\,\delta(1-x_1)\,\delta(1-x_2)\nonumber\\
  \ph{5}&&-\,E_{3,q^\prime\to g}^{0}(j,1,i)\,\hat{B}_{1,II}^{\gamma,1}((\widetilde{ij}),\overline{1},k,6,2)\,\delta(1-x_1)\,\delta(1-x_2)\nonumber\\
  \ph{6}&&-\,\hat{E}_{3,q^\prime}^{1}(j,1,i)\,B_{1,,II}^{\gamma,0}((\widetilde{ij}),\overline{1},k,6,2)\,\delta(1-x_1)\,\delta(1-x_2)\nonumber\\
\end{eqnarray}


==> sub/autoqbCt0g1AT.tex <==
\section*{qbCt0g1AT(i,k,j,1,6,2)}
\begin{eqnarray}
 \ph{1}&&+\bigg[ 
 +2J_{2,QQ}^{1,IF}(s_{1k})
 -2J_{2,QQ}^{1,FF}(s_{ki})
 -J_{2,QQ}^{1,IF}(s_{1i})
 -J_{2,QQ}^{1,FF}(s_{jk})
 +2J_{2,QQ}^{1,FF}(s_{ij})
 -2J_{2,QQ}^{1,IF}(s_{1j})\bigg]\,C_0^{\gamma,0}(i,k,j,1,6,2)\,J_2^{(3)}(\lbrace p\rbrace_{3})\nonumber\\
  \ph{2}&&+\frac{1}{2}\,\bigg[\,\tilde{E}_{3}^{1}(i,j,k)\,\delta(1-x_1)\,\delta(1-x_2)
 +J_{2,QQ}^{1,FF}(s_{jk})\,E_3^{0}(i,j,k)\bigg]\,B_{1,I}^{\gamma,0}((\widetilde{ij}),(\widetilde{jk}),1,6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
  \ph{3}&&+\frac{1}{2}\,\bigg[\,\tilde{E}_{3,q}^{1}(1,j,k)\,\delta(1-x_1)\,\delta(1-x_2)
 +J_{2,QQ}^{1,FF}(s_{jk})\,E_{3,q}^{0}(1,j,k)\bigg]\,B_{1,I}^{\gamma,0}(i,(\widetilde{jk}),\overline{1},6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
  \ph{4}&&+\frac{1}{2}\,\,E_3^{0}(i,j,k)\,\bigg[\,\tilde{B}_{1,I}^{\gamma,1}((\widetilde{ij}),(\widetilde{jk}),1,6,2)\,\delta(1-x_1)\,\delta(1-x_2)\nonumber\\
 &&\phantom{\bigg[}+J_{2,QQ}^{1,IF}(s_{1(\widetilde{ij})})\,B_{1,I}^{\gamma,0}((\widetilde{ij}),(\widetilde{jk}),1,6,2) \bigg]\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
  \ph{5}&&+\frac{1}{2}\,\,E_{3,q}^{0}(1,j,k)\,\bigg[\,\tilde{B}_{1,I}^{\gamma,1}(i,(\widetilde{jk}),\overline{1},6,2)\,\delta(1-x_1)\,\delta(1-x_2)\nonumber\\
 &&\phantom{\bigg[}+J_{2,QQ}^{1,IF}(s_{\overline{1}i})\,B_{1,I}^{\gamma,0}(i,(\widetilde{jk}),\overline{1},6,2) \bigg]\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
 \ph{6}&&-2\bigg[ +J_{2,QQ}^{1,IF}(s_{1k})
 +J_{2,QQ}^{1,FF}(s_{ij})
 -J_{2,QQ}^{1,IF}(s_{1j})
 -J_{2,QQ}^{1,FF}(s_{ki})
 \nonumber\\ &&+\bigg(  -{\cal S}^{FF}(s_{1k},s_{kj},x_{1k,kj})
 -{\cal S}^{FF}(s_{ij},s_{kj},x_{ij,kj})
 +{\cal S}^{FF}(s_{1j},s_{kj},x_{1j,kj})
 +{\cal S}^{FF}(s_{ki},s_{kj},x_{ki,kj})
 \bigg)\bigg]\nonumber\\
 &&\times E_3^{0}(i,j,k)\,B_{1,I}^{\gamma,0}((\widetilde{ij}),(\widetilde{jk}),1,6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
  \ph{7}&&-\frac{1}{2}\,\,E_{3,q^\prime\to g}^{0}(j,1,i)\,\bigg[\,\tilde{B}_{1,II}^{\gamma,1}((\widetilde{ij}),\overline{1},k,6,2)\,\delta(1-x_1)\,\delta(1-x_2)\nonumber\\
 &&\phantom{\bigg[}+J_{2,QQ}^{1,FF}(s_{k(\widetilde{ij})})\,B_{1,,II}^{\gamma,0}((\widetilde{ij}),\overline{1},k,6,2) \bigg]\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
  \ph{8}&&-\frac{1}{2}\,\,E_{3,q^\prime\to g}^{0}(k,1,i)\,\bigg[\,\tilde{B}_{1,II}^{\gamma,1}(j,\overline{1},(\widetilde{ik}),6,2)\,\delta(1-x_1)\,\delta(1-x_2)\nonumber\\
 &&\phantom{\bigg[}+J_{2,QQ}^{1,FF}(s_{j(\widetilde{ik})})\,B_{1,,II}^{\gamma,0}(j,\overline{1},(\widetilde{ik}),6,2) \bigg]\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
  \ph{9}&&-\frac{1}{2}\,\bigg[\,\tilde{E}_{3,q^\prime}^{1}(j,1,i)\,\delta(1-x_1)\,\delta(1-x_2)
 +J_{2,QQ}^{1,IF}(s_{1i})\,E_{3,q^\prime\to g}^{0}(j,1,i)\bigg]\,B_{1,,II}^{\gamma,0}((\widetilde{ij}),\overline{1},k,6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
  \ph{10}&&-\frac{1}{2}\,\bigg[\,\tilde{E}_{3,q^\prime}^{1}(k,1,i)\,\delta(1-x_1)\,\delta(1-x_2)
 +J_{2,QQ}^{1,IF}(s_{1i})\,E_{3,q^\prime\to g}^{0}(k,1,i)\bigg]\,B_{1,,II}^{\gamma,0}(j,\overline{1},(\widetilde{ik}),6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2})\nonumber\\
 \ph{11}&&+2\bigg[ +J_{2,QQ}^{1,IF}(s_{1k})
 +J_{2,QQ}^{1,FF}(s_{ij})
 -J_{2,QQ}^{1,IF}(s_{1j})
 -J_{2,QQ}^{1,FF}(s_{ki})
 \nonumber\\ &&+\bigg(  -{\cal S}^{FF}(s_{1k},s_{jk},x_{1k,jk})
 -{\cal S}^{FF}(s_{ij},s_{jk},x_{ij,jk})
 +{\cal S}^{FF}(s_{1j},s_{jk},x_{1j,jk})
 +{\cal S}^{FF}(s_{ki},s_{jk},x_{ki,jk})
 \bigg)\bigg]\nonumber\\
 &&\times E_3^{0}(j,1,i)\,B_{1,,II}^{\gamma,0}((\widetilde{ij}),\overline{1},k,6,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\end{eqnarray}


==> sub/autoqbCt1g0AS.tex <==
\section*{qbCt1g0AS(l,i,k,j,1,7,2)}
\begin{eqnarray}
\lefteqn{{\tt qbCt1g0AS(l,i,k,j,1,7,2) =}} \\
 \ph{1}&&+A_3^{0}(1,i,l)\,C_0^{\gamma,0}((\widetilde{il}),k,j,\overline{1},7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{2}&&+A_3^{0}(j,i,k)\,C_0^{\gamma,0}(l,(\widetilde{ki}),(\widetilde{ji}),1,7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{3}&&-2A_3^{0}(1,i,k)\,C_0^{\gamma,0}(l,(\widetilde{ki}),j,\overline{1},7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{4}&&-2A_3^{0}(j,i,l)\,C_0^{\gamma,0}((\widetilde{li}),k,(\widetilde{ji}),1,7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{5}&&+2A_3^{0}(1,i,j)\,C_0^{\gamma,0}(l,k,(\widetilde{ji}),\overline{1},7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{6}&&+2A_3^{0}(l,i,k)\,C_0^{\gamma,0}((\widetilde{li}),(\widetilde{ki}),j,1,7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{7}&&+E_3^{0}(l,j,k)\,\tilde{B}_{2,I}^{\gamma,0}((\widetilde{lj}),(\widetilde{kj}),i,1,7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
\snip \ph{8}&&+\,B_4^0(1,j,k,l)\,B_{1,I}^{\gamma,0}((\widetilde{jkl}),i,\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{9}&&-\,E_3^{0}(l,j,k)\,A_3^{0}(1,(\widetilde{kj}),(\widetilde{lj}))\,B_{1,I}^{\gamma,0}([(\widetilde{kj}), (\widetilde{lj})],i,\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\snip \ph{10}&&+\frac{1}{2}\,\,\tilde{E}_4^0(1,j,i,k)\,B_{1,I}^{\gamma,0}(l,(\widetilde{ijk}),\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{11}&&-\frac{1}{2}\,\,A_3^{0}(j,i,k)\,E_{3,q}^{0}(1,(\widetilde{ji}),(\widetilde{ki}))\,B_{1,I}^{\gamma,0}(l,[(\widetilde{ji}), (\widetilde{ki})],\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\snip \ph{12}&&+\frac{1}{2}\,\,\tilde{E}_4^0(l,j,i,k)\,B_{1,I}^{\gamma,0}((\widetilde{lji}),(\widetilde{kij}),1,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{13}&&-\frac{1}{2}\,\,A_3^{0}(j,i,k)\,E_3^{0}(l,(\widetilde{ji}),(\widetilde{ki}))\,B_{1,I}^{\gamma,0}((\widetilde{l\widetilde{(ji})}),[(\widetilde{ji}), (\widetilde{ki})],1,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{14}&&-\,E_3^{0}(l,j,k)\,A_3^{0}(1,i,(\widetilde{lj}))\,B_{1,I}^{\gamma,0}((\widetilde{i\widetilde{(lj})}),(\widetilde{jk}),\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{15}&&+\,A_3^{0}(1,i,k)\,E_3^{0}(\overline{1},(\widetilde{ik}),j)\,B_{1,I}^{\gamma,0}(l,(\widetilde{j\widetilde{(ik})}),\overline{\overline{1}},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{16}&&+\,A_3^{0}(j,i,l)\,E_3^{0}(1,k,(\widetilde{ji}))\,B_{1,I}^{\gamma,0}((\widetilde{li}),(\widetilde{k\widetilde{(ji})}),\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{17}&&-\,A_3^{0}(1,i,j)\,E_3^{0}(\overline{1},k,(\widetilde{ji}))\,B_{1,I}^{\gamma,0}(l,(\widetilde{k\widetilde{(ji})}),\overline{\overline{1}},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{18}&&-\,A_3^{0}(l,i,k)\,E_3^{0}(1,(\widetilde{ki}),j)\,B_{1,I}^{\gamma,0}((\widetilde{li}),(\widetilde{(\widetilde{ki})j}),\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{19}&&-\bigg[      +S^{FF}_{1i(\widetilde{ki})}       +S^{FF}_{(\widetilde{ji})il}       -S^{FF}_{1i(\widetilde{ji})}       -S^{FF}_{li(\widetilde{ik})}  \bigg]\nonumber\\
 &&\times E_3^{0}(1,(\widetilde{ki}),(\widetilde{ji}))\,B_{1,I}^{\gamma,0}(l,[(\widetilde{ki}), (\widetilde{ji})],\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{20}&&+\,A_3^{0}(1,i,k)\,E_3^{0}(l,(\widetilde{ik}),j)\,B_{1,I}^{\gamma,0}((\widetilde{l\widetilde{(ik})}),(\widetilde{j\widetilde{(ik})}),\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{21}&&+\,A_3^{0}(j,i,l)\,E_3^{0}((\widetilde{li}),k,(\widetilde{ji}))\,B_{1,I}^{\gamma,0}((\widetilde{(\widetilde{li})k}),(\widetilde{k\widetilde{(ji})}),1,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{22}&&-\,A_3^{0}(1,i,j)\,E_3^{0}(l,k,(\widetilde{ji}))\,B_{1,I}^{\gamma,0}((\widetilde{lk}),(\widetilde{k\widetilde{(ji})}),\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{23}&&-\,A_3^{0}(l,i,k)\,E_3^{0}((\widetilde{li}),(\widetilde{ki}),j)\,B_{1,I}^{\gamma,0}([(\widetilde{li}), (\widetilde{ki})],(\widetilde{(\widetilde{ki})j}),1,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{24}&&-\bigg[      +S^{FF}_{1i(\widetilde{ki})}       +S^{FF}_{(\widetilde{ji})il}       -S^{FF}_{1i(\widetilde{ji})}       -S^{FF}_{li(\widetilde{ik})}  \bigg]\nonumber\\
 &&\times E_3^{0}(l,(\widetilde{ki}),(\widetilde{ji}))\,B_{1,I}^{\gamma,0}((\widetilde{l\widetilde{(ki})}),[(\widetilde{ki}), (\widetilde{ji})],1,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{25}&&-\frac{1}{2}\,E_{3,q^\prime\to g}^{0}(j,1,l)\,sf2Bt2g0A((\widetilde{jl}),i,\overline{1},k,7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{26}&&-\frac{1}{2}\,E_{3,q^\prime\to g}^{0}(k,1,l)\,sf2Bt2g0A(j,\overline{1},i,(\widetilde{kl}),7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
\snip \ph{27}&&+\,B_4^0(j,1,l,k)\,{sB}_{1,II}^{\gamma,0}((\widetilde{jlk}),i,\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{28}&&-\frac{1}{2}\,\,E_{3,q^\prime\to g}^{0}(j,1,l)\,A_3^{0}((\widetilde{jl}),\overline{1},k)\,{sB}_{1,II}^{\gamma,0}((\widetilde{(\widetilde{jl})k}),i,\overline{\overline{1}},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{29}&&-\frac{1}{2}\,\,E_{3,q^\prime\to g}^{0}(k,1,l)\,A_3^{0}((\widetilde{kl}),\overline{1},j)\,{sB}_{1,II}^{\gamma,0}((\widetilde{(\widetilde{kl})j}),i,\overline{\overline{1}},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\snip \ph{30}&&-\frac{1}{2}\,\,\tilde{E}_4^0(j,1,i,l)\,B_{1,,II}^{\gamma,0}((\widetilde{jil}),\overline{1},k,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{31}&&+\frac{1}{2}\,\,A_3^{0}(1,i,l)\,E_{3,q^\prime\to g}^{0}(j,\overline{1},(\widetilde{il}))\,B_{1,,II}^{\gamma,0}((\widetilde{j\widetilde{(il})}),\overline{\overline{1}},k,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\snip \ph{32}&&-\frac{1}{2}\,\,\tilde{E}_4^0(k,1,i,l)\,B_{1,,II}^{\gamma,0}(j,\overline{1},(\widetilde{kil}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{33}&&+\frac{1}{2}\,\,A_3^{0}(1,i,l)\,E_{3,q^\prime\to g}^{0}(k,\overline{1},(\widetilde{il}))\,B_{1,,II}^{\gamma,0}(j,\overline{\overline{1}},(\widetilde{k\widetilde{(il})}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{34}&&+\frac{1}{2}\,\,E_{3,q^\prime\to g}^{0}(j,1,l)\,A_3^{0}((\widetilde{jl}),i,k)\,B_{1,,II}^{\gamma,0}((\widetilde{(\widetilde{jl})i}),\overline{1},(\widetilde{ki}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{35}&&+\frac{1}{2}\,\,E_{3,q^\prime\to g}^{0}(k,1,l)\,A_3^{0}((\widetilde{kl}),i,j)\,B_{1,,II}^{\gamma,0}((\widetilde{ij}),\overline{1},(\widetilde{(\widetilde{kl})i}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{36}&&-\,A_3^{0}(1,i,k)\,E_3^{0}((\widetilde{ik}),\overline{1},l)\,B_{1,,II}^{\gamma,0}(j,\overline{\overline{1}},(\widetilde{l\widetilde{(ik})}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{37}&&-\,A_3^{0}(j,i,l)\,E_3^{0}(k,1,(\widetilde{li}))\,B_{1,,II}^{\gamma,0}((\widetilde{ji}),\overline{1},(\widetilde{k\widetilde{(li})}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{38}&&+\,A_3^{0}(1,i,j)\,E_3^{0}(k,\overline{1},l)\,B_{1,,II}^{\gamma,0}((\widetilde{ji}),\overline{\overline{1}},(\widetilde{lk}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{39}&&+\,A_3^{0}(l,i,k)\,E_3^{0}((\widetilde{ki}),1,(\widetilde{li}))\,B_{1,,II}^{\gamma,0}(j,\overline{1},[(\widetilde{ki}), (\widetilde{li})],7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{40}&&+\bigg[      +S^{FF}_{1i(\widetilde{ik})}       +S^{FF}_{ji(\widetilde{li})}       -S^{FF}_{1ij}       -S^{FF}_{(\widetilde{li})i(\widetilde{ik})}  \bigg]\nonumber\\
 &&\times E_3^{0}((\widetilde{ik}),1,(\widetilde{li}))\,B_{1,,II}^{\gamma,0}(j,\overline{1},[(\widetilde{ik}), (\widetilde{li})],7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{41}&&-\,A_3^{0}(1,i,k)\,E_3^{0}(j,\overline{1},l)\,B_{1,,II}^{\gamma,0}((\widetilde{lj}),\overline{\overline{1}},(\widetilde{ki}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{42}&&-\,A_3^{0}(j,i,l)\,E_3^{0}((\widetilde{ji}),1,(\widetilde{li}))\,B_{1,,II}^{\gamma,0}([(\widetilde{ji}), (\widetilde{li})],\overline{1},k,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{43}&&+\,A_3^{0}(1,i,j)\,E_3^{0}((\widetilde{ji}),\overline{1},l)\,B_{1,,II}^{\gamma,0}((\widetilde{l\widetilde{(ji})}),\overline{\overline{1}},k,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{44}&&+\,A_3^{0}(l,i,k)\,E_3^{0}(j,1,(\widetilde{li}))\,B_{1,,II}^{\gamma,0}((\widetilde{j\widetilde{(li})}),\overline{1},(\widetilde{ki}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{45}&&-\bigg[      +S^{FF}_{1i(\widetilde{ij})}       +S^{FF}_{ki(\widetilde{li})}       -S^{FF}_{1ik}       -S^{FF}_{(\widetilde{li})i(\widetilde{ij})}  \bigg]\nonumber\\
 &&\times E_3^{0}((\widetilde{ij}),1,(\widetilde{li}))\,B_{1,,II}^{\gamma,0}([(\widetilde{ij}), (\widetilde{li})],\overline{1},k,7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\end{eqnarray}


==> sub/autoqbD0g1AT.tex <==
\section*{qbD0g1AT(i,1,j,k,6,2)}
\begin{eqnarray}
 \ph{1}&&+\bigg[ 
 +J_{2,QQ}^{1,IF}(s_{1k})
 +J_{2,QQ}^{1,FF}(s_{ji})\bigg]\,D_0^{\gamma,0}(i,1,j,k,6,2)\,J_2^{(3)}(\lbrace p\rbrace_{3})\nonumber\\
\end{eqnarray}


==> sub/autoqbD1g0AS.tex <==
\section*{qbD1g0AS(l,i,1,j,k,7,2)}
\begin{eqnarray}
\lefteqn{{\tt qbD1g0AS(l,i,1,j,k,7,2) =}} \\
 \ph{1}&&+A_3^{0}(1,i,k)\,D_0^{\gamma,0}(l,(\widetilde{ik}),j,\overline{1},7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{2}&&+A_3^{0}(j,i,l)\,D_0^{\gamma,0}((\widetilde{li}),k,(\widetilde{ji}),1,7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
\snip \ph{3}&&+2\,C_4^0(1,k,j,l)\,B_{1,I}^{\gamma,0}((\widetilde{jkl}),i,\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\snip \ph{4}&&+2\,C_4^0(k,1,j,l)\,B_{1,I}^{\gamma,0}(\overline{1},i,(\widetilde{jkl}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\snip \ph{5}&&+2\,C_4^0(l,j,k,1)\,B_{1,I}^{\gamma,0}((\widetilde{jkl}),i,\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\snip \ph{6}&&+2\,C_4^0(j,l,k,1)\,B_{1,I}^{\gamma,0}((\widetilde{jkl}),i,\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\end{eqnarray}


==> sub/autoqbDt0g1AT.tex <==
\section*{qbDt0g1AT(i,1,j,k,6,2)}
\begin{eqnarray}
 \ph{1}&&+\bigg[ 
 +J_{2,QQ}^{1,IF}(s_{1k})
 -J_{2,QQ}^{1,IF}(s_{1i})
 -J_{2,QQ}^{1,IF}(s_{1j})
 -J_{2,QQ}^{1,FF}(s_{jk})
 +J_{2,QQ}^{1,FF}(s_{ji})
 -J_{2,QQ}^{1,FF}(s_{ki})\bigg]\,D_0^{\gamma,0}(i,1,j,k,6,2)\,J_2^{(3)}(\lbrace p\rbrace_{3})\nonumber\\
\end{eqnarray}


==> sub/autoqbDt1g0AS.tex <==
\section*{qbDt1g0AS(l,i,1,j,k,7,2)}
\begin{eqnarray}
\lefteqn{{\tt qbDt1g0AS(l,i,1,j,k,7,2) =}} \\
 \ph{1}&&-A_3^{0}(1,i,k)\,D_0^{\gamma,0}(l,(\widetilde{ik}),j,\overline{1},7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{2}&&+A_3^{0}(1,i,l)\,D_0^{\gamma,0}((\widetilde{il}),k,j,\overline{1},7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{3}&&+A_3^{0}(1,i,j)\,D_0^{\gamma,0}(l,k,(\widetilde{ij}),\overline{1},7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{4}&&+A_3^{0}(j,i,k)\,D_0^{\gamma,0}(l,(\widetilde{ki}),(\widetilde{ji}),1,7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{5}&&-A_3^{0}(j,i,l)\,D_0^{\gamma,0}((\widetilde{li}),k,(\widetilde{ji}),1,7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
 \ph{6}&&+A_3^{0}(k,i,l)\,D_0^{\gamma,0}((\widetilde{li}),(\widetilde{ki}),j,1,7,2)\,J_2^{(3)}(\lbrace p\rbrace_{3}) \nonumber\\
\snip \ph{7}&&+2\,C_4^0(1,k,j,l)\,B_{1,I}^{\gamma,0}((\widetilde{jkl}),i,\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\snip \ph{8}&&+2\,C_4^0(k,1,j,l)\,B_{1,I}^{\gamma,0}(\overline{1},i,(\widetilde{jkl}),7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\snip \ph{9}&&+2\,C_4^0(l,j,k,1)\,B_{1,I}^{\gamma,0}((\widetilde{jkl}),i,\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\snip \ph{10}&&+2\,C_4^0(j,l,k,1)\,B_{1,I}^{\gamma,0}((\widetilde{jkl}),i,\overline{1},7,2)\,J_2^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\end{eqnarray}


==> sub/autoqbtoQBh1g2AU.tex <==
\section*{qbtoQBh1g2AU}
\begin{eqnarray}
\lefteqn{{\tt qbtoQBh1g2AU(1,3,4,5,2) =}} \\
 \ph{1}&&+\bigg[ 
 -\,{\cal B}_{4,q^\prime}^{0}(s_{14}) 
 -S_{q\to g}\,{\cal A}_{3,g\to q}^{0}(s_{14})\otimes\Gamma^{(1)}_{gq}(z_1) 
 -\,\Gamma^{(1)}_{gq}(z_1)\otimes\Gamma^{(1)}_{qg}(z_1) 
 \nonumber \\ && \phantom{+\bigg[} 
 +\,\Gamma^{(2)}_{qQ}(z_1) 
 +\,\Gamma^{(2)}_{q\bar{Q}}(z_1) 
 \bigg] 
 {sB}_1^{\gamma,0}(4,3,1,5,2)
 \nonumber\\
\end{eqnarray}


==> sub/autoqbtoQBth1g2AU.tex <==
\section*{qbtoQBth1g2AU}
\begin{eqnarray}
\lefteqn{{\tt qbtoQBth1g2AU(1,3,4,5,2) =}} \\
 \ph{1}&&+\bigg[ 
 +\,{\cal B}_{4,q^\prime}^{0}(s_{14}) 
 -\,\Gamma^{(2)}_{qQ}(z_1) 
 -\,\Gamma^{(2)}_{q\bar{Q}}(z_1) 
 \nonumber \\ && \phantom{+\bigg[} 
 +\,\Gamma^{(1)}_{gq}(z_1)\otimes\Gamma^{(1)}_{qg}(z_1) 
 +S_{q\to g}\,{\cal A}_{3,g\to q}^{0}(s_{14})\otimes\Gamma^{(1)}_{gq}(z_1) 
 \bigg] 
 {sB}_1^{\gamma,0}(4,3,1,5,2)
 \nonumber\\
\end{eqnarray}


==> sub/autoqbtogBh1g2AU.tex <==
\section*{qbtogBh1g2AU}
\begin{eqnarray}
\lefteqn{{\tt qbtogBh1g2AU(1,3,4,5,2) =}} \\
 \ph{1}&&+\bigg[ 
 +\,{\cal E}_{3,q^\prime \to g}^{0}(s_{13}) 
 +S_{q\to g}\,\Gamma^{(1)}_{gq}(z_1) 
 \bigg] 
\left( -\frac{b_0}{\epsilon}B_1^{\gamma,0}(4,1,3,5,2) +B_1^{\gamma,1}(4,1,3,5,2)\right)
 \nonumber\\
 \ph{2}&&+\bigg[ 
 +\,{\cal D}_{3,g\to g}^{0}(s_{13})\otimes{\cal E}_{3,q^\prime \to g}^{0}(s_{13}) 
 +\,{\cal D}_{3,g\to g}^{0}(s_{14})\otimes{\cal E}_{3,q^\prime \to g}^{0}(s_{13}) 
 -\,\Gamma^{(1)}_{gg}(z_1)\otimes{\cal E}_{3,q^\prime \to g}^{0}(s_{13}) 
 \nonumber \\ && \phantom{+\bigg[} 
 +S_{q\to g}\,{\cal D}_{3,g\to g}^{0}(s_{13})\otimes\Gamma^{(1)}_{gq}(z_1) 
 +S_{q\to g}\,{\cal D}_{3,g\to g}^{0}(s_{14})\otimes\Gamma^{(1)}_{gq}(z_1) 
 -S_{q\to g}\,\Gamma^{(1)}_{gg}(z_1)\otimes\Gamma^{(1)}_{gq}(z_1) 
 \bigg] 
 B_1^{\gamma,0}(4,1,3,5,2)
 \nonumber\\
 \ph{3}&&+\bigg[ 
 +\frac{b_0}{\epsilon}\,\bigg( \frac{s_{13}}{\mu_R^2}\bigg)^{-\epsilon}\,{\cal E}_{3,q^\prime \to g}^{0}(s_{13}) 
 -S_{q\to g}\,{\cal A}_{3,g\to q}^{0}(s_{14})\otimes\Gamma^{(1)}_{gq}(z_1) 
 +2S_{q\to g}\,{\cal D}_{3,g\to q}^{0}(s_{13})\otimes\Gamma^{(1)}_{gq}(z_1) 
 \nonumber \\ && \phantom{+\bigg[} 
 +\frac{1}{2}S_{q\to g}\,\Gamma^{(1)}_{gg}(z_1)\otimes\Gamma^{(1)}_{gq}(z_1) 
 -\frac{1}{2}S_{q\to g}\,\Gamma^{(1)}_{gq}(z_1)\otimes\Gamma^{(1)}_{qq}(z_1) 
 -2\,{\cal D}_{3,g\to g}^{0}(s_{13})\otimes{\cal E}_{3,q^\prime \to g}^{0}(s_{13}) 
 \nonumber \\ && \phantom{+\bigg[} 
 +\,\Gamma^{(1)}_{gg}(z_1)\otimes{\cal E}_{3,q^\prime \to g}^{0}(s_{13}) 
 -\,\Gamma^{(1)}_{qq}(z_1)\otimes{\cal E}_{3,q^\prime \to g}^{0}(s_{13}) 
 +S_{q\to g}\,\Gamma^{(2)}_{gq}(z_1) 
 \nonumber \\ && \phantom{+\bigg[} 
 +\,{\cal E}_{4,q^\prime}^{0}(s_{13}) 
 +\,{\cal E}_{4,\bar{q}^\prime}^{0}(s_{13}) 
 +\,{\cal{E}}_{3,q^\prime}^{1}(s_{13}) 
 \nonumber \\ && \phantom{+\bigg[} 
 -\,{\cal B}_{4,q^\prime}^{0}(s_{14}) 
 \bigg] 
 B_1^{\gamma,0}(4,1,3,5,2)
 \nonumber\\
\end{eqnarray}


==> sub/autoqbtogBhh1g2AU.tex <==
\section*{qbBhh1g2AUqtog}
\begin{eqnarray}
\lefteqn{{\tt qbBhh1g2AUqtog(1,3,4,5,2) =}} \\
 \ph{1}&&+\bigg[ 
 +\,{\cal E}_{3,q^\prime \to g}^{0}(s_{13}) 
 +S_{q\to g}\,\Gamma^{(1)}_{gq}(z_1) 
 \bigg] 
\left( -\frac{b_F}{\epsilon}B_1^{\gamma,0}(4,1,3,5,2) +\hat{B}_1^{\gamma,1}(4,1,3,5,2)\right)
 \nonumber\\
 \ph{2}&&+\bigg[ 
 +\frac{b_F}{\epsilon}\,\bigg( \frac{s_{13}}{\mu_R^2}\bigg)^{-\epsilon}\,{\cal E}_{3,q^\prime \to g}^{0}(s_{13}) 
 -\frac{1}{2}S_{q\to g}\,\Gamma^{(1)}_{gg,F}(z_1)\otimes\Gamma^{(1)}_{gq}(z_1) 
 +S_{q\to g}\,\Gamma^{(2)}_{gq,F}(z_1) 
 \nonumber \\ && \phantom{+\bigg[} 
 +\,\hat{\cal{E}}_{3,q^\prime}^{1}(s_{13}) 
 \bigg] 
 B_1^{\gamma,0}(4,1,3,5,2)
 \nonumber\\
\end{eqnarray}


==> sub/autoqbtogBth1g2AU.tex <==
\section*{qbtogBth1g2AU}
\begin{eqnarray}
\lefteqn{{\tt qbtogBth1g2AU(1,3,4,5,2) =}} \\
 \ph{1}&&+\bigg[ 
 -S_{q\to g}\,\Gamma^{(1)}_{gq}(z_1) 
 -\frac{1}{2}\,\,{\cal E}_{3,q^\prime \to g}^{0}(s_{13}) 
 -\frac{1}{2}\,\,{\cal E}_{3,q^\prime \to g}^{0}(s_{14}) 
 \bigg] 
 \tilde{B}_3^{\gamma,1}(4,1,3,5,2)
 \nonumber\\
 \ph{2}&&+\bigg[ 
 -S_{q\to g}\,\Gamma^{(1)}_{gq}(z_1)\otimes{\cal A}_{3}^{0}(s_{34}) 
 -\frac{1}{2}\,\,{\cal E}_{3,q^\prime \to g}^{0}(s_{13})\otimes{\cal A}_{3}^{0}(s_{34}) 
 -\frac{1}{2}\,\,{\cal E}_{3,q^\prime \to g}^{0}(s_{14})\otimes{\cal A}_{3}^{0}(s_{34}) 
 \bigg] 
 B_1^{\gamma,0}(4,1,3,5,2)
 \nonumber\\
 \ph{3}&&+\bigg[ 
 +1/4S_{q\to g}\,\Gamma^{(1)}_{qq}(z_1)\otimes\Gamma^{(1)}_{gq}(z_1) 
 +\frac{1}{2}\,\,\Gamma^{(1)}_{qq}(z_1)\otimes{\cal E}_{3,q^\prime \to g}^{0}(s_{13}) 
 +\frac{1}{2}S_{q\to g}\,\widetilde{\Gamma}^{(2)}_{gq}(z_1) 
 \nonumber \\ && \phantom{+\bigg[} 
 -\frac{1}{4}\,\,\tilde{\cal E}_{4,\bar{q}^\prime}^{0}(s_{13}) 
 -\frac{1}{4}\,\,\tilde{\cal E}_{4,q^\prime}^{0}(s_{13}) 
 -\frac{1}{2}\,\,\tilde{\cal{E}}_{3,q^\prime}^{1}(s_{13}) 
 \bigg] 
 B_1^{\gamma,0}(4,1,3,5,2)
 \nonumber\\
 \ph{4}&&+\bigg[ 
 +1/4S_{q\to g}\,\Gamma^{(1)}_{qq}(z_1)\otimes\Gamma^{(1)}_{gq}(z_1) 
 +\frac{1}{2}\,\,\Gamma^{(1)}_{qq}(z_1)\otimes{\cal E}_{3,q^\prime \to g}^{0}(s_{14}) 
 +\frac{1}{2}S_{q\to g}\,\widetilde{\Gamma}^{(2)}_{gq}(z_1) 
 \nonumber \\ && \phantom{+\bigg[} 
 -\frac{1}{4}\,\,\tilde{\cal E}_{4,\bar{q}^\prime}^{0}(s_{14}) 
 -\frac{1}{4}\,\,\tilde{\cal E}_{4,q^\prime}^{0}(s_{14}) 
 -\frac{1}{2}\,\,\tilde{\cal{E}}_{3,q^\prime}^{1}(s_{14}) 
 \bigg] 
 B_1^{\gamma,0}(4,1,3,5,2)
 \nonumber\\
\end{eqnarray}


==> sub/autoqtoQBh1g2AU.tex <==
\section*{qtoQBh1g2AU}
\begin{eqnarray}
\lefteqn{{\tt qtoQBh1g2AU(1,3,4,5,2) =}} \\
 \ph{1}&&+\bigg[ 
 -\,{\cal B}_{4,q^\prime}^{0}(s_{14}) 
 -S_{q\to g}\,{\cal A}_{3,g\to q}^{0}(s_{14})\otimes\Gamma^{(1)}_{gq}(z_1) 
 -\,\Gamma^{(1)}_{gq}(z_1)\otimes\Gamma^{(1)}_{qg}(z_1) 
 \nonumber \\ && \phantom{+\bigg[} 
 +\,\Gamma^{(2)}_{qQ}(z_1) 
 +\,\Gamma^{(2)}_{q\bar{Q}}(z_1) 
 \bigg] 
 {sB}_1^{\gamma,0}(1,3,4,5,2)
 \nonumber\\
\end{eqnarray}


==> sub/autoqtoQBth1g2AU.tex <==
\section*{qtoQBth1g2AU}
\begin{eqnarray}
\lefteqn{{\tt qtoQBth1g2AU(1,3,4,5,2) =}} \\
 \ph{1}&&+\bigg[ 
 +\,{\cal B}_{4,q^\prime}^{0}(s_{14}) 
 -\,\Gamma^{(2)}_{qQ}(z_1) 
 -\,\Gamma^{(2)}_{q\bar{Q}}(z_1) 
 \nonumber \\ && \phantom{+\bigg[} 
 +\,\Gamma^{(1)}_{gq}(z_1)\otimes\Gamma^{(1)}_{qg}(z_1) 
 +S_{q\to g}\,{\cal A}_{3,g\to q}^{0}(s_{14})\otimes\Gamma^{(1)}_{gq}(z_1) 
 \bigg] 
 {sB}_1^{\gamma,0}(1,3,4,5,2)
 \nonumber\\
\end{eqnarray}


==> sub/autoqtogBh1g2AU.tex <==
\section*{qtogBh1g2AU}
\begin{eqnarray}
\lefteqn{{\tt qtogBh1g2AU(1,3,4,5,2) =}} \\
 \ph{1}&&+\bigg[ 
 +\,{\cal E}_{3,q^\prime \to g}^{0}(s_{13}) 
 +S_{q\to g}\,\Gamma^{(1)}_{gq}(z_1) 
 \bigg] 
\left( -\frac{b_0}{\epsilon}B_1^{\gamma,0}(3,1,4,5,2) +B_1^{\gamma,1}(3,1,4,5,2)\right)
 \nonumber\\
 \ph{2}&&+\bigg[ 
 +\,{\cal D}_{3,g\to g}^{0}(s_{13})\otimes{\cal E}_{3,q^\prime \to g}^{0}(s_{13}) 
 +\,{\cal D}_{3,g\to g}^{0}(s_{14})\otimes{\cal E}_{3,q^\prime \to g}^{0}(s_{13}) 
 -\,\Gamma^{(1)}_{gg}(z_1)\otimes{\cal E}_{3,q^\prime \to g}^{0}(s_{13}) 
 \nonumber \\ && \phantom{+\bigg[} 
 +S_{q\to g}\,{\cal D}_{3,g\to g}^{0}(s_{13})\otimes\Gamma^{(1)}_{gq}(z_1) 
 +S_{q\to g}\,{\cal D}_{3,g\to g}^{0}(s_{14})\otimes\Gamma^{(1)}_{gq}(z_1) 
 -S_{q\to g}\,\Gamma^{(1)}_{gg}(z_1)\otimes\Gamma^{(1)}_{gq}(z_1) 
 \bigg] 
 B_1^{\gamma,0}(3,1,4,5,2)
 \nonumber\\
 \ph{3}&&+\bigg[ 
 +\frac{1}{2}S_{q\to g}\,\Gamma^{(1)}_{gg}(z_1)\otimes\Gamma^{(1)}_{gq}(z_1) 
 -S_{q\to g}\,{\cal A}_{3,g\to q}^{0}(s_{14})\otimes\Gamma^{(1)}_{gq}(z_1) 
 +2S_{q\to g}\,{\cal D}_{3,g\to q}^{0}(s_{13})\otimes\Gamma^{(1)}_{gq}(z_1) 
 \nonumber \\ && \phantom{+\bigg[} 
 -\frac{1}{2}S_{q\to g}\,\Gamma^{(1)}_{gq}(z_1)\otimes\Gamma^{(1)}_{qq}(z_1) 
 +\frac{b_0}{\epsilon}\,{\cal E}_{3,q^\prime \to g}^{0}(s_{13})\,\bigg( \frac{s_{13}}{\mu_R^2}\bigg)^{-\epsilon} 
 -2\,{\cal D}_{3,g\to g}^{0}(s_{13})\otimes{\cal E}_{3,q^\prime \to g}^{0}(s_{13}) 
 \nonumber \\ && \phantom{+\bigg[} 
 +\,\Gamma^{(1)}_{gg}(z_1)\otimes{\cal E}_{3,q^\prime \to g}^{0}(s_{13}) 
 -\,\Gamma^{(1)}_{qq}(z_1)\otimes{\cal E}_{3,q^\prime \to g}^{0}(s_{13}) 
 +S_{q\to g}\,\Gamma^{(2)}_{gq}(z_1) 
 \nonumber \\ && \phantom{+\bigg[} 
 +\,{\cal E}_{4,q^\prime}^{0}(s_{13}) 
 +\,{\cal E}_{4,\bar{q}^\prime}^{0}(s_{13}) 
 +\,{\cal{E}}_{3,q^\prime}^{1}(s_{13}) 
 \nonumber \\ && \phantom{+\bigg[} 
 -\,{\cal B}_{4,q^\prime}^{0}(s_{14}) 
 \bigg] 
 B_1^{\gamma,0}(3,1,4,5,2)
 \nonumber\\
\end{eqnarray}


==> sub/autoqtogBhh1g2AU.tex <==
\section*{qBhh1g2AUqtog}
\begin{eqnarray}
\lefteqn{{\tt qBhh1g2AUqtog(1,3,4,5,2) =}} \\
 \ph{1}&&+\bigg[ 
 +\,{\cal E}_{3,q^\prime \to g}^{0}(s_{13}) 
 +S_{q\to g}\,\Gamma^{(1)}_{gq}(z_1) 
 \bigg] 
\left( -\frac{b_F}{\epsilon}B_1^{\gamma,0}(3,1,4,5,2) +\hat{B}_1^{\gamma,1}(3,1,4,5,2)\right)
 \nonumber\\
 \ph{2}&&+\bigg[ 
 +\frac{b_F}{\epsilon}\,\bigg( \frac{s_{13}}{\mu_R^2}\bigg)^{-\epsilon}\,{\cal E}_{3,q^\prime \to g}^{0}(s_{13}) 
 -\frac{1}{2}S_{q\to g}\,\Gamma^{(1)}_{gg,F}(z_1)\otimes\Gamma^{(1)}_{gq}(z_1) 
 +S_{q\to g}\,\Gamma^{(2)}_{gq,F}(z_1) 
 \nonumber \\ && \phantom{+\bigg[} 
 +\,\hat{\cal{E}}_{3,q^\prime}^{1}(s_{13}) 
 \bigg] 
 B_1^{\gamma,0}(3,1,4,5,2)
 \nonumber\\
\end{eqnarray}


==> sub/autoqtogBth1g2AU.tex <==
\section*{qtogBth1g2AU}
\begin{eqnarray}
\lefteqn{{\tt qtogBth1g2AU(1,3,4,5,2) =}} \\
 \ph{1}&&+\bigg[ 
 -S_{q\to g}\,\Gamma^{(1)}_{gq}(z_1) 
 -\frac{1}{2}\,\,{\cal E}_{3,q^\prime \to g}^{0}(s_{13}) 
 -\frac{1}{2}\,\,{\cal E}_{3,q^\prime \to g}^{0}(s_{14}) 
 \bigg] 
 \tilde{B}_3^{\gamma,1}(3,1,4,5,2)
 \nonumber\\
 \ph{2}&&+\bigg[ 
 -S_{q\to g}\,\Gamma^{(1)}_{gq}(z_1)\otimes{\cal A}_{3}^{0}(s_{34}) 
 -\frac{1}{2}\,\,{\cal E}_{3,q^\prime \to g}^{0}(s_{13})\otimes{\cal A}_{3}^{0}(s_{34}) 
 -\frac{1}{2}\,\,{\cal E}_{3,q^\prime \to g}^{0}(s_{14})\otimes{\cal A}_{3}^{0}(s_{34}) 
 \bigg] 
 B_1^{\gamma,0}(3,1,4,5,2)
 \nonumber\\
 \ph{3}&&+\bigg[ 
 +1/4S_{q\to g}\,\Gamma^{(1)}_{qq}(z_1)\otimes\Gamma^{(1)}_{gq}(z_1) 
 +\frac{1}{2}\,\,\Gamma^{(1)}_{qq}(z_1)\otimes{\cal E}_{3,q^\prime \to g}^{0}(s_{13}) 
 +\frac{1}{2}S_{q\to g}\,\widetilde{\Gamma}^{(2)}_{gq}(z_1) 
 \nonumber \\ && \phantom{+\bigg[} 
 -\frac{1}{4}\,\,\tilde{\cal E}_{4,\bar{q}^\prime}^{0}(s_{13}) 
 -\frac{1}{4}\,\,\tilde{\cal E}_{4,q^\prime}^{0}(s_{13}) 
 -\frac{1}{2}\,\,\tilde{\cal{E}}_{3,q^\prime}^{1}(s_{13}) 
 \bigg] 
 B_1^{\gamma,0}(3,1,4,5,2)
 \nonumber\\
 \ph{4}&&+\bigg[ 
 +1/4S_{q\to g}\,\Gamma^{(1)}_{qq}(z_1)\otimes\Gamma^{(1)}_{gq}(z_1) 
 +\frac{1}{2}\,\,\Gamma^{(1)}_{qq}(z_1)\otimes{\cal E}_{3,q^\prime \to g}^{0}(s_{14}) 
 +\frac{1}{2}S_{q\to g}\,\widetilde{\Gamma}^{(2)}_{gq}(z_1) 
 \nonumber \\ && \phantom{+\bigg[} 
 -\frac{1}{4}\,\,\tilde{\cal E}_{4,\bar{q}^\prime}^{0}(s_{14}) 
 -\frac{1}{4}\,\,\tilde{\cal E}_{4,q^\prime}^{0}(s_{14}) 
 -\frac{1}{2}\,\,\tilde{\cal{E}}_{3,q^\prime}^{1}(s_{14}) 
 \bigg] 
 B_1^{\gamma,0}(3,1,4,5,2)
 \nonumber\\
\end{eqnarray}


==> sub/autotestZ.tex <==
\section*{qqpC1g0ZS(1,i,k,2,j,Z)}
\begin{eqnarray}
 \ph{1}&&+A_{3,q}^{0}(1,i,k)\,C_0^{Z,0}(\overline{1},(\widetilde{ik}),2,j,Z)\,J_1^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{2}&&-E_{3,qq^\prime\to qg}^{0}(1,k,2)\,B_2^{Z,0}(\overline{1},i,\overline{2},j,Z)\,J_1^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{3}&&-E_{3,qq^\prime\to qg}^{0}(2,j,1)\,B_2^{Z,0}(\overline{2},\overline{1},i,k,Z)\,J_1^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{4}&&+A_{3,q}^{0}(2,i,j)\,C_0^{Z,0}(1,k,\overline{2},(\widetilde{ij}),Z)\,J_1^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{5}&&-E_{3,qq^\prime\to qg}^{0}(1,k,2)\,B_2^{Z,0}(\overline{1},\overline{2},i,j,Z)\,J_1^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
 \ph{6}&&-E_{3,qq^\prime\to qg}^{0}(2,j,1)\,B_2^{Z,0}(\overline{2},i,\overline{1},k,Z)\,J_1^{(2)}(\lbrace p\rbrace_{2}) \nonumber\\
\snip \ph{7}&&-\,E_4^0(1,2,k,i)\,B_1^{Z,0}(\overline{1},\overline{2},j,Z)\,J_1^{(1)}(\lbrace p\rbrace_{1}) \nonumber\\
 \ph{8}&&+\,E_{3,qq^\prime\to qg}^{0}(1,k,2)\,D_{3,qg}^{0}(\overline{1},\overline{2},i)\,B_1^{Z,0}(\overline{\overline{1}},\overline{\overline{2}},j,Z)\,J_1^{(1)}(\lbrace p\rbrace_{1}) \nonumber\\
 \ph{9}&&+\,A_{3,q}^{0}(1,i,k)\,E_{3,qq^\prime\to qg}^{0}(\overline{1},(\widetilde{ik}),2)\,B_1^{Z,0}(\overline{\overline{1}},\overline{2},j,Z)\,J_1^{(1)}(\lbrace p\rbrace_{1}) \nonumber\\
\snip \ph{10}&&-\,E_4^0(2,j,1,i)\,B_1^{Z,0}(\overline{2},\overline{1},k,Z)\,J_1^{(1)}(\lbrace p\rbrace_{1}) \nonumber\\
 \ph{11}&&+\,E_{3,qq^\prime\to qg}^{0}(2,j,1)\,D_{3,gq}^{0}(\overline{2},i,\overline{1})\,B_1^{Z,0}(\overline{\overline{2}},\overline{\overline{1}},k,Z)\,J_1^{(1)}(\lbrace p\rbrace_{1}) \nonumber\\
\snip \ph{12}&&+\,B_4^0(1,k,2,j)\,B_1^{Z,0}(\overline{1},i,\overline{2},Z)\,J_1^{(1)}(\lbrace p\rbrace_{1}) \nonumber\\
 \ph{13}&&-\,E_{3,qq^\prime\to qg}^{0}(1,k,2)\,A_{3,qg\to qq}^{0}(\overline{1},\overline{2},j)\,B_1^{Z,0}(\overline{\overline{1}},i,\overline{\overline{2}},Z)\,J_1^{(1)}(\lbrace p\rbrace_{1}) \nonumber\\
\snip \ph{14}&&-\,E_4^0(1,k,2,i)\,B_1^{Z,0}(\overline{1},\overline{2},j,Z)\,J_1^{(1)}(\lbrace p\rbrace_{1}) \nonumber\\
 \ph{15}&&+\,E_{3,qq^\prime\to qg}^{0}(1,k,2)\,D_{3,qg}^{0}(\overline{1},i,\overline{2})\,B_1^{Z,0}(\overline{\overline{1}},\overline{\overline{2}},j,Z)\,J_1^{(1)}(\lbrace p\rbrace_{1}) \nonumber\\
\snip \ph{16}&&-\,E_4^0(2,1,j,i)\,B_1^{Z,0}(\overline{2},\overline{1},k,Z)\,J_1^{(1)}(\lbrace p\rbrace_{1}) \nonumber\\
 \ph{17}&&+\,E_{3,qq^\prime\to qg}^{0}(2,j,1)\,D_{3,gq}^{0}(\overline{2},\overline{1},i)\,B_1^{Z,0}(\overline{\overline{2}},\overline{\overline{1}},k,Z)\,J_1^{(1)}(\lbrace p\rbrace_{1}) \nonumber\\
 \ph{18}&&+\,A_{3,q}^{0}(2,i,j)\,E_{3,qq^\prime\to qg}^{0}(\overline{2},(\widetilde{ij}),1)\,B_1^{Z,0}(\overline{\overline{2}},\overline{1},k,Z)\,J_1^{(1)}(\lbrace p\rbrace_{1}) \nonumber\\
\snip \ph{19}&&+\,B_4^0(2,j,1,k)\,B_1^{Z,0}(\overline{2},i,\overline{1},Z)\,J_1^{(1)}(\lbrace p\rbrace_{1}) \nonumber\\
 \ph{20}&&-\,E_{3,qq^\prime\to qg}^{0}(2,j,1)\,A_{3,qg\to qq}^{0}(\overline{2},\overline{1},k)\,B_1^{Z,0}(\overline{\overline{2}},i,\overline{\overline{1}},Z)\,J_1^{(1)}(\lbrace p\rbrace_{1}) \nonumber\\
 \ph{21}&&+\,A_{3,q}^{0}(2,i,j)\,E_{3,qq^\prime\to qg}^{0}(1,k,\overline{2})\,B_1^{Z,0}(\overline{1},\overline{\overline{2}},(\widetilde{ij}),Z)\,J_1^{(1)}(\lbrace p\rbrace_{1}) \nonumber\\
 \ph{22}&&+\,A_{3,q}^{0}(1,i,k)\,E_{3,qq^\prime\to qg}^{0}(2,j,\overline{1})\,B_1^{Z,0}(\overline{2},\overline{\overline{1}},(\widetilde{ik}),Z)\,J_1^{(1)}(\lbrace p\rbrace_{1}) \nonumber\\
 \ph{23}&&-\,E_{3,qq^\prime\to qg}^{0}(2,j,1)\,A_{3,q}^{0}(\overline{2},i,k)\,B_1^{Z,0}(\overline{\overline{2}},\overline{1},(\widetilde{ik}),Z)\,J_1^{(1)}(\lbrace p\rbrace_{1}) \nonumber\\
 \ph{24}&&+\,A_{3,q}^{0}(2,i,k)\,E_{3,qq^\prime\to qg}^{0}(\overline{2},j,1)\,B_1^{Z,0}(\overline{\overline{2}},\overline{1},(\widetilde{ik}),Z)\,J_1^{(1)}(\lbrace p\rbrace_{1}) \nonumber\\
 \ph{25}&&-\,E_{3,qq^\prime\to qg}^{0}(1,k,2)\,A_{3,q}^{0}(\overline{1},i,j)\,B_1^{Z,0}(\overline{\overline{1}},\overline{2},(\widetilde{ij}),Z)\,J_1^{(1)}(\lbrace p\rbrace_{1}) \nonumber\\
 \ph{26}&&+\,A_{3,q}^{0}(1,i,j)\,E_{3,qq^\prime\to qg}^{0}(\overline{1},k,2)\,B_1^{Z,0}(\overline{\overline{1}},\overline{2},(\widetilde{ij}),Z)\,J_1^{(1)}(\lbrace p\rbrace_{1}) \nonumber\\
 \ph{27}&&-\bigg[      +S^{IF}_{1i(\widetilde{ik})}       -S^{IF}_{\overline{1}i(\widetilde{ik})}       +S^{IF}_{\overline{2}i(\widetilde{ik})}       -S^{IF}_{\overline{\overline{2}}i(\widetilde{ik})}       -S^{IF}_{1i\overline{2}}       +S^{IF}_{\overline{1}i\overline{\overline{2}}}  \bigg]\nonumber\\
 &&\times E_{3,qq^\prime\to qg}^{0}(\overline{2},j,1)\,B_1^{Z,0}(\overline{\overline{2}},\overline{1},(\widetilde{ik}),Z)\,J_1^{(1)}(\lbrace p\rbrace_{1}) \nonumber\\
 \ph{28}&&-\bigg[      +S^{IF}_{\overline{1}i(\widetilde{ij})}       -S^{IF}_{\overline{\overline{1}}i(\widetilde{ij})}       +S^{IF}_{2i(\widetilde{ij})}       -S^{IF}_{\overline{2}i(\widetilde{ij})}       -S^{IF}_{2i\overline{1}}       +S^{IF}_{\overline{2}i\overline{\overline{1}}}  \bigg]\nonumber\\
 &&\times E_{3,qq^\prime\to qg}^{0}(\overline{1},k,2)\,B_1^{Z,0}(\overline{\overline{1}},\overline{2},(\widetilde{ij}),Z)\,J_1^{(1)}(\lbrace p\rbrace_{1}) \nonumber\\
\end{eqnarray}

